Disk dissipation, giant planet formation and star-formation-rate fluctuations in the past three-million-year history of Gould's Belt

Although episodic star formation (SF) had been suggested for nearby SF regions, a panoramic view to the latest episodic SF history in the solar neighborhood is still missing. By uniformly constraining the slope $\alpha$ of infrared spectral energy distributions (SEDs) of young stellar objects (YSOs) in the 13 largest Gould's Belt (GB) protoclusters surveyed by Spitzer Space Telescope, we have constructed a cluster-averaged histogram of $\alpha$ representing YSO evolution lifetime as a function of the $\alpha$ value. Complementary to the traditional SED classification scheme (0, I, F, II, III) that is based on different $\alpha$ values, a staging scheme (A,B,C,D,E) of SED evolution is advised on the basis of the $\alpha$ statistical features that can be better matched to the physical stages of disk dissipation and giant planet formation. This has also allowed us to unravel the fluctuations of star formation rate (SFR) in the past three-million-year (3 Myr) history of these GB protoclusters. Diverse evolutionary patterns such as single peak, double peaks and on-going acceleration of SFR are revealed. The SFR fluctuations are between $20\%\sim60\%$ ($\sim40\%$ on average) and no dependence on the average SFR or the number of SFR episodes is found. However, spatially close protoclusters tend to share similar SFR fluctuation trends, indicating that the driving force of the fluctuations should be at size scales beyond the typical cluster sizes of several parsec.

==> cjk-4.8.5/ChangeLog <==
2021-10-16  Werner LEMBERG  <wl@gnu.org>

	Version 4.8.5 released
	======================

	Set version to 4.8.5.

	* doc/history.txt: Updated.

	Update headers in all text files.

2021-10-16  Werner LEMBERG  <wl@gnu.org>

	[hbf2gf] Update config and auxiliary scripts.

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub,
	utils/hbf2gf/install-sh, utils/hbf2gf/mkinstalldirs: Updated to
	current versions.

	* utils/hbf2gf/configure: Regenerated with autoconf 2.71.

2021-10-16  Werner Lemberg  <wl@gnu.org>

	Update to current LaTeX version.

	Currently, there is a first-aid patch in the LaTeX kernel to make
	the CJK package work.  This commit moves the corresponding code to
	here so that the first-aid stuff can be removed.

	* texinput/CJK.sty (\IfFormatAtLeastTF): New macro.
	(\selectfont): Use the `\selectfont' hook for recent LaTeX versions.

2018-11-25  Werner Lemberg  <wl@gnu.org>

	Generate pinyin hyphenation pattern files from last commit.

	* utils/pyhyphen/hyph-zh-latn-pinyin.tex,
	utils/pyhyphen/hyph-zh-latn-tonepinyin.tex: New files.

2018-11-25  Werner Lemberg  <wl@gnu.org>

	Rewrite pinyin hyphenation support.

	Investigation has shown that the apostrophe before a syllable
	starting with `a', `e', or `o' should vanish if a line break occurs. 
	This commit fixes this bug: The apostrophe should now be entered
	with the Babel shorthand "'; character ' itself is no longer part of
	the hyphenation patterns.

	It also adds support for pinyin syllables with tone markers, to be
	used with Unicode engines like XeTeX or luatex.

	Finally, the license for the resulting pattern files have been
	changed from GPL to MIT to allow broader usage.

	* utils/pyhyphen/GNUmakefile: New file.  Saying `make' will generate
	the hyphenation pattern files `hyph-zh-latn-pinyin.tex' and
	`hyph-zh-latn-tonepinyin.tex'.

	* utils/pyhyphen/hyph-zh-latn-pinyin.in,
	utils/pyhyphen/make-patterns.sh: New auxiliary files.

	* utils/pyhyphen/pyhyph.tex: Removed.  Obsolete.

	* utils/pyhyphen/pytestutf8.tex: New file to demonstrate patterns
	for tone pinyin.

	* utils/pyhyphen/pinyin.c, utils/pyhyphen/pinyin.ldf,
	utils/pyhyphen/pinyin.tr, utils/pytest.tex: Updated.

	* doc/pyhyphen.txt, MANIFEST: Updated.

2016-12-27  Werner Lemberg  <wl@gnu.org>

	* utils/lisp/emacs/cjk-enc.el (cjk-coding): Remove `chinese-big5'.

	Hin-Tak reports this doesn't work...

2016-12-26  Hin-Tak Leung <htl10@users.sourceforge.net>

	[cjk-enc.el] Updated to work with Emacs 25 and later.

	In batch mode, `message' in Emacs 25+ obeys coding-system-for-write.

	  http://git.savannah.gnu.org/cgit/emacs.git/commit/?h=emacs-25&id=c63246628461f748d66a8a07ba008de2e00fd33a

	`cjk-encode' can mis-behave and, at worst, crash from `message'
	recursing.

	  https://debbugs.gnu.org/cgi/bugreport.cgi?bug=25203

	The charset priority system introduced with Emacs 23+ changes
	further in Emacs 25+.  Charset `big5' has been updated (together
	with `big5-hkscs') and now takes priority over the historical
	`chinese-big5-2' and `chinese-big5-1'.

	  http://git.savannah.gnu.org/cgit/emacs.git/commit/?h=emacs-25&id=9f89ea1f84dbf708228ced0202774b36f30f2b01
	  http://git.savannah.gnu.org/cgit/emacs.git/commit/?h=emacs-25&id=49fa1919e9be863f22ec8042704bf3436d0ec26d

	Also worth noting is that, "Wrote output.cjk" is no longer seen with
	Emacs 25+.

	  http://git.savannah.gnu.org/cgit/emacs.git/commit/?h=emacs-25&id=d20f82e6f1ab902469723ebd530ca21bea9cc41b

	Tested against example/{Big5.tex, Big5vert.tex, CJKbabel.tex,
	muletest.tex, rubytest.tex, thai.tex}, and LANG'ed non-'coding:'ed
	big5 example, with emacs 21.4, 22.3, 23.3, 24.5 and 25.1.

	Thanks for advice from Eli Zaretskii.

	* utils/lisp/emacs/cjk-enc.el (cjk-enc-table,
	cjk-format-spec-table): Add `big5' encoding.
	(cjk-coding): Add `chinese-big5'.
	(cjk-encode): Adjust Big5 language detection heuristics for Emacs
	25+; support `big5' encoding.
	Use `terminal-coding-system' while emitting messages.

2015-04-18  Werner LEMBERG  <wl@gnu.org>

	Version 4.8.4 released
	======================

	Set version to 4.8.4.

	* doc/history.txt: Updated.

	* Makefile (distsrc, distdoc): Use tar's `ustar' format.
	Compress better.

	Update headers in all text files.

2015-04-18  Werner LEMBERG  <wl@gnu.org>

	[hbf2gf] Update aux scripts.

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub,
	utils/hbf2gf/install-sh: Updated to current versions.

2014-08-31  Peter Breitenlohner  <peb@mppmu.mpg.de>

	[hbf2gf]: Avoid undefined behaviour when `char' is signed.

	* utils/hbf2gf/hbf.c (match, add_property, skip_word, get_line): Use
	proper cast.
	* utils/hbf2gf/hbf2gf.w (fsearch, <Check for environment
	variables>): Ditto.

2014-08-31  Peter Breitenlohner  <peb@mppmu.mpg.de>

	* utils/hbf2gf/hbf2hf.w (path_open): Drop unused variable.

2014-06-28  Leo Liu  <leoliu.pku@gmail.com>

	[CJKutf8] Fix space handing of non-CJK characters.

	* texinput/CJKutf8.sty (\CJK@XX, \CJK@XXp, \CJK@XXX, \CJK@XXXp):
	Only apply \CJK@ignorespaces for CJK characters (or rather, only for
	multibyte sequences that don't map to a `\u8:...' macro).

2012-09-13  Werner LEMBERG  <wl@gnu.org>

	* examples/CJKutf8.tex: Add Greek.

	This finally works due to the recent lgrx package which delivers
	good Babel UTF8 support for LGR encoding.

	An unsolved problem yet, however, is proper cut-and-paste support.
	While dvipdfmx properly generates CMaps for CJK encodings (even
	for virtual fonts which pdftex doesn't handle at all), it doesn't
	handle encodings like LGR correctly, something the `cmap' package
	provides for pdflatex.

2012-08-26  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\Unicode): Fix conditional to allow line breaks.

	Problem reported by Jinsong Zhao <jszhao@yeah.net>; it seems that
	this bug has been there since from the beginning.

2012-06-21  Werner LEMBERG  <wl@gnu.org>

	Make some commands robust.

	* texinput/CJK.sty (\CJKtilde, \standardtilde, \CJKspace,
	\CJKnospace): Use \DeclareRobustCommand.

2012-05-20  Peter Breitenlohner  <peb@mppmu.mpg.de>

	[hbf2gf] Build fix for 64-bit Mac OS X 10.7.3.

	* utils/hbf2gf/hbf2gf.w: Clang does not like non-static inline
	functions as used here.  While at it, all local functions are
	declared static.
	Do not extend #ifdef HAVE_EMTEXDIR...#endif over several sections.

2012-05-08  Werner LEMBERG  <wl@gnu.org>

	* texlive/cjk.pl: Add missing file.

2012-05-07  Werner LEMBERG  <wl@gnu.org>

	Version 4.8.3 released
	======================

	Set version to 4.8.3.

	* doc/history.txt: Updated.

	* Makefile (CJK2DVI, LATEX2DVI): Set TFMFONTS.

	Update headers in all text files.

2012-05-07  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub,
	utils/hbf2gf/install-sh, utils/hbf2gf/mkinstalldirs: Updated to
	current versions.

	* utils/hbf2gf/configure: Regenerated with autoconf 2.69.

2012-05-07  Werner LEMBERG  <wl@gnu.org>

	[thai] Update to font-tlwg 0.5.

	* doc/thaifont.txt, utils/thaifont/tools/INSTALL: Updated.

	* utils/thaifont/texmf/fonts/tfm/public/norasi/ftnr8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnb8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnbo8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftno8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdr8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdb8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdbo8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdo8z.tfm: Regenerated
	with fontinst.

2012-05-05  Hin-Tak Leung  <htl10@users.sourceforge.net>

	[cjk-enc.el] Accept Thai input in utf-8 encoding.

	* utils/lisp/emacs/cjk-enc.el: Treat Unicode 0x0EXX inputs as Thai.

	* examples/thai_utf8.tex: New sample file.

	* Makefile (DISTTARGETS): Add `thai_utf8.tex'.
	(thai_utf8): New target.

	* MANIFEST, texlive/cjk.pl: Updated.

2012-05-05  Werner LEMBERG  <wl@gnu.org>

	Remove xCJK files.

	The stuff is obsolete and no longer works out of the box.  Given
	that there exists the `xeCJK' package, those files are really
	useless today.

	* examples/xCJK.tex, texinput/UTF8/xUTF8.chr,
	texinput/UTF8/xUTF8.enc, texinput/xCJK.sty, texinput/xpmC.chr,
	texinput/xpmC.enc, doc/xCJK.txt: Removed.

	* MANIFEST, texlive/cjk.pl: Updated.

	* Makefile (XELATEX, xCJK): Removed.
	(DISTTARGETS): Updated.

2012-05-05  Qing Lee  <sobenlee@gmail.com>

	[CJKfntef] Fix incompatibility with `ulem.sty'.

	* texinput/CJKfntef.tex (\CJKunderdot): Version 2010-01-21 of
	`ulem.sty' silently adds a line which redefines \par (its author
	says this was an oversight).  This exhibits a bug in \CJKunderdot
	which implicitly emits \par by inserting an \hskip command in
	vertical mode.  Simply omitting this \hskip fixes the issue.

2012-04-20  Werner LEMBERG  <wl@gnu.org>

	* texinput/Bg5/Bg5.cpx, texinput/JIS/JIS.cpx: Fix typos.

2012-04-20  Werner LEMBERG  <wl@gnu.org>

	* texinput/UTF8/zh-Hans.cpx: Synchronize.

2012-04-20  Jiangsheng Yu  <yujs@ittc.ku.edu>

	* texinput/GB/GB.cap, texinput/GB/GB.cpx: Improve.

2011-12-16 Hin-Tak Leung <htl10@users.sourceforge.net>

	[cjk-enc.el] Make it work with emacs 23 and newer.

	Emacs 23+ introduces native Unicode support and uses a new charset
	priority system: `char-charset' and `split-char' preferably now
	return the Unicode charset and code points, respectively;
	non-Unicode charsets and code points are only used if they have a
	higher charset priority.  On the other hand, information on the
	original charset is preserved in the text property `charset'.

	Another change is the new charset/text-property called `tis620-2533'
	(a superset of `ascii' and `thai-tis620'), introduced in emacs 23.
	This has the tendency of swallowing up every ASCII character and
	goes into an infinite loop with `examples/thai.tex', so we have to
	handle this also.

	Tested with emacs 22.3 and 23.3, and
	EMACS_PRETEST_24_0_92-142-g559675b on examples/{CJKbabel.tex,
	muletest.tex, rubytest.tex, thai.tex}.

	* utils/lisp/emacs/cjk-enc.el [emacs version >= 23]:
	`make-coding-system' is deprecated -- use `define-coding-system'
	instead.

	Use the `charset' text property instead of the outcome of
	`char-charset' to explicitly set the charset priority; this makes
	`split-char' work as with emacs 22 and earlier.

	Set new optional `restriction' argument of `char-charset' to avoid
	problems with `tis620-2533'.

2011-12-03  Werner LEMBERG  <wl@gnu.org>

	* examples/thai.tex: Improve prologue comments.

2011-10-04  Werner LEMBERG  <wl@gnu.org>

	[CEFconv, SJISconv] Document missing range 0xF0-0xFC.

	* utils/CEFconv/cefsconv.w, utils/SJISconv/sjisconv.w: Do it.

2011-10-04  Peter Breitenlohner  <peb@mppmu.mpg.de>

	[cjklatex] Don't include `kpathsea/win32lib.h'.
	This is already done from `kpathsea/config.h'.

	* utils/cjklatex/cjklatex.c: Implement it.

2011-10-04  Peter Breitenlohner  <peb@mppmu.mpg.de>

	[cefconv] Various fixes.

	* utils/CEFconv/cef5conv.w: Fix output so that it really works as
	bg5conv + cefconv.
	* utils/CEFconv/cefsconv.w: Fix output so that it really works as
	sjisconv + cefconv.
	* utils/CEFconv/cefconv.w: Typo.

2011-09-03  Peter Breitenlohner  <peb@mppmu.mpg.de>

	[cjklatex] Introduce `LATEX' preprocessor macro.

	* utils/cjklatex/cjklatex.c (LATEX): New macro.  Use it where
	appropriate to remove the hardcoded usage of `latex'.  For example,
	LATEX can be defined as `pdflatex' (as done in TeXLive).

2011-09-03  Peter Breitenlohner  <peb@mppmu.mpg.de>

	[cjklatex] Various updates to stay in sync with TeXLive.

	* utils/cjklatex/cjklatex.c: Include kpathsea/win32lib.h instead of
	win32lib.h directly.
	Decorate with `const'.
	(usage_str, CJKtable): Updated.

2011-09-03  Werner LEMBERG  <wl@gnu.org>

	[hbf2gf] Update manpage.

	* utils/hbf2gf/hbf2gf.1, doc/hbf2gf.txt: Remove information on
	ancient kpathsea versions.

2011-09-03  Peter Breitenlohner  <peb@mppmu.mpg.de>

	[hbf2gf] Update kpathsea support.

	* utils/hbf2gf/hbf2gf.w (OLD_KPATHSEA, VERY_OLD_KPATHSEA): Removed.
	(DllImport, KPSEDLL): Removed.
	[HAVE_CONFIG_H]: Include `c-auto.h'.

2011-09-03  Peter Breitenlohner  <peb@mppmu.mpg.de>

	[hbf2gf] Decorate with `const'.

	* utils/hbf2gf/hbf2gf.w, utils/hbf2gf/hbf.c: Do it.

2011-09-03  Peter Breitenlohner  <peb@mppmu.mpg.de>

	Adapt utility programs to ANSI C.

	* utils/Bg5conv/bg5conv.w, utils/CEFconv/cefconv.w,
	utils/CEFconv/cef5conv.w, utils/CEFconv/cefsconv.w,
	utils/SJISconv/sjisconv.w, utils/extconv/extconv.w,
	utils/hbf2gf/hbf.c, utils/hbf2gf/hbf2gf.w: Do it.

2011-02-07  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.txt: Document possible problems in `tabular' environment.
	Problem reported by LI Ruo-Meng <15003990378@163.com>.

2010-01-04  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.txt: Document Babel bug related to ^^xx notation.
	Problem reported by Peter Grzybek <peter.grzybek@uni-graz.at>.

2009-11-07  Werner LEMBERG  <wl@gnu.org>

	Fix line breaks with furigana.

	* texinput/ruby.txt (\ruby): If the furigana is smaller than
	the base glyph, really behave as documented, this is, behave like an
	ordinary CJK character.

2009-08-25  Werner LEMBERG  <wl@gnu.org>

	* examples/CJKfntef.tex: Updated.

2009-08-25  Wenchang Sun  <sunwch@hotmail.com>

	New macros for CJKfntef.sty.

	* texinput/CJKfntef.sty (\varCJKunderline, \CJKunderanyline,
	\CJKunderanysymbol): New macros.
	(\CJKunderdot): Fix interaction with XeTeX.

	* doc/history.txt: Document it.

2009-08-25  Wenchang Sun  <sunwch@hotmail.com>

	* texinput/CJKfntef.sty: Replace \global with \CJKf@global.

2009-01-19  Werner LEMBERG  <wl@gnu.org>

	* texlive/cjk-build.pl: Remove unused stuff.
	From Karl Berry.

2009-01-05  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.txt: Document usage of CJKutf8.sty with beamer class.

2008-12-29  Werner LEMBERG  <wl@gnu.org>

	Version 4.8.2 released
	======================

	Set version to 4.8.2.

	* doc/history.txt: Updated.

	Update headers in all text files.

2008-12-29  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub,
	utils/hbf2gf/install-sh, utils/hbf2gf/mkinstalldirs: Updated to
	current versions.

	* utils/hbf2gf/configure: Regenerated with autoconf 2.63.

2008-12-29  Werner LEMBERG  <wl@gnu.org>

	* doc/TeXLive.txt: Replaced with...
	* texlive/*.pl: These new files which define the various TeXLive
	packages derived from the CJK bundle.

	* MANIFEST: Updated.

2008-12-28  Werner LEMBERG  <wl@gnu.org>

	* doc/history.txt: Updated.

	* doc/CJKnumb.txt: New file.

	* MANIFEST: Updated.

2008-12-28  Werner LEMBERG  <wl@gnu.org>

	Rename garuda & norasi stuff to garuda-c90 & norasi-c90.

	* MANIFEST, doc/thaifont.txt, utils/thaifont/tools/INSTALL: Updated.

	* utils/thaifont/texmf/dvips/garuda/config.garuda: Moved to...
	* utils/thaifont/texmf/dvips/garuda-c90/config.garuda-c90: This
	file.  Updated.
	* utils/thaifont/texmf/dvips/norasi/config.norasi: Moved to...
	* utils/thaifont/texmf/dvips/norasi-c90/config.norasi-c90: This
	file.  Updated.
	* utils/thaifont/texmf/fonts/map/dvips/garuda/garuda.map: Moved
	to...
	* utils/thaifont/texmf/fonts/map/dvips/garuda-c90/garuda-c90.map:
	This file.
	* utils/thaifont/texmf/fonts/map/dvips/norasi/norasi.map: Moved
	to...
	* utils/thaifont/texmf/fonts/map/dvips/norasi-c90/norasi-c90.map:
	This file.
	* utils/thaifont/texmf/fonts/tfm/public/garuda/*: Moved to...
	* utils/thaifont/texmf/fonts/tfm/public/garuda-c90/*: This
	directory.
	* utils/thaifont/texmf/fonts/tfm/public/norasi/*: Moved to...
	* utils/thaifont/texmf/fonts/tfm/public/norasi-c90/*: This
	directory.
	* utils/thaifont/tools/garuda.fontinst: Moved to...
	* utils/thaifont/tools/garuda-c90.fontinst: This file.
	* utils/thaifont/tools/norasi.fontinst: Moved to...
	* utils/thaifont/tools/norasi-c90.fontinst: This file.

2008-12-28  Werner LEMBERG  <wl@gnu.org>

	* contrib/wadalab/DNP.txt: Renamed to...
	* contrib/wadalab/wadalab.txt: This.
	* MANIFEST: Updated.

2008-12-28  Werner LEMBERG  <wl@gnu.org>

	Use same font names as in thailatex.

	* doc/thaifont.txt,
	utils/thaifont/texmf/fonts/map/dvips/garuda/garuda.map,
	utils/thaifont/texmf/fonts/map/dvips/norasi/norasi.map: Updated.


	Update to thailatex 0.4.2.

	* doc/thaifont.txt,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnr8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnb8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnbo8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftno8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdr8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdb8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdbo8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdo8z.tfm: Regenerated
	with fontinst.

2008-11-25  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKnumb.sty: Use U+3007 (IDEOGRAPHIC NUMBER ZERO),
	not U+25CB (WHITE CIRCLE).

	* texinput/UTF8/c70bkai.fdx, texinput/UTF8/c70bsmi.fdx: Map U+25CB
	to U+3007.
	* texinput/UTF8/c70gbsn.fdx, texinput/UTF8/c70gkai.fdx,
	texinput/UTF8/c70mj.fdx: New files which do the same.

	* MANIFEST: Updated.

2008-11-25  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\Unicode): Use vertical glyph representation
	forms.

2008-11-25  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKnumb.sty (\CJKdigits*): New command to use traditional
	form of glyph zero.

	* doc/history.txt: Updated.

2008-10-01  Werner LEMBERG  <wl@gnu.org>

	* *.fd: Add \CJKnormal to all font families which use \CJKbold.  This
	is necessary because NFSS doesn't call \selectfont if a font gets
	substituted by another one (and \selectfont resets the \CJK@bold@
	flag).  Here an example (where `gbsn' uses \CJKbold for boldface
	emulation):

	  \begin{CJK*}{GB}{gbsn}
	  {\bf\CJKchar{"D6}{"D0}}
	  {\em\CJKchar{"D6}{"D0}}
	  \end{CJK*}

2008-09-23  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/subfonts.pe: Fix error message for too-old
	FontForge versions.

2008-08-21  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/subfonts.pe: Handle CID-keyed fonts.

2008-08-10  Werner LEMBERG  <wl@gnu.org>

	Version 4.8.1 released
	======================

	Set version to 4.8.1.

	* doc/history.txt, README: Updated.

	* doc/TeXLive.txt: Updated.
	PDF man pages are now autogenerated in TeXLive.

	Update headers in all text files.

	* utils/hbf2gf/config.sub: Updated to current version.

2008-08-03  Werner LEMBERG  <wl@gnu.org>

	Add some missing files.  Found by Daniel Flipo.

	* texinput/Bg5/c00bkai.fd, texinput/GB/c10gkai.fd,
	texinput/GB/c10gkai.fdx: New files.

	* MANIFEST: Updated.

2008-07-11  Werner LEMBERG  <wl@gnu.org>

	Make macros in pinyin.sty robust.

	Problem reported by Denis Roegel <roegel@loria.fr>.

	* texinput/pinyin.sty (\py@macron): Make it work again with Plain
	TeX.
	(\py@@@): No longer needed.
	(\py@): Do what \py@@@ did formerly.
	(py@DRC): New macro to make the pinyin syllables robust.
	Update all pinyin syllable macro definitions to use it.

	* doc/history.txt: Updated.

2008-07-11  Werner LEMBERG  <wl@gnu.org>

	Incorporate Wen-Chang's CJKspace package.

	* texinput/CJKspace.sty, examples/CJKspace.tex, doc/CJKspace.txt:
	New files.
	* texinput/CJK.sty (\CJK@@@): New signature macro for CJKspace.sty.
	(\CJK@namedef, \CJK@namepdef, \CJK@nameppdef, \CJK@namepppdef,
	\CJK@nameppppdef): Use it.

	* Makefile, doc/history.txt, MANIFEST: Updated.

2008-05-22  Werner LEMBERG  <wl@gnu.org>

	Version 4.8.0 released
	======================

	Set version to 4.8.0.

	* doc/history.txt, doc/INSTALL, doc/TeXLive.txt, README: Updated.

	Update headers in all text files.

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub: Updated to
	current versions.

	* utils/hbf2gf/configure: Regenerated with autoconf 2.62.

2008-05-18  Werner LEMBERG  <wl@gnu.org>

	* Makefile (DISTDIRS): We are now using git, not CVS.

2008-05-18  Werner LEMBERG  <wl@gnu.org>

	* doc/history.txt: Mention xCJK.sty.

2008-05-17  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\CJK@UnicodeEnc): New macro (so that xCJK.sty
	can overwrite it).
	* texinput/CJKnumb.sty: Use it.

	* texinput/xCJK.sty: Simplify -- unicode mappings to other encodings
	are no longer supported (since it hasn't worked for Big5 or GBK
	anyway).

	(\xCJK@xUTF): Removed.
	(\CJKsymbol): Simplified.
	(\toutf@XXX): Removed.
	(\xCJK@CJKenc, \CJKenc): Removed.
	(\CJK@envStart): Produce error if encoding is not `UTF8'.
	Simplified.
	(\xCJK@setenc, \CJK@xpmC, \xCJK@enc@UTF8, \xCJK@xUTF8@hook):
	Removed.
	(\CJK@xUTF8@hook, \CJK@UnicodeEnc): New macros.
	(\xCJK@@char): Removed.
	(\CJK@XXpdf): Simplified.
	(\CJK@@XXpdf): Removed.

	Add support for non-BMP Unicode.

	(\CJK@nameppppdef): New macro.
	(\xCJK@char): Redefined.
	(\xCJK@@char, \xCJK@@@char): New macros.
	(\CJK@XXp, \CJK@XXXp): Redefined.
	(\CJK@XXXXp): New macro.

	xdvipdfmx automatically handles UTF-8 encoded bookmarks.

	(\xCJK@four, \xCJK@@@char, <\if@filesw>): Removed.

	(\special): Use \utfout.

2008-05-12  Danai SAE-HAN  <danai.sae-han@edpnet.be>

	* utils/hbf2gf/hbf2gf.1: Replace some `-' with `\-'.

2008-03-10  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/hbf2gf.1: s|-|\-| where appropriate.

2008-03-09  Werner LEMBERG  <wl@gnu.org>

	* Makefile (XELATEX): Call xelatex twice.
	(manpages): Increase font size to 11pt for DVI and PDF output.

2008-03-09  Werner LEMBERG  <wl@gnu.org>

	Add support for EUC-JP with DNP font encoding.

	* texinput/CJK.enc (\CJK@@@EUC-JPdnp@hook, \CJK@EUC-JPdnp@enc): New
	macros.

	* texinput/JIS/EUC-JPdnp.enc: New file.

	* texinput/JIS/EUC-JP.chr (\CJK@shiftchar): Define \CJK@plane as
	empty.

	* doc/history.txt, MANIFEST: Updated.

2008-03-09  Werner LEMBERG  <wl@gnu.org>

	Make \CJK@bold work with C49 encoding too.  The idea is to handle
	the font as a CJK font but with \CJK@plane set to empty.

	* texinput/SJIS/SJIS.chr, texinput/SJIS/SJIdnp.chr (\CJK@sjischar):
	Define \CJK@plane as empty.

	* texinput/SJIS/c49song.fd: Use `CJK' size function.

	* doc/history.txt: Updated.

2008-03-03  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKutf8.sty, texinput/xCJK.sty,
	texinput/mule/MULEenc.sty: Use \ProvidesPackage, not \ProvidesFile.

2008-03-03  Werner LEMBERG  <wl@gnu.org>

	Better control for \baselinestretch with CJKvert.sty.

	* texinput/CJKvert.sty (usebaselinestretch): New option.
	(\CJKbaselinestretch): New macro.

	* doc/history.txt, doc/vertical.txt: Document it.

2008-02-11  Werner LEMBERG  <wl@gnu.org>

	* doc/xCJK.txt: New file.
	* MANIFEST: Updated.

2008-02-11  Werner LEMBERG  <wl@gnu.org>

	* doc/fonts.txt: Document installation of cyberbit.ttf.

2008-02-05  Werner LEMBERG  <wl@gnu.org>

	Add SUN Wen-Chang's xCJK bundle.

	* examples/xCJK.tex, texinput/UTF8/xUTF8.chr,
	texinput/UTF8/xUTF8.enc, texinput/xCJK.sty, texinput/xpmC.chr,
	texinput/xpmC.enc: New files.

	* MANIFEST: Updated.

	* Makefile (XELATEX): New macro.
	(xCJK): New target.
	(CJK2DVI, LATE2DVI): Simplify.

2008-01-15  Gernot Hassenpflug  <aikishugyo@gmail.com>

	* contrib/wadalab/c70goth.fdx, contrib/wadalab/c70min.fdx,
	contrib/wadalab/c70maru.fdx: Rotate more glyphs for vertical
	typesetting.
	Shift small kana for vertical typesetting.
	Other minor improvements.

2007-12-27  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/vertical.pe, utils/subfonts/vertref.pe: Abort if no
	vertical glyph representation forms are available.

2006-12-05  Werner LEMBERG  <wl@gnu.org>

	Make pinyin syllables work with \MakeUppercase and \MakeLowercase.

	* pinyin.sty: Almost completely rewrite macro logic to replace e.g.
	`\py@@@a' with `\py@ a' so that the argument gets handled by
	\MakeUppercase.

2006-12-04  Werner LEMBERG  <wl@gnu.org>

	Make pinyin syllables work with hyperref bookmarks.

	* pinyin.sty: Use \AtBeginDocument hook to add missing characters to
	PU encoding needed for pinyin syllables.
	Use \AtBeginDocument hook to set up some replacement macros for
	bookmarks.
	(\py@hr@macron, \py@hr@v): New replacement macros for
	bookmarks.

2007-11-23  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.enc: Add punctuation tables for GBK encoding.

2007-11-06  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/subfonts.pe, utils/subfonts/vertical.pe,
	utils/subfonts/vertref.pe: Put current time stamp into copyright
	string.
	Need FontForge 20071105 or newer.

2007-11-02  SUN Wenchang  <sunwch@hotmail.com>

	* texinput/CJKfntef.sty (\CJK@preUnderdot): Use \cdot (in math mode).
	(\CJKxout): Use `/' in math mode.
	(\CJKunderdotbasesep, \CJKunderdotsep): Adjusted.

2007-10-26  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/vertical.pe: Use glyph names of the horizontal
	representation glyphs with an appended `.vert'.  This makes dvipdfmx
	automatically create a correct /ToUnicode CMap.

2007-10-25  Werner LEMBERG  <wl@gnu.org>

	Provide final fix for patch 2007-10-04.

	* utils/subfonts/makefdx.pl: Provide flag `-u' to produce a CMap
	macro in the FDX file.
	Don't specify FDX file directly on the command line but give family
	name and encoding separately which are then concatenated to give the
	FDX name (we need the family name separately).
	Add code to produce a macro which provides a /ToUnicode CMap entry
	as needed by pdfTeX.
	Fix loop to not omit last glyph.

	* texinput/UTF8/c70bsmi.fdx, texinput/UTF8/c70bkai.fdx: Regenerated.
	These now provide the macros \CJK@cmap@bsmiv and \CJK@cmap@bkaiv,
	respectively.

	* texinput/CJKutf8.sty (\pickup@font): Call `\CJK@cmap@...' if it
	exists.

2007-10-04  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKutf8.sty (\pickup@font): Disable generation of
	ToUnicode cmap for `v' subfont (which holds vertical representation
	glyphs).  This is a temporary hack; the right solution is to modify
	makefdx.pl so that it creates a ToUnicode macro for the specific
	font; \CJK@addcmap should be then modified to use this macro instead
	of autogenerating a cmap.

	Problem reported by Edward G.J. Lee.

2007-09-10  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/vertical.pe, utils.subfonts/vertref.pe: Adapt to
	FontForge version 2007-Sep-10 and newer.

2007-07-26  Gernot Hassenpflug  <gernot@nict.go.jp>

	* contrib/wadalab/c70goth.fdx, contrib/wadalab/c70min.fdx,
	contrib/wadalab/c70maru.fdx: New files to support vertical writing
	with Unicode encoded Wadalab fonts.

2007-07-07  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty (\ding): Rename to...
	(\py@ding): This to make \ding work actually.

2007-05-04  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKvert.sty (\CJKsymbol): Honour \CJKhdef{offset}{...}.
	* doc/fdxfiles.txt, doc/history.txt: Document it.

2007-04-08  Werner LEMBERG  <wl@gnu.org>

	* utils/pyhyphen/pyhyph.tex: Replace latin-1 characters with
	^^xx sequences.  Suggested by David Kastrup.

	* doc/cjk-enc.txt: Document special space handling for Emacs quail
	input methods.

2006-11-06  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty (\py@macron, \py@@@v): Support T5 encoding.
	* doc/history.txt: Document it.

2006-10-31  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.txt, doc/CJKutf8.txt: Mention Byte Order Mark in UTF-8.

2006-10-19  Werner LEMBERG  <wl@gnu.org>

	* doc/TeXLive.txt, MANIFEST: Minor fixes.

	* Makefile (DVI2PDF): Add argument for paper format.
	(CONVERT, MULE, LATEX): Add optional argument for paper format;
	default to `letter'.
	(manpages, cweb): Use letter paper format.
	(READMEb5): Use A4 paper.

	* examples/README: Minor fix.

2006-10-17  Werner LEMBERG  <wl@gnu.org>

	Version 4.7.0 released
	======================

	Set version to 4.7.0.

	* doc/history.txt, doc/INSTALL, doc/TeXLive.txt, README: Updated.

	Update headers in all text files.

2006-10-09  Werner LEMBERG  <wl@gnu.org>

	* Makefile (abs-distdir): Fix assignment.
	(distdoc): Remove generated C files.

	* utils/hbf2gf/hbf2gf.1: s/`/\(oq/ and s/'/\(cq/ where appropriate.

2006-10-06  Werner LEMBERG  <wl@gnu.org>

	* doc/CJKutf8.txt, doc/history.txt: Minor additions.
	* MANIFEST: Sorted and updated.

2006-10-05  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKutf8.sty (\CJK@surr): Use \expandafter to make
	\uppercase work actually.

	* texinput/CJK.sty (\CJK@makeActive, \CJK@makeInactive): Handle 0x80
	also (which is needed for UTF8).

2006-10-05  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKutf8.sty (\CJK@surr): New function.
	(\CJK@addcmap): Use \CJK@surr so that values > U+FFFF are correctly
	represented as surrogates.

2006-09-30  Werner LEMBERG  <wl@gnu.org>

	In CJKutf8.sty, add ToUnicode cmaps for pdfTeX.  Note, however, that
	it currently fails with virtual fonts: pdftex 3.141592-1.30.4-2.2
	can't resolve them to the used base fonts.

	* texinput/CJKutf8.sty: Require ifpdf package.
	(\pickup@font) [\ifpdf]: Redefine, adding a call to CJK@addcmap.
	(\CJK@addcmap) [\ifpdf]: New function.

	* doc/history.txt: Updated.

2006-09-16  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\CJK@ifundefined): New macro.
	Update all affected files where possible to use it instead of
	\@ifundefined.  This fixes a bug reported by Danai which made
	\chapter work in the `scrartcl' article class (instead of
	reporting an error) after using a CJK caption file.

	* *.cap, *.cpx: Don't redefine \thepart but use its previous
	definition for \partformat.  This fixes a bug reported by Danai
	which produced bad TOC entries.

	* doc/history.txt: Updated.

2006-09-12  Werner LEMBERG  <wl@gnu.org>

	* texinput/UTF8/ko-Hanj.cpx: Renamed to...
	* texinput/UTF8/ko-Hani.cpx: This to use the correct ISO 15924
	script tag.

	* doc/history.txt, doc/CJK.txt: Updated.

2006-09-08  Werner LEMBERG  <wl@gnu.org>

	Add caption files for UTF8 encoding.

	* texinput/UTF8/{ja,ko-Hang,ko-Hang2,ko-Hanj,zh-Hans,zh-Hant}.cap:
	New files.

	* doc/history.txt, doc/CJK.txt: Mention them.

2006-08-31  Werner LEMBERG  <wl@gnu.org>

	Reimplement the \CJKbold mechanism to call the last argument of
	\DeclareFontShape each time the font is selected only if a CJK size
	function has been used.  This fixes shape declarations like the ones
	in the fourier package which rely on being called only once.

	* texinput/CJK.sty (\CJK@curr@fontshape): New macro.
	(\CJK@empty, \CJK@fixed, \CJK@sub, \CJK@DNPgen, \CJK@DNP): Define a
	macro where the name is the argument of \CJK@curr@fontshape.
	(\selectfont): Execute macro where the name is the argument of
	\CJK@curr@fontshape only if it exists.

	* doc/history.txt, doc/CJK.txt: Mention it.

2006-08-29  Danai SAE-HAN  <danai.sae-han@skynet.be>

	* utils/subfonts/hlatex2agl.pl: Make it accept a third parameter
	which specifies the used SFD file.
	(process_afmfile, process_pfbfile): Add minor tweaks to handle fonts
	generated with other tools than FontForge.

2006-08-29  Werner LEMBERG  <wl@gnu.org>

	* utils/Bg5conv/bg5conv.w, utils/extconv/extconv.w,
	utils/hbf2gf/hbf2gf.w, utils/CEFconv/cefconv.w,
	utils/CEFconv/cef5conv.w, utils/CEFconv/cefsconv.w,
	utils/SJISconv/sjisconv.w: s/@/@@/ in email address.

	* utils/Bg5conv/bg5conv.c, utils/extconv/extconv.c,
	utils/hbf2gf/hbf2gf.c, utils/CEFconv/cefconv.c,
	utils/CEFconv/cef5conv.c, utils/CEFconv/cefsconv.c,
	utils/SJISconv/sjisconv.c: Removed.  These files are now generated
	by the Makefile.

	* Makefile (version): Set to 4.7.0.
	(CJK2DVI, LATEX2DVI): Add `texlive' subdirectory
	(distsrc): Build .c from .w files.

2006-08-28  Werner LEMBERG  <wl@gnu.org>

	* texinput/*: Add various replacement files for TeXLive.

2006-08-17  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.txt: Mention problem with fourier.sty.

2006-08-01  Werner LEMBERG  <wl@gnu.org>

	* doc/cjk-enc.txt: Mention problems with UTF-8.

2006-07-30  Werner LEMBERG  <wl@gnu.org>

	* contrib/wadalab/DNP.txt: Fix patch for wftodm.c.

2006-04-25  Danai SAE-HAN  <danai.sae-han@skynet.be>

	* <many files>: Add GPL.
	* MANIFEST: New file.

2006-03-25  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKutf8.sty (\pdfstringdefPreHook): Don't overwrite but
	prepend to this macro.

2006-03-23  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/hlatex2agl.pl: New script (which has been used
	to create the Korean fonts in TeXLive 2005).


	* texinput/CJKutf8.sty: Add support for Unicode bookmarks.
	(\CJK@UnicodeFourBytesFirst, \CJK@UnicodeFourBytesSecond,
	\CJK@UnicodeFourBytesThird, \CJK@UnicodeThreeBytesFirst,
	\CJK@UnicodeThreeBytesSecond, \CJK@UnicodeTwoBytesFirst,
	\CJK@UnicodeLast): New macros to convert UTF-8 into UTF-16BE.
	(\CJK@XXpdf, \CJK@XXXpdf, \CJK@XXXXpdf): Replacements for the
	\CJK@XX, \CJK@XXX, and \CJK@XXXX macros, respectively.
	(\pdfstringdefPreHook): Activate them.

2006-03-22  Werner LEMBERG  <wl@gnu.org>

	* texinput/KS/HLaTeX/c63sh.fd, texinput/KS/HLaTeX/c64sh.fd,
	texinput/KS/HLaTeX/c65sh.fd: Fix font declaration.  Bug reported by
	Danai SAE-HAN <danai.sae-han@skynet.be>.

2006-02-20  Werner LEMBERG  <wl@gnu.org>

	* texinput/UTF8/UTF8.bdg: Bugfix: Handle 0x80 also.

	* doc/history.txt: Mention it.

2006-02-09  Werner LEMBERG  <wl@gnu.org>

	Support complete Unicode range (up to U+10FFFF).

	* texinput/UTF8/UTF8.bdg: Handle leading characters 0xF0-0xF4.

	* texinput/UTF8/UTF8.enc: Ditto.

	* texinput/UTF8/UTF8.chr (\CJK@altxchar): New macro for four-byte
	Unicode values.

	* texinput/CJK.enc (\CJK@unicodexError): New error macro.

	* texinput/CJK.sty (\CJK@numbxToHex): New auxiliary macro to convert
	a number to a four-digit hex number string.
	(\Unicode): Accept values greater than U+FFFF.

	* doc/command.txt, doc/CJK.txt: Document extended \Unicode (and
	\CJKchar) command.
	* doc/history.txt: Updated.

2006-01-23  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.enc (\CJK@HK@enc): Load `HK' encoding, not `Bg5'.
	Use \def, not \@namedef.

	* doc/CJK.txt: Mention `HKtext' environment.

2006-01-22  Werner LEMBERG  <wl@gnu.org>

	Add new encoding `HK' (C05) for Hong Kong's HKSCS-2004.

	* texinput/Bg5/HK.enc, texinput/Bg5/c05song.fd: New files.
	* texinput/CJK.enc: Add support for `HK' (C05).
	* texinput/CJKnumb.sty: Handle `HK'.

	* doc/CJK.txt: Bg5+ *cannot* be used for HKSCS.  Fix this.
	* doc/history.txt: Document `HK' encoding.

2006-01-19  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.txt: Mention usage of Bg5+ for HKSCS-2001/HKSCS-2004.

2006-01-04  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty (\PYding): New \let.
	(\PYactivate, \PYdeacticate): Handle \ding (from pifont.sty).

	* doc/pinyin.tex: Document possible problems with pifont.sty.

	* doc/history.txt: Updated.

2005-12-27  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/cfg/csso12.cfg: Fix typo.

2005-10-31  Danai SAE-HAN  <danai.sae-han@skynet.be>

	* utils/subfonts/makefdx.pl: Provide header for output.
	Add \CJKvlet lines.

2005-08-19  Werner LEMBERG  <wl@gnu.org>

	* doc/TeXLive.txt: New file, describing the relationship between
	CJK files and TeXLive packages.

2005-08-18  Werner LEMBERG  <wl@gnu.org>

	* texinput/mule/MULEenc.sty: Define \CJK@verbatim correctly if not
	already defined.  Reported by Andre Dierker.

	* doc/pdf/*: Move to...
	* doc/pdfhowto/*: This.

2005-08-11  Werner LEMBERG  <wl@gnu.org>

	Version 4.6.0 released
	======================

	Set version to 4.6.0.

	* doc/history.txt, doc/INSTALL, Makefile (version): Updated.

	Update headers in all text files.

2005-08-10  Werner LEMBERG  <wl@gnu.org>

	* doc/CEF.txt, doc/CJK.txt, doc/CJKutf8.txt, doc/INSTALL,
	doc/TDS.txt, doc/cjk-enc.txt, doc/commands.txt, doc/dvidrv.txt,
	doc/fonts.txt, doc/hbf2gf.txt, doc/history.2_5, doc/history.txt,
	doc/pinyin.txt, doc/pyhyphen.txt, doc/ruby.txt, doc/thaifont.txt,
	doc/vertical.txt: Updated and revised.

2005-08-05  Werner LEMBERG  <wl@gnu.org>

	* COPYING: Updated to new FSF address.

2005-08-05  Werner LEMBERG  <wl@gnu.org>

	After email exchange with Ross Paterson, the old (too restrictive)
	license of the hbf module has been changed to the three-clause BSD
	license -- Ross no longer maintains and distributes this code.

	* utils/hbf2gf/hbf.c: Change license to BSD.
	(strdup) [WIN32]: Define.  Change taken from teTeX distribution.

	* utils/hbf2gf/hbf.h: Change license to BSD.

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub: Updated to
	current versions.

	* utils/hbf2gf/configure: Regenerated with autoconf 2.59b.

2005-08-04  Werner LEMBERG  <wl@gnu.org>

	Update files to compile with the forthcoming TeXLive 2005.

	* doc/README: Updated, extended.

	* examples/muletest.tex: Updated to new VnTeX (for Vietnamese).
	Use type1ec.sty.
	Suppress hyphenation.

	* examples/CJKbabel.tex: Don't use t5.sty but `vietnam' option of
	babel.
	Use type1ec.sty.

	* examples/CJKmixed.tex: Define and use `TChinese' environment.
	Call \CJKhorz at the beginning of document.

	* examples/CJKutf8.tex: Don't use cyberbit but the new Unicode
	(virtual) fonts of gbsn, bsmi, and mj.

	* texinput/Bg5/c00bsmi.fdx: Updated to new bsmi vertical glyph font.

	* texinput/Bg5/c00bkai.fdx: New file.

	* texinput/UTF8/c70bkai.fd, texinput/UTF8/c70bkai.fdx,
	texinput/UTF8/c70bsmi.fd, texinput/UTF8/c70bsmi.fdx,
	texinput/UTF8/c60gbsn.fd, texinput/UTF8/c70gkai.fd,
	texinput/UTF8/c70mj.fd: New files.

	* utils/pyhyphen/pytest.tex: Usae type1ec.sty.

	* Makefile: Add rules for new example and documentation files.
	(version): Set top 4.5.3.
	(CJK2DVI, LATEX2DVI): Add `utils/pyhyphen' to TEXINPUTS variable.
	(DVI2PS): Replace it with...
	(DVI2PDF): New variable.
	Update all callers.
	(MULE): Add path to `cjk-enc.el' while calling emacs.
	(DISTTARGETS): Add new example and documentation files.
	(predistdoc): Don't create `ps' but `pdf' subdirectories.
	(manpages): Add `-ww' option to groff.
	Don't create `ps' but `pdf' files.
	(cweb): Don't create `ps' but `pdf' file.

2005-08-04  Werner LEMBERG  <wl@gnu.org>

	* doc/*.doc, doc/japanese/*.doc, doc/chinese/*.doc,
	contrib/wadalab/DNP.doc: Renamed to ...
	* doc/*.txt, doc/japanese/*.txt, doc/chinese/*.txt,
	contrib/wadalab/DNP.txt: This.

	Update all references.

2005-08-03  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKvert.sty (\CJKvert, \CJKhorz): Make commands act
	completely local.
	* doc/history.txt: Mention it.

	* doc/pdf/HOWTO.txt: Mention new $SFDFONTS variable from TDS 1.1.

2005-08-02  Werner LEMBERG  <wl@gnu.org>

	Update of HLaTeX support to version 1.0.1.

	* texinput/KS/HLaTeX/c63mg.fd, texinput/KS/HLaTeX/c63mgt.fd,
	texinput/KS/HLaTeX/c63mmj.fd, texinput/KS/HLaTeX/c63mnv.fd,
	texinput/KS/HLaTeX/c63msr.fd, texinput/KS/HLaTeX/c63ol.fd,
	texinput/KS/HLaTeX/c63pbm.fd, texinput/KS/HLaTeX/c63pgr.fd,
	texinput/KS/HLaTeX/c63pgs.fd, texinput/KS/HLaTeX/c63pgt.fd,
	texinput/KS/HLaTeX/c63pmg.fd, texinput/KS/HLaTeX/c63pmgt.fd,
	texinput/KS/HLaTeX/c63pmj.fd, texinput/KS/HLaTeX/c63pmmj.fd,
	texinput/KS/HLaTeX/c63pmnv.fd, texinput/KS/HLaTeX/c63pmsr.fd,
	texinput/KS/HLaTeX/c63pol.fd, texinput/KS/HLaTeX/c63ppg.fd,
	texinput/KS/HLaTeX/c63ppn.fd, texinput/KS/HLaTeX/c63psm.fd,
	texinput/KS/HLaTeX/c63ptt.fd, texinput/KS/HLaTeX/c63pyt.fd,
	texinput/KS/HLaTeX/c63sm.fd, texinput/KS/HLaTeX/c63tt.fd,
	texinput/KS/HLaTeX/c64mg.fd, texinput/KS/HLaTeX/c64mgt.fd,
	texinput/KS/HLaTeX/c64mmj.fd, texinput/KS/HLaTeX/c64mnv.fd,
	texinput/KS/HLaTeX/c64msr.fd, texinput/KS/HLaTeX/c64ol.fd,
	texinput/KS/HLaTeX/c64pbm.fd, texinput/KS/HLaTeX/c64pgr.fd,
	texinput/KS/HLaTeX/c64pgs.fd, texinput/KS/HLaTeX/c64pgt.fd,
	texinput/KS/HLaTeX/c64pmg.fd, texinput/KS/HLaTeX/c64pmgt.fd,
	texinput/KS/HLaTeX/c64pmj.fd, texinput/KS/HLaTeX/c64pmmj.fd,
	texinput/KS/HLaTeX/c64pmnv.fd, texinput/KS/HLaTeX/c64pmsr.fd,
	texinput/KS/HLaTeX/c64pol.fd, texinput/KS/HLaTeX/c64ppg.fd,
	texinput/KS/HLaTeX/c64ppn.fd, texinput/KS/HLaTeX/c64psm.fd,
	texinput/KS/HLaTeX/c64ptt.fd, texinput/KS/HLaTeX/c64pyt.fd,
	texinput/KS/HLaTeX/c64sm.fd, texinput/KS/HLaTeX/c64tt.fd,
	texinput/KS/HLaTeX/c65mg.fd, texinput/KS/HLaTeX/c65mgt.fd,
	texinput/KS/HLaTeX/c65mmj.fd, texinput/KS/HLaTeX/c65mnv.fd,
	texinput/KS/HLaTeX/c65msr.fd, texinput/KS/HLaTeX/c65ol.fd,
	texinput/KS/HLaTeX/c65pbm.fd, texinput/KS/HLaTeX/c65pgr.fd,
	texinput/KS/HLaTeX/c65pgs.fd, texinput/KS/HLaTeX/c65pgt.fd,
	texinput/KS/HLaTeX/c65pmg.fd, texinput/KS/HLaTeX/c65pmgt.fd,
	texinput/KS/HLaTeX/c65pmj.fd, texinput/KS/HLaTeX/c65pmmj.fd,
	texinput/KS/HLaTeX/c65pmnv.fd, texinput/KS/HLaTeX/c65pmsr.fd,
	texinput/KS/HLaTeX/c65pol.fd, texinput/KS/HLaTeX/c65ppg.fd,
	texinput/KS/HLaTeX/c65ppn.fd, texinput/KS/HLaTeX/c65psm.fd,
	texinput/KS/HLaTeX/c65ptt.fd, texinput/KS/HLaTeX/c65pyt.fd,
	texinput/KS/HLaTeX/c65sm.fd, texinput/KS/HLaTeX/c65tt.fd: Removed.

	* texinput/KS/HLaTeX/c63dn.fd, texinput/KS/HLaTeX/c63jgt.fd,
	texinput/KS/HLaTeX/c63jmj.fd, texinput/KS/HLaTeX/c63jnv.fd,
	texinput/KS/HLaTeX/c63jsr.fd, texinput/KS/HLaTeX/c63pga.fd,
	texinput/KS/HLaTeX/c63ph.fd, texinput/KS/HLaTeX/c63sh.fd,
	texinput/KS/HLaTeX/c63tz.fd, texinput/KS/HLaTeX/c63vd.fd,
	texinput/KS/HLaTeX/c64dn.fd, texinput/KS/HLaTeX/c64jgt.fd,
	texinput/KS/HLaTeX/c64jmj.fd, texinput/KS/HLaTeX/c64jnv.fd,
	texinput/KS/HLaTeX/c64jsr.fd, texinput/KS/HLaTeX/c64pga.fd,
	texinput/KS/HLaTeX/c64ph.fd, texinput/KS/HLaTeX/c64sh.fd,
	texinput/KS/HLaTeX/c64tz.fd, texinput/KS/HLaTeX/c64vd.fd,
	texinput/KS/HLaTeX/c65dn.fd, texinput/KS/HLaTeX/c65jgt.fd,
	texinput/KS/HLaTeX/c65jmj.fd, texinput/KS/HLaTeX/c65jnv.fd,
	texinput/KS/HLaTeX/c65jsr.fd, texinput/KS/HLaTeX/c65pga.fd,
	texinput/KS/HLaTeX/c65ph.fd, texinput/KS/HLaTeX/c65sh.fd,
	texinput/KS/HLaTeX/c65tz.fd, texinput/KS/HLaTeX/c65vd.fd: New files.

	* texinput/KS/HLaTeX/c63bm.fd, texinput/KS/HLaTeX/c63gr.fd,
	texinput/KS/HLaTeX/c63gs.fd, texinput/KS/HLaTeX/c63gt.fd,
	texinput/KS/HLaTeX/c63mj.fd, texinput/KS/HLaTeX/c63pg.fd,
	texinput/KS/HLaTeX/c63pn.fd, texinput/KS/HLaTeX/c63yt.fd,
	texinput/KS/HLaTeX/c64bm.fd, texinput/KS/HLaTeX/c64gr.fd,
	texinput/KS/HLaTeX/c64gs.fd, texinput/KS/HLaTeX/c64gt.fd,
	texinput/KS/HLaTeX/c64mj.fd, texinput/KS/HLaTeX/c64pg.fd,
	texinput/KS/HLaTeX/c64pn.fd, texinput/KS/HLaTeX/c64yt.fd,
	texinput/KS/HLaTeX/c65bm.fd, texinput/KS/HLaTeX/c65gr.fd,
	texinput/KS/HLaTeX/c65gs.fd, texinput/KS/HLaTeX/c65gt.fd,
	texinput/KS/HLaTeX/c65mj.fd, texinput/KS/HLaTeX/c65pg.fd,
	texinput/KS/HLaTeX/c65pn.fd, texinput/KS/HLaTeX/c65yt.fd: Updated.

	* texinput/KS/HLaTeX/pshan.sty: No longer needed.  Make it empty for
	backwards compatibility.

	* texinput/CJK.enc (\CJK@KSHL@enc): Updated.

	* doc/history.txt, doc/CJK.doc: Updated.

2005-08-01  Werner LEMBERG  <wl@gnu.org>

	* utils/subfont/uni2sfd.pl (read_tfmfile): Fix reading CHARWD,
	CHARHT, and CHARDP.

2005-07-31  Werner LEMBERG  <wl@gnu.org>

	* utils/subfont/sfd2uni.pl: New script to produce Unicode virtual
	subfonts from encoding specific subfonts.

2005-07-29  Werner LEMBERG  <wl@gnu.org>

	* contrib/wadalab/DNP.sfd: Fix typo.  Found by Shunsaku Hirata.
	* contrib/wadalab/fixwada2.pl: Since Wadalab fonts have already
	been uploaded to CTAN, and the bug in DNP.sfd makes it necessary to
	regenerate the fonts, and to update the version number and creation
	date.

2005-07-18  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/makefdx.pl, utils/subfonts/uni2sfd.pl: Fix typos.

	* utils/subfonts/clonevf.pl: New script to produce a VF clone of
	a TFM file.

2005-07-18  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/makefdx.pl: New script to create FDX entries.

2005-07-17  Werner LEMBERG  <wl@gnu.org>

	* utils/subfonts/subfonts.pe, utils/subfonts/uni2sfd.pl,
	utils/subfonts/vertical.pe, utils/vertref.pe: New perl and FontForge
	scripts for creating and handling subfonts.

2005-07-12  Werner LEMBERG  <wl@gnu.org>

	* contrib/wadalab/fixwada2.pl, contrib/wadalab/makeuniwada.pl: New
	scripts which fix glyph names and create virtual Unicode fonts for
	the Wadalab font families.

	* contrib/wadalab/DNP.sfd: A subfont definition file used by
	`fixwada2.pl' and `makeuniwada.pl'.

	* contrib/wadalab/c70goth.fd, contrib/wadalab/c70maru.fd,
	contrib/wadalab/c70min.fd: New font definition files for Wadalab
	fonts in Unicode encoding.

	* contrib/wadalab/DNP.doc: Completely revised and updated.

2005-07-07  Werner LEMBERG  <wl@gnu.org>

	* doc/history.txt: Updated.

2005-07-05  Werner LEMBERG  <wl@gnu.org>

	* utils/thaifont/tools/c90.etx: Fix some typos.

2005-07-04  Werner LEMBERG  <wl@gnu.org>

	Update Thai support:

	. Use fontinst.  We no longer need virtual fonts.
	. Replace support for dbtt (which has an uncertain license) with
	  garuda.
	. Update to TDS 1.1.

	* utils/thaifont/texmf/dvips/base/dbtt.enc: Removed.
	* utils/thaifont/texmf/dvips/config/config.dbtt: Removed.
	* utils/thaifont/texmf/dvips/config/dbtt.map: Removed.
	* utils/thaifont/texmf/fonts/tfm/public/dbtt/*: Removed.
	* utils/thaifont/texmf/fonts/vf/public/dbtt/*: Removed.

	* utils/thaifont/texmf/dvips/base/norasi.enc: Removed.
	* utils/thaifont/texmf/dvips/config/config.norasi: Move to...
	* utils/thaifont/texmf/dvips/norasi/config.norasi: Here.
	* utils/thaifont/texmf/dvips/config/norasi.map: Moved to...
	* utils/thai/font/texmf/fonts/map/dvips/norasi/norasi.map: Here.
	Updated.
	* utils/thaifont/texmf/fonts/tfm/public/norasi/ftnr9z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnb9z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnbo9z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftno9z.tfm: Removed.
	* utils/thaifont/texmf/fonts/tfm/public/norasi/ftnr8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnb8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftnbo8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/norasi/ftno8z.tfm: Updated.
	* utils/thaifont/texmf/fonts/vf/public/norasi/*: Removed.

	* utils/thaifont/texmf/dvips/garuda/config.garuda: New file.
	* utils/thaifont/texmf/fonts/map/dvips/garuda/garuda.map: New file.
	* utils/thaifont/texmf/fonts/tfm/public/garuda/fgdr8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdb8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdbo8z.tfm,
	utils/thaifont/texmf/fonts/tfm/public/garuda/fgdo8z.tfm: New files.

	* utils/thaifont/texmf/fonts/enc/dvips/thai/c90.enc: New file,
	generated by fontinst.

	* utils/thaifont/tools/c90.etx: New file.
	* utils/thaifont/tools/c90.mtx: New file.
	* utils/thaifont/tools/garuda.fontinst: New file.
	* utils/thaifont/tools/norasi.fontinst: New file.
	* utils/thaifont/tools/INSTALL: New file.
	* utils/thaifont/tools/dbtt-old/*: New files.
	* utils/thaifont/tools/README: Removed.
	* utils/thaifont/tools/thai-dummy.afm: Removed.
	* utils/thaifont/tools/thai.enc: Removed.
	* utils/thaifont/tools/thailigs.vpl: Removed.

	* texinput/thai/c90cmss.fd, texinput/thai/c90cmtt.fd,
	texinput/thai/c90nrsr.fd: Updated.
	* texinput/thai/c90dbss.fd: Removed.
	* texinput/thai/c90gar.fd: New file.

2005-06-27  Werner LEMBERG  <wl@gnu.org>

	Remove the `rotate' keyword for vertical typesetting and introduce
	the opposite, `norotate'.

	* texinput/Bg5/c00bsmir.fdx, texinput/Bg5/c00kair.fdx: New files.

	* doc/fdxfiles.doc, doc/vertical.doc, texinput/Bg5/c00bsmi.fdx,
	texinput/GB/c10gbsn.fdx, texinput/CJKvert.sty: Updated.

2005-06-25  Werner LEMBERG  <wl@gnu.org>

	* examples/CJKmixed.tex: New example file to demonstrate how to
	use CJK scripts vertically and horizontally at the same time.

2005-06-24  Werner LEMBERG  <wl@gnu.org>

	* doc/vertical.doc: Mention that you need an `.fdx' file if you
	want to use rotated glyphs for vertical typesetting.

2005-05-23  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.doc: Improve documentation of `encapsulated' option.
	Suggested by Brian Murphy.

2005-04-26  Werner LEMBERG  <wl@gnu.org>

	* texinput/UTF8/UTF8.chr (\CJK@punctchar): Wrap code after \usefont
	into three groups to make it work with CJKulem.sty.

	* texinput/CJKutf8.sty, examples/CJKutf8.tex, doc/CJKutf8.doc: New
	files.

	* doc/history.txt: Updated.

2005-04-22  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/emacs/cjk-enc.el (cjk-viscii-lower, cjk-viscii-upper),
	utils/lisp/mule-2.3/cjk-enc.el (cjk-viscii-lower, cjk-viscii-upper):
	Update to next vntex version which no longer uses dblaccnt.sty.

2005-03-27  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\CJKspace): Don't use \relax but \@empty.

2005-03-02  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.doc: Mention `CJKbookmarks' option of hyperref package.

2005-02-23  Werner LEMBERG  <wl@gnu.org>

	* README: Updated.  No public CVS access possible currently.

2004-07-26  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/emacs/thai-word.el (thai-word-table): Use Thai word
	list from IBM's ICU4J project; it is slightly larger and uses an
	X license.

2004-07-25  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/emacs-20.3/*: Moved to...
	* utils/lisp/emacs/*: This.

	* utils/thaifont/tools/thai.enc: Minor updates.  Will be replaced
	with a fontinst solution soon.

2004-06-08  Werner LEMBERG  <wl@gnu.org>

	* doc/reftex.doc: New file.
	* doc/history.txt: Updated.

2004-06-07  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/emacs-20.3/cjk-enc.el (cjk-write-all-files): Handle
	case where files are in other directories.  Bug reported by Hartwig
	Crailsheim.

	* doc/cjk-enc.doc, doc/history.txt: Updated.

2004-06-04  Werner LEMBERG  <wl@gnu.org>

	* contrib/wadalab/c42goth.fdx, contrib/wadalab/c42maru.fdx,
	contrib/wadalab/c42min.fdx: Don't rotate the Hiragana-Katagana
	prolongation mark.

	* doc/vertical.doc: Updated.
	Move text describing .fdx files to...
	* doc/fdxfiles.doc: New file.

	* texinput/CJK.sty: Minor spelling improvements.

2004-06-03  Werner LEMBERG  <wl@gnu.org>

	* contrib/wadalab/DNP.doc: Improve patch for wftodm.c.

2004-04-29  Werner LEMBERG  <wl@gnu.org
	    Wenchang Sun  <sunwch@hotmail.com>

	Add a style file for various CJK font effects.

	* texinput/CJKfntef.sty, examples/CJKfntef.tex: New files.
	* doc/CJK.doc, doc/history.txt: Document it.

2004-03-13  Werner LEMBERG  <wl@gnu.org>

	* texinput/*.enc: Replace \relax with \@empty in the \CJK@namegdef
	assignments to assure that we only have expansion at this macro
	level.

	* doc/history.txt: Updated.

2004-02-08  Werner LEMBERG  <wl@gnu.org>

	Bug fix: Umlaut u with diacritic appears bold.

	* texinput/pinyin.sty (\py@@@v): Apply kerning at correct place.

2004-02-07  Werner LEMBERG  <wl@gnu.org>

	Bug fix: Umlaut u with macron above was broken.

	* texinput/pinyin.sty (\py@macron): Add second argument to
	initialize \dimen@.  Update all callers.

2004-02-06  Werner LEMBERG  <wl@gnu.org>

	Bug fix: Use user-defined \CJKglue value.

	* texinput/CJKulem.sty (\CJK@skip): New skip register.
	(\UL@CJKglue): Use it.
	(\UL@hook): Initialize \CJK@skip.
	Move assignments of \LA@CJKglue, \LA@Thaiglue, and \LA@Thaibreak
	to here.

2004-02-05  Wenchang Sun  <sunwch@hotmail.com>

	Bug fix: Disable line breaks before a post-punctuation CJK glyph
	when \uline, \uwave, etc., are used.

	* texinput/CJK.sty (\CJKnobreakglue): New macro.
	(\Unicode): Use it.

	* texinput/CJKulem.sty (\UL@CJKnobreakglue): New macro.

	* texinput/standard.chr, texinput/extended.chr, texinput/pmC.chr,
	texinput/Bg5/bg5.chr, texinput/JIS/EUC-JP.chr,
	texinput/SJIS/SJIS.chr, texinput/SJIS/SJISdnp.chr,
	texinput/UTF8/UTF8.chr, texinput/CNS/EUC-TW.chr (\CJK@char,
	\CJK@charx, \CJK@punctchar, \CJK@punctcharx): Use \CJKnobreakglue.

2004-02-02  Hin-Tak Leung  <htl10@users.sourceforge.net>

	* doc/pdf/*: New directory tree documenting usage of CJK for
	improved PDF output.
	* doc/history.txt: Document it.

2004-01-29  Wenchang Sun  <sunwch@hotmail.com>

	* texinput/CJK.sty (\CJKpunctsymbol): New \let to \CJKsymbol.

	* texinput/standard.chr, texinput/extended.chr, texinput/pmC.chr,
	texinput/Bg5/bg5.chr, texinput/JIS/EUC-JP.chr, texinput/KS/KS.chr,
	texinput/SJIS/SJIS.chr, texinput/SJIS/SJISdnp.chr,
	texinput/UTF8/UTF8.chr, texinput/CNS/EUC-TW.chr (\CJK@punctchar,
	\CJK@punctcharx): Replace \CJKsymbol with \CJKpunctsymbol.

2003-10-12  Werner LEMBERG  <wl@gnu.org>

	A first step to allow modification of horizontal character widths
	which is needed for CJK fonts which don't have punctuation glyphs
	centered within the CJK square.  The same mechanism will work with
	vertical glyphs also; since a common interface will differ from the
	current implementation, *.fdv files are renamed to *.fdx.  Note that
	special character width handling of punctuation characters is still
	missing.

	* texinput/CJK.sty (\CJK@load@fdx): New function, used as a hook
	for \try@load@fontshape.  It defines the macros \CJKhdef, \CJKhlet,
	\CJKvdef, and \CJKvlet.  The writing direction is appended to the
	character macros -- this also fixes a bug for vertical writing
	support with Big5 encoding (some characters disappeared in the
	output without any warning due to character macro name clashes with
	the subfont macro names).
	(\CJK@direction): New macro to select the writing direction.
	(\ifCJK@vertical@): Moved to CJKvert.sty.

	* texinput/CJKvert.sty (\ifCJK@vertical@): Moved from CJK.sty.
	(\CJKvert, \CJKhorz): Set \CJK@direction.
	(\CJKsymbol): Updated to use writing direction.
	(\CJK@load@fdv): Removed.

	* texinput/*.chr: Simplified since \ifCJK@vertical@ is no longer
	needed.

	* texinput/*.fdv, contrib/wadalab/*.fdv: Renamed to...
	* texinput/*.fdx, contrib/wadalab/*.fdx: This.

2003-10-25  Werner LEMBERG  <wl@gnu.org>

	* texinput/mule/MULEenc.sty: Fix positions of \texordfeminine and
	\textordmasculine.

2003-09-20  Werner LEMBERG  <wl@gnu.org>

	With the help of Paul Eggert <eggert@twinsum.com> and Edward G.J.
	Lee <edt1023@ms17.hinet.net>, the conversion scripts now accept
	parameters.

	* utils/Bg5conv/bg5{pdf,}latex,
	utils/CEFconv/{cef5{pdf,}latex,cef{pdf,}latex,cefs{pdf,}latex},
	utils/SJISconv/sjis{pdf,}latex,
	utils/extconv/{bg5+{pdf,}latex,gbk{pdf,}latex}: Rewritten to accept
	arguments.
	* doc/history.txt: Updated.

2003-09-16  Werner LEMBERG  <wl@gnu.org>

	* utils/Bg5conv/bg5pdflatex,
	utils/CEFconv/{cef5pdflatex,cefpdflatex,cefspdflatex},
	utils/SJISconv/sjispdflatex,
	utils/extconv/{bg5+pdflatex,gbkpdflatex}: New scripts to call
	pdflatex.
	* doc/history.txt: Updated.

2003-07-06  Werner LEMBERG  <wl@gnu.org>

	* texinput/mule/MULEenc.sty: Add some \@gobble macros in commands
	defined with \mule@def.
	Change definition of Thai EOL macro to make it really work.
	(\mule@ignorespaces, \Thaispace, \Thainospace): New macros.

	* doc/cjk-enc.doc, doc/history.txt: Document \Thaispace and
	\Thainospace.

2003-03-30  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.doc: Add item how to handle \bibliography which has
	author names containing CJK characters.

	* utils/hbf2gf/hbf2gf.1: Minor workarounds for current grohtml bugs.

2003-03-28  Werner LEMBERG  <wl@gnu.org>

	Version 4.5.2 released
	======================

	Update version numbers and time stamps in all non-binary files.

2003-03-19  Werner LEMBERG  <wl@gnu.org>

	Add improved support for pseudo-vertical typesetting.  Based on
	ideas by Robert Fendt <robert.fendt@epost.de>.

	* texinput/CJK.sty (\ifCJK@vertical@): New if.

	* texinput/CJKvert.sty: Require `graphicx' package.
	(\CJKvert, \CJKhorz, \CJKvdef, \CJKvlet, \CJKsymbolsimple): New
	commands.
	(\CJKsymbol): Add support for vertical parameters (`rotate',
	`offset', `fullheight, `height') in the new *.fdv files.
	(\CJK@load@fdv): New command to be appended to LaTeX's
	\try@load@fontshape.

	* texinput/*/*.chr: Replace calls to \CJKsymbol with an extended
	version which, if \CJKvert is active, checks the existence of a
	macro

	  \<encoding>/<family>/<series>/<shape>/<plane>/<code>

	This macro is then called if it exists, instead of calling
	\CJKsymbol.  For halfwidth katakana, the macro is called

	  \<encoding>/<family>/<series>/<shape>/<code>

	For HLaTeX, the macro is called

	  \<encoding>/<family>/<series>/<shape>/<first byte>/<second byte>

	For UTF8, only characters in the range 0x800-0xFFFF get the new
	code.

	<code>, <first byte>, and <second byte> are decimal numbers.

	* contrib/wadalab/c42{goth,maru,min}.fdv,
	contrib/wadalab/c52{maru,min}.fdv, texinput/Bg5/c00bsmi.fdv,
	texinput/GB/c10gbsn.fdv: New files containing information for
	vertical typesetting.

	* examples/Big5vert.tex: Use font shape `bsmi'.

	* doc/history.txt, doc/chinese/README, contrib/wadalab/DNP.doc,
	doc/vertical.doc, examples/README, README: Updated.

	* Makefile (DVI2PS): Load bsmilp.map and gbsnlp.map.
	(cweb): Fix typo (cms->cmz).

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub: Updated to
	current versions.

	* utils/extconv/extconv.w: Remove duplicated lines.
	Fix incorrect use of \@.
	* utils/extconv/extconv.c: Regenerated.

2003-03-18  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty (\rua): New syllable.  While only dialect, it
	actually is used...

2003-03-12  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty (\den, \chua): Add missing syllables (found by
	Jean-Luc Koning <Jean-Luc.Koning@esisar.inpg.fr>).

2003-03-07  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty (\py@hy): Assure horizontal mode.

2003-02-10  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\CJKchar): Make \CJKchar accept 7bit input for
	character definitions other than standard.chr.
	* doc/history.txt: Updated.

2003-02-06  Werner LEMBERG  <wl@gnu.org>

	Horizontal hints in Wadalab fonts weren't shifted vertically,
	causing inferior results at small sizes.

	* contrib/wadalab/makefont: Rewritten using awk.
	* contrib/wadalab/fixwada: New.
	* contrib/wadalab/DNP.doc, doc/history.txt: Updated.
	* doc/INSTALL: Minor fixes.  Mention wadalab.doc and pfaedit.

2003-01-31  Werner LEMBERG  <wl@gnu.org>

	Add two commands \CJKhwkatakana and \CJKnohwkatakana to control
	whether C49 encoding is used or whether SJIS half-width katakana are
	mapped to full-width glyphs instead.

	* texinput/CJK.sty (\CJKhwkatakana, \CJK@nohwkatakana): New commands.
	(\ifCJK@hwkatakana@): New if-macro.

	* texinput/SJIS/SJIS.chr, texinput/SJIS/SJISdnp.chr (\CJK@sjischar):
	Add second and third parameter to call \CJK@XXX conditionally.
	* texinput/SJIS/SJIS.enc (\CJK@SJISEncoding): Fill second and
	third parameters for half-width katakana.
	* texinput/SJIS/SJISdnp.enc (\CJK@SJISdnpEncoding): Ditto.
	* doc/commands.doc, doc/CJK.doc, doc/history.txt: Updated.

	* examples/README: New file.

2002-07-29  Werner LEMBERG  <wl@gnu.org>

	* texinput/CNS/EUC-TW.chr (\CJK@shiftchar): Pass correct parameters
	to \CJKchar.

2002-06-19  Werner LEMBERG  <wl@gnu.org>

	Version 4.5.1 released
	======================

	Update version numbers and time stamps in all non-binary files.

2002-06-17  Werner LEMBERG  <wl@gnu.org>

	Preparation of release 4.5.1.

	* README: Updated.
	* texinput/CJK.sty, doc/CJK.doc: Require LaTeX 2001/06/01 to have
	support for \textkra, \texttstroke, and \textTstroke.
	Other minor documentation updates.
	* doc/*: Updated.

2002-06-16  Werner LEMBERG  <wl@gnu.org>

	* doc/chinese/READMEgb.tex: Use `gbsn' font.
	* Makefile (CJK2DVI): Remove *.toc also.
	(LATEX2DVI): Take two arguments.
	(LATEX): Ditto.
	(DISTTARGETS): Add READMEb5 and pytest.
	(READMEgb, pytest): New rules
	(GB...): Updated.
	(predistdoc): Create README file.
	(distdoc): Depend also on `cweb'.
	(cweb): New target.

2002-06-14  Edward Lee  <edt1023@ms17.hinet.net>

	* texinput/Bg5/c00bsmi.fd, texinput/Bg5/c00bsmir.fd: Fix typo.

2002-06-13  Werner LEMBERG  <wl@gnu.org>

	* Makefile: New file, used for creating the tarballs.
	* README: Updated.
	* texinput/GB/c10gbsn.fd, texinput/Bg5/c00bsmi.fd,
	texinput/Bg5/c00bsmir.fd: New files for fonts from the TeXLive CD.
	* doc/chinese/READMEb5.tex, examples/*: Changed to use the fonts
	provided by the TeXLive CD.

2002-06-12  Werner LEMBERG  <wl@gnu.org>

	* texinput/JISdnp.enc (\CJK@JISdnpEncoding): Fix position of closing
	brace.

2002-06-07  Werner LEMBERG  <wl@gnu.org>

	* texinput/thai/c90enc.def: New file, contributed by Dominique
	Unruh <dominique@unruh.de>.
	* texinput/thai/thaicjk.ldf: Use it.
	* doc/history.txt: Updated.

2002-05-16  Werner LEMBERG  <wl@gnu.org>

	* doc/cjk-enc.doc: Document behaviour for master files without CJK
	characters.
	* doc/CJK.doc: Explain usage of `~' for BibTeX.

2002-05-10  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKnumb.sty (\CJKnullspace): New macro to control the
	additional space inserted before and after a circle used as a
	CJK zero digit.
	* doc/history.txt: Updated.

2002-05-09  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKnumb.sty (\CJK@traditionalNumbers,
	\CJK@simplifiedNumbers): New macros.
	Use them for GB, GBK, Bg5, Bg5+ hooks.

2002-05-01  Werner LEMBERG  <wl@gnu.org>

	* doc/commands.doc: Minor fix.

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub: Updated to
	current versions.
	* utils/hbf2gf/configure.in: Renamed to...
	* utils/hbf2gf/configure.ac: This.
	Updated to autoconf 2.53.
	* utils/hbf2gf/configure: Regenerated with autoconf 2.53.
	* utils/hbf2gf/README: Text improved.
	* utils/hbf2gf/hbf2gf.1: Minor typographical fixes.

2002-04-30  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\CJK@errxx, \CJKindent): New macros.
	* texinput/CJK.enc (\CJK@spaceChar): Define it for all encodings.
	It is used by \CJKindent.
	(\CJK@KSHL@enc): Add \CJK@min and \CJK@max.
	* texinput/SJIS/SJISdnp.enc (\CJK@SJISdnpEncoding),
	texinput/JIS/JISdnp.enc (\CJK@JISdnpEncoding),
	texinput/KS/HLaTeX/KSHL.enc (\CJK@KSHLEncoding): Use \CJK@errxx
	for unused slots.

	* doc/history.txt, doc/commands.doc: Document \CJKindent.

	* utils/CEFconv/cef5conv.w, utils/CEFconv/cefconv.w: Fix
	documentation errors.
	* utils/CEFconv/cef5conv.c, utils/CEFconv/cefconv.c: Regenerated.

2002-04-29  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\pickup@font): Add comment character.

2002-04-28  Werner LEMBERG  <wl@gnu.org>

	Preparation of release 4.5.0.

	* README: Updated.

2002-04-27  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty (\CJKsymbol, \CJKsymbols): Simplified.
	(\Unicode, \CJKenc): Fix error text.

2001-10-08  Mike Fabian <mfabian@suse.de>

	* contrib/wadalab/c42goth.fd: Use `dgj' for normal series and add
	`\CJKbold' for bold series.

2001-07-31  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.doc: Note use of \cleardoublepage if problems occur with
	two-column printing.

2001-07-27  Fabrice Popineau  <Fabrice.Popineau@supelec.fr>

	* utils/cjklatex/cjklatex.c: New file.

2001-06-27  Werner LEMBERG  <wl@gnu.org>

	* doc/CJK.doc: Add info how to use a CJK environment in the
	preamble.
	* doc/cjk-enc.doc: Simplify usage of AUC TeX.
	Modify definition of `TeX-run-CJK-LaTeX' to handle directories
	properly.

2001-06-15  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.enc (\CJK@disableMakeUppercase): Define it as \relax
	if in preprocessed mode.

2001-06-14  HANDA Ken'ichi  <handa@etl.go.jp>

	* utils/lisp/emacs-20.3/cjk-enc.el (cjk-set-buffer-multibyte):
	Use backquote operator to make cjk-enc.elc work correctly.

2001-06-08  Werner LEMBERG  <wl@gnu.org>

	The next LaTeX release will use \textkra, \texttstroke, and
	\textTstroke for the missing latin-4 characters.

	* texinput/mule/MULEenc.sty: Use \textkra.  Add \TEXTTSTROKE.
	* utils/lisp/emacs-20.3/cjk-enc.el, utils/lisp/mule-2.3/cjk-enc.el:
	Use \texttstroke and \TEXTTSTROKE.

2001-05-26  Werner LEMBERG  <wl@gnu.org>

	* texinputs/CJK.sty: Restore EOL character before loading `CJK.cfg'.

2001-05-18  Werner LEMBERG  <wl@gnu.org>

	* contrib/wadalab/DNP.doc: Document installation for pdfTeX.
	* contrib/wadalab/makefont: Updated to normalize font matrix of
	PS fonts.

2001-04-24  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub: Updated to
	latest version from gnu.org.

2001-04-21  Werner LEMBERG  <wl@gnu.org>

	* examples/muletest.tex: Remove Thai support so that this file can
	really be run with Mule 2.3.
	Update comment.
	* example/CJKbabel.tex, example/rubytest.tex: Update comment.

	* utils/lisp/emacs-20.3/cjk-enc.el (cjk-format-spec-table): Fix
	Thai.
	* texinput/mule/MULEenc.sty (\mule@char): Don't use delimiter.
	* texinput/SJIS/sjisdnp.enc: Update this file also to the changes
	introduced 2001-03-15.

2001-04-17  Werner LEMBERG  <wl@gnu.org>

	* examples/*.tex: Added local variables for Emacs to specify
	encoding.
	* doc/history.txt: Emphasize the need of local variables for the
	encoding if `cjk-enc.el' is used.

2001-04-02  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/emacs-20.3/cjk-enc.el: Fix documentation to follow
	Elisp documentation conventions.

2001-04-01  Werner LEMBERG  <wl@gnu.org>

	Make UTF8 encoding work in TOC.

	* texinput/CJK.sty (\CJK@namedef): New macro.
	* texinput/UTF8/UTF8.bdg: Use it.

2001-03-28  Werner LEMBERG  <wl@gnu.org>

	* texinput/mule/MULEenc.sty: Use \textnumero instead of \CYRNo
	(found by Vladimir Volovich).

2001-03-18  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/cjkspace.el, INSTALL: Fix documentation.

2001-03-15  Werner LEMBERG  <wl@gnu.org>

	A major change: Preprocessed and non-preprocessed mode can be used
	simultaneously!  For example, you can now use include a file encoded
	in UTF-8 in another file encoded in Big5.

	To achieve this, ^^7f will always start a command in preprocessed
	mode, even for CJK macros.

	* texinput/CJK.sty: Require MULEenc.sty.
	Remove ^^7f handling.
	Remove preprocessed versions of \CJK@XX, \CJK@XXX, and \CJK@XXXX.
	(\CJKcaption): Always include .cpx files.

	* texinput/CJK.enc (\CJK@disableMakeUppercase): New macro.
	(\CJK@shiftError): New macro.
	(\CJK@unicodeError): New macro.
	(\CJK@makeEnvironment): Don't handle \MakeUppercase.
	(\CJK@*@enc): Always use `true' branch in \CJKpreproc conditionals.

	* texinput/mule/MULEenc.sty (\mule@@@arg, \mule@def): Use \string.
	(\mule@@def): New function to set up macros for leading bytes in the
	range ^^81-^^fe.
	* texinput/extended.enc (\CJK@extendedEncoding),
	texinput/Bg5/Bg5.enc (\CJK@Bg5Encoding), texinput/SJIS/SJIS.enc
	(\CJK@SJISEncoding): Use \CJK@disableMakeUppercase.
	* texinput/pmCbig.enc (\CJK@pmCbigEncoding), texinput/pmCsmall.enc
	(\CJK@pmCsmallEncoding), texinput/standard.enc
	(\CJK@standardEncoding): Add \relax.
	* texinput/CNS/EUC-TW.enc (\CJK@EUC-TWEncoding),
	texinput/JIS/EUC-JP.enc (\CJK@EUC-JPEncoding): Use \CJK@shiftError
	for single shifts.  Add	\relax for all other macros.
	* texinput/UTF8/UTF8.enc (\CJK@UTF8Encoding): Use \CJK@unicodeError
	for three-byte sequences.  Add \relax for all other macros.

	* texinput/*/*.cpx: Updated to new preprocessing scheme.

	* utils/*conv/*conv.w: Updated to new preprocessing scheme.
	* utils/*conv/*conv.c: Regenerated.

	* utils/lisp/emacs-20.3/cjk-enc.el (cjk-format-spec-table): Updated
	to new preprocessing scheme.
	(cjk-encode): Fix file header insertion strings.
	* utils/lisp/mule-2.3/cjk-enc.el (cjk-enc-table): Updated to new
	preprocessing scheme.
	(cjk-encode): Fix file header insertion strings.

	* doc/*: Updated and revised.

2001-03-13  Werner LEMBERG  <wl@gnu.org>

	Implement \CJKinput.

	* mule/MULEenc.sty (\CJKinput): New macro.
	(\CJKinclude): Fix error message.

	* utils/lisp/emacs-20.3/cjk-enc.el (cjk-write-all-files): Update
	docstring.
	(tex-input-regexp): New test for \CJKinput.
	(do-batch-cjk-write-file): Fix typo.

	* texinput/thai/thaicjk.ldf: Fix typo.

2001-02-21  Werner LEMBERG  <wl@gnu.org>

	* doc/INSTALL: Minor improvements.

2001-02-13  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/config.{guess,sub}: Updated (from ftp.gnu.org).

2000-12-17  Werner LEMBERG  <wl@gnu.org>

	* utils/SJISconv/sjisconv.w: Fix typo ff -> 7f.
	* utils/CEFconv/cef5conv.w, utils/CEFconv/cefconv.w: Ditto.

	* utils/*conv/*conv.w: \XXXpreproc will now contain the version of
	the conversion program.
	* utils/*conv/*conv.c: Updated.

	* doc/history.txt: Updated.

	* all files: Version number changed to 4.4.0.

2000-12-03  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/configure.in: Fix kpathsea checking message.
	* utils/hbf2gf/configure: Updated.

2000-12-02  Werner LEMBERG  <wl@gnu.org>

	* doc/cjk-enc.doc: Clarify usage of cjk-coding.
	* doc/INSTALL: Add hints how to use kpsewhich to check
	configuration.

2000-12-01  Werner LEMBERG  <wl@gnu.org>

	* doc/INSTALL: Fix documentation of --with-kpathsea-include.
	* doc/cjk-enc.doc: Fix typo.

2000-09-21  Werner LEMBERG  <wl@gnu.org>

	* texinput/{CJK.sty, CJKulem.sty, pinyin.sty, ruby.sty}: Replacing
	some \ifdim with \ifnum.

2000-09-20  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKulem.sty: Fixed two nasty bugs (spotted by Sim Ing
	<sim@ubs-aptsocap.org>): No underlining for \CJKglue and no \CJKglue
	before and after \uline.

2000-08-28  Werner LEMBERG  <wl@gnu.org>

	* utils/thaifont/texmf/dvips/config/config.{norasi,dbtt}: New files.
	* doc/thaifont.doc: Added info about PS font configuration.

2000-08-24  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/emacs-20.3/thai-word.el (thai-update-word-table): Add
	documentation string.

2000-08-24  HANDA Ken'ichi  <handa@etl.go.jp>

	* utils/lisp/emacs-20.3/thai-word.el (thai-update-word-table): New
	function.
	(thai-find-word-ends): Fix loop.

2000-08-23  Werner LEMBERG  <wl@gnu.org>

	* texinput/thai/thaicjk.ldf: Remove warning about nonexistent
	hyphenation patterns.

2000-08-20  Werner LEMBERG  <wl@gnu.org>

	Another big sigh.  Wrong glyph names for Norasi's Thai digits.
	Additionally, all ligature rules no longer use `>' to make kerning
	possible.

	* utils/thaifont/texmf/dvips/base/norasi.enc: Fixed.
	* utils/thaifont/tools/{thai.enc,thailigs.vpl}: Updated.
	* utils/thaifont/texmf/fonts/{tfm,vf}/public/{dbtt,norasi}/*:
	Regenerated.

2000-08-19  Werner LEMBERG  <wl@gnu.org>

	* examples/thai.tex: New file.
	* doc/history.txt: Updated.

	* examples/CJKbabel.tex: Doc fixes.

2000-08-17  Werner LEMBERG  <wl@gnu.org>

	* doc/cjk-enc.el, doc/thaifont.doc: Give better URL for thailatex
	package.

2000-08-15  Werner LEMBERG  <wl@gnu.org>

	Sigh, another forgotten Thai ligature rule.

	* utils/thaifont/tools/{thai.enc,thailigs.vpl}: Updated.
	* utils/thaifont/texmf/fonts/{tfm,vf}/public/{dbtt,norasi}/*:
	Regenerated.

2000-08-15  Werner LEMBERG  <wl@gnu.org>

	* texinput/thai/c90{cmr,cmss.cmtt}.fd: Make font substitution
	silent.

	* utils/thaifont/texmf/dvips/base/norasi.enc: Fixing typo.
	* utils/thaifont/texmf/fonts/{tfm,vf}/public/norasi/*: Updated.

2000-08-13  Werner LEMBERG  <wl@gnu.org>

	Improved support for Thai.

	* doc/thaifont.doc: New file.

	* utils/thaifont/*: Metrics and support files for Thai fonts.

	* texinput/thai/c90{nrsr,dbss}.fd: New font definition files for
	dbtt and norasi font families.
	* texinput/thai/c90{cmr,cmss,cmtt}.fd: Font alias files.
	* texinput/thai/thaicjk.ldf: New file for thai support in Babel.
	* texinput/thai/thai.sty: Removed.

	* utils/lisp/emacs20.3/cjk-enc.el: Redesigned Thai support by
	HANDA Ken'ichi <handa@etl.go.jp>.
	Will now run under XEmacs also (with help of Martin Buchholz
	<martin@xemacs.org>).  No Thai support yet due to limitations in
	current XEmacs version (21.2).
	(cjk-write-all-files): New optional argument to force the processing
	of all files.
	(do-batch-cjk-write-file): New function.
	(batch-cjk-write-file): Use do-batch-cjk-write-file.
	(batch-force-cjk-write-file): New function.  Uses
	do-batch-cjk-write-file also.
	* utils/lisp/mule-2.3/cjk-enc.el: Rename write-cjk-file to
	cjk-write-file for consistency.
	* utils/lisp/emacs20.3/thai-word.el: New file written by HANDA
	Ken'ichi for Thai word breaking support.  Replaces thaiconv.
	* utils/thaiconv: Removed.

	* utils/lisp/emacs20/cjk-enc.el: Removed.  No longer supported.

	* texinput/mule/MULEenc.sty: Adapted to new cjk-enc.el version.
	Make it robust for CJKulem.sty.

	* examples/CJKbabel.tex: Use CJKulem.sty and thaicjk module for
	Babel.
	* examples/muletest.tex: Remove \if... \fi clause for Thai.

	* doc/history.txt, doc/INSTALL: Updated.

2000-08-12  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJKulem.sty: New file which provides CJK support for
	ulem.sty.
	* doc/history.txt, doc/CJK.doc: Updated.

2000-08-09  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/configure.in: Replaced --with-kpathsea-dir with
	--with-kpathsea-lib and --with-kpathsea-include.
	* utils/hbf2gf/configure, doc/history.txt, doc/INSTALL,
	doc/hbf2gf.doc: Updated.

	* texinput/CJK.sty, texinput/mule/MULEenc.sty: New command
	\CJKverbatim which disables \Thaiglue and \CJKglue in verbatim
	environments if the `verbatim' package is loaded.
	* doc/history.txt, doc/CJK.doc, doc/commands.doc: Updated.

2000-07-30  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub: Updated to
	latest version from ftp.gnu.org.

2000-07-27  Werner LEMBERG  <wl@gnu.org>

	* utils/thaiconv/thaiconv.c: Improve comment.

	* *.fd: Set \hyphenchar to -1 for all CJK fonts.

2000-06-23  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/config.guess, utils/hbf2gf/config.sub: Updated to
	latest version from ftp.gnu.org.

	* texinput/CJK.enc: Removed redefinition of C42 and C49.

2000-05-03  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty: Specifying an optional argument to the `CJK'
	size function will no longer produce a warning message for each
	subfont.

	* contrib/wadalab/*.fd, doc/CJK.doc, doc/fonts.doc: Wadalab PS fonts
	now use `CJK' size functions instead of `DNP' ones.

	* doc/history.txt: Updated.

2000-05-02  Werner LEMBERG  <wl@gnu.org>

	* texinput/*/*.cpx: Replace incorrect 0xFF with 0x7F.

2000-04-18  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty, texinput/pinyin.sty, texinput/ruby.sty:
	Balancing the small kern control values, e.g. using
	`\kern -1sp\kern 1sp' instead of `\kern 1sp' only.

	Replacing kern value of 3sp with 5sp to avoid clash with ulem.sty.

2000-04-01  Werner LEMBERG  <wl@gnu.org>

	Version 4.3.0 released
	======================

	This version exists on the Tex Live CD 5 only; a lot of files have
	been adapted to the special needs of the CD's texmf tree -- these
	changes are not in the CVS tree.

2000-03-15  Werner LEMBERG  <wl@gnu.org>

	* contrib/wadalab/wadalab.map: Renamed from Wadalab.map
	* contrib/wadalab/DNP.doc: Updated accordingly.

	* utils/hbf2gf/cfg/*: Updated -- if possible, the foundry is used
	as the target directory instead of the encoding, e.g.
	`tfm/ntu/b5ka12'.

2000-03-14  Werner LEMBERG  <wl@gnu.org>

	* texinput/SJIS/SJISdnp.{chr,enc}: New files to support SJIS
	encoding with DNP fontencoding.
	* texinput/CJK.enc: Add SJISdnp.
	Add forgotten punctuation pattern macro to KSHL encoding.
	* doc/history.txt, doc/CJK.doc, doc/command.doc: Update.

2000-03-13  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty: Fixing definition of ^^7f to do nothing if
	written to the TOC file.

2000-03-12  Werner LEMBERG  <wl@gnu.org>

	* texinput/KS/HLaTeX/pshan.sty: Fix typo.

	Call \mj to activate default family correctly.

	* contrib/wadalab/makefont: Add echo commands.
	* contrib/wadalab/DNP.doc: Updated. Add info about gsftopk.

2000-03-03  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/README: New file.
	* utils/hbf2gf/hbf2gf.1, doc/hbf2gf.doc: Small improvements.

	* README: Removed `romaji environment' from TODO section.  According
	to HANDA Ken'ichi <handa@etl.go.jp> it is impossible to provide
	hyphenation patterns for transcribed Japanese without semantic
	analysis.

2000-03-02  Werner LEMBERG  <wl@gnu.org>

	* README, doc/INSTALL: Slight improvements.

	* utils/hbf2gf/Makefile.in, utils/hbf2gf/configure.in: Fix incorrect
	test for NO_STRDUP.  Thanks to <Andries.Brouwer@cwi.nl>.

2000-02-06  Werner LEMBERG  <wl@gnu.org>

	* texinput/CJK.sty, texinput/mule/MULEenc.sty,
	utils/lisp/*/cjk-enc.el, utils/*conv/*conv.[cw], history.txt,
	CJK.doc, cjk-enc.doc: Use 0x7F both as the multiplex character and
	as a delimiter -- apparently no package uses this character...
	This solves all problems with \uppercase and \lowercase.

	* utils/hbf2gf/cfg/j2so12.cfg: Added `min_char' parameter to get
	correct offsets (thanks to Martin Minich
	<minich5@kepler.fmph.uniba.sk> for finding this bug).

2000-01-26  Werner LEMBERG  <wl@gnu.org>

	* doc/cjk-enc.doc, doc/history.txt, examples/CJKbabel.tex,
	examples/muletest.tex, texinput/mule/MULEenc.sty,
	utils/lisp/*/cjk-enc.el: Change X5 to T5.

2000-01-20  Werner LEMBERG  <wl@gnu.org>

	* examples/muletest.tex: Greek added; updated to X5 encoding.
	* examples/CJKbabel.tex: Greek added; updated to X5 encoding.

	* texinput/mule/MULEenc.sty: Use \AtBeginDocument for \mule@<accent>
	definitions.

2000-01-14  Werner LEMBERG  <wl@gnu.org>

	* doc/cjk-enc.doc: Added info about file variables to specify
	document encoding.

2000-01-03  Ching-Mo CHANG  <chingmo@mail.onweb.com.tw>

	* utils/lisp/emacs-20.3/cjk-enc.el (cjk-write-all-files): Always
	returned nul for include and bib file names due to incorrect
	pattern matching.

1999-12-18  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/configure.in: Removed `-pedantic' flag which causes
	problems with newer gcc versions.

1999-11-19  Werner LEMBERG  <wl@gnu.org>

	* examples/muletest.tex, examples/CJKbabel.tex: Fixing a typo.

1999-11-07  Werner LEMBERG  <wl@gnu.org>

	* doc/CEF.doc: Minor fixes.

	* doc/CJK.doc: Updated; minor fixes.

1999-11-06  Werner LEMBERG  <wl@gnu.org>

	* doc/cjk-enc.doc, doc/commands.doc, doc/fonts.doc: Minor fixes.

	* doc/vertical.doc, doc/history.txt: Updated.

1999-11-05  Werner LEMBERG  <wl@gnu.org>

	* texinput/mule/MULEenc.sty: Added \CJKinclude{<file>} and
	\CJKbibliography{<file>}.  These functions act identically to
	\include resp. \bibliography but load <file>.cjk
	resp. <file>-cjk.bib.

	* utils/lisp/emacs-20.3/cjk-enc.el: Using `cjk' throughout as the
	prefix to variable and function names.  This causes a renaming of
	virtually all functions.  Some other local variables were renamed
	also for consistency.

	Changing ET5 to X5 encoding for Vietnamese.

	(decompose-char): Removed.  Not needed at all.

	(cjk-tex-in-comment): New function.  Similar to AUC TeX's
	TeX-in-comment function; has been added to be independent from AUC
	TeX.

	(cjk-write-all-files): New function.  It checks for \CJKinclude
	and \CJKbibliography commands in the master file and converts the
	referenced files accordingly if necessary.  Intended as a hook to
	AUC TeX to make multiple files work as expected.

1999-11-02  Werner LEMBERG  <wl@gnu.org>

	* doc/cjk-enc.doc: Small improvement in explanation of usage with
	AUC TeX.

1999-10-24  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/emacs-20.3/cjk-enc.el (get-cjk-name): New function.

	(file-write-cjk-file, batch-write-cjk-file): New functions which
	do the same as write-cjk-file but operate on a given file (resp. a
	suite of files and directories given on the command line).

	(write-cjk-file): Will now properly ask for a file name if the
	current buffer is not visiting a file.

	* doc/cjk-enc.doc: Expanded TeX-translate-location-hook to cover
	CJK BibTeX input files also.

	TeX-run-CJK-LaTeX now checks whether it must call write-cjk-file
	at all (emacs > 20.3 only).

1999-10-07  Werner LEMBERG  <wl@gnu.org>

	* texinput/mule/MULEenc.sty: Removed \textendash wrapper macro.

	* utils/lisp/{emacs-20.3,emacs-20,mule-2.3}/cjk-enc.el: Added
	iso-8859-9 (Greek) support (mapped to LGR encoding as used in the
	Babel package).

	Fixed character `SOFT-HYPHEN' in iso-8859-x encodings (using `\-'
	instead of \textendash).

	* README, doc/cjk-enc.doc, doc/history.txt: Updated.

	* doc/CJK.doc: Fixed a typo.

	* texinput/CJK.enc, texinput/CJK.sty, texinput/*/{*.cap,*.cpx}:
	Replaced `\ifx\foo \undefined' with `\@ifundefined{}{}' to fix the
	case that a not-defined macro has been tested with \@ifundefined
	before.  In this case, it is no longer undefined but identical to
	\relax.

	* texinput/pmC.chr: Fixed punctuation macros for pmC.

1999-10-02  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty: The method with appending `\-' to all
	syllables fails (stupid I am :-), so here a solution which really
	works.  It uses a small kern (4sp, similar to the ruby and CJK
	packages) to tell the following pinyin syllable that a
	discretionary has to be inserted.

1999-10-01  Werner LEMBERG  <wl@gnu.org>

	* texinput/mule/MULEenc.sty: \lccode and \uccode of ^^ff must not
	be modified, otherwise hyphenation patterns containing \ss will
	fail (which happens e.g. in German).

1999-09-28  Werner LEMBERG  <wl@gnu.org>

	* doc/history.txt: Updated.

	* utils/pyhyphen/pyhyph.tex, utils/pyhyphen/pytest.tex,
	utils/pyhyphen/pinyin.ldf, doc/pyhpyhen.doc: Hyphenation patterns
	for unaccented pinyin syllables to be used with the Babel package.

	* utils/pyhyphen/pinyin.c, utils/pyhpyhen/pinyin.tr: Utility files
	for creating pinyin hyphenation patterns.

1999-09-27  Werner LEMBERG  <wl@gnu.org>

	* doc/history.txt: Updated.

1999-09-21  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty: Adding hyphenation points at the end of all
	syllables.

1999-09-18  Werner LEMBERG  <wl@gnu.org>

	* texinput/pinyin.sty: Making accent commands like \py@a robust.

	Added option `useCMmacron' (for LaTeX only) to use a macron accent
	from the CM fonts in case the used font doesn't have it
	(e.g. some versions of virtual files for Palatino).

1999-08-26  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/hbf2gf.1: Added some documentation how to find out
	the expanded value of a kpathsea variable (like $MISCFONT).

1999-08-07  Werner LEMBERG  <wl@gnu.org>

	* utils/thaiconv/thaiconv.c (adj): Fixed invalid array index in
	case of marks without base characters.

1999-07-07  Werner LEMBERG  <wl@gnu.org>

	* texinput/Bg5/Bg5.chr,
	  texinput/extended.chr: Fixed a typo \CJK@temp->\CJK@gtemp

1999-06-30  Werner LEMBERG  <wl@gnu.org>

	* utils/lisp/emacs-20/cjk-enc.el,
	  utils/lisp/emacs-20.3/cjk-enc.el,
	  utils/lisp/mule-2.3: Fixed code for 0x80 multiplex character.

1999-06-22  Werner LEMBERG  <wl@gnu.org>

	* doc/TDS.doc: Completely revised.

1999-06-10  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/configure.in: Removed `-ansi' flag which can cause
	problems with the kpathsea library (which is not compiled with
	-ansi).

1999-06-07  Werner LEMBERG  <wl@gnu.org>

	* utils/hbf2gf/hbf2gf.1: Added documentation about MiKTeX.

	* utils/hbf2gf/hbf2gf.w: Added support for MiKTeX file search
	library.

	* texinput/CEF/*.fd: Removed -- these files were erroneously
	included into the CVS repository.

1999-06-04  Werner LEMBERG  <wl@gnu.org>

	* *.fd files: minor documentation addition regarding font
	encoding.

	* all files: Changed date/version to 4.3.0.

1999-06-02  Werner LEMBERG  <wl@gnu.org>

	* README: Added info about http and ftp home sites and how to
	access the CVS repository.

1999-06-01  Werner LEMBERG  <wl@gnu.org>

	* README: Added info about CVS mailing list.

1999-05-29  Werner LEMBERG  <wl@gnu.org>

	* README: Added mailing list.

	* doc/INSTALL: Small correction.

	* README: Small additions.

;; Local Variables:
;; coding: utf-8
;; End:

    Copyright (C) 1999, 2001-2012
      Werner Lemberg <wl@gnu.org>

  This file is part of the CJK package for using Asian logographs
  (Chinese/Japanese/Korean) with LaTeX2e.

  This program is free software; you can redistribute it and/or modify
  it under the terms of the GNU General Public License as published by
  the Free Software Foundation; either version 2, or (at your option)
  any later version.

  This program is distributed in the hope that it will be useful,
  but WITHOUT ANY WARRANTY; without even the implied warranty of
  MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
  GNU General Public License for more details.

  You should have received a copy of the GNU General Public License
  along with GNU Emacs; see the file COPYING.  If not, write to the
  Free Software Foundation, Inc., 51 Franklin Street, Fifth Floor,
  Boston, MA 02110-1301, USA.


==> cjk-4.8.5/Makefile <==
# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

# You need GNU make to run this Makefile.
#
# Some issues:
#
# o This Makefile is intended to build the distribution tarballs only,
#   not to compile binaries.
#
# o Binaries of the CJK utility programs (and the standard tex stuff,
#   including dvipdfmx) must work.
#
# o GNU extensions of various utility programs are used.
#
# o emacs 22 (or newer) and the `cweave' program from the `c2cweb'
#   package, renamed to `cweavex', are needed.
#
# o The TeXLive version of some font definition files are used (in the
#   `texlive' subdirectory).

version=4.8.5

distdir=cjk-$(version)
abs-distdir=$(shell pwd)/$(distdir)

DISTDIRS=$(shell find . -type d | grep -v .git | grep -v $(distdir))

# expected: subdirs `dvi' and `cjk'
CJK2DVI=\
  (cd dvi; \
   TEXINPUTS=$(abs-distdir)/{texlive,texinput//,contrib/wadalab,utils/pyhyphen}: \
   TFMFONTS=$(abs-distdir)/utils/thaifont/texmf/fonts/tfm//: \
     texi2dvi -l latex ../cjk/$@.cjk; \
   rm -f $@.aux $@.log $@.toc)

# LATEX2DVI srcdir targetdir
# expected: targetdir/dvi
LATEX2DVI=\
  cp $(1)/$@.tex $(2)/dvi; \
  (cd $(2)/dvi; \
   TEXINPUTS=$(abs-distdir)/{texlive,texinput//,contrib/wadalab,utils/pyhyphen}: \
   TFMFONTS=$(abs-distdir)/utils/thaifont/texmf/fonts/tfm//: \
     texi2dvi -l latex $@.tex; \
   rm -f $@.tex $@.aux $@.log $@.toc)

# DVI2PDF paper-format
# expected: subdir `pdf' and `dvi'
DVI2PDF=\
  dvipdfmx -v -p $(1) -o pdf/$@.pdf dvi/$@.dvi
  

# CONVERT converter srcdir targetdir [paper-format]
CONVERT=\
  cd $(distdir); \
  $(1) < $(2)/$@.tex > $(3)/cjk/$@.cjk; \
  cd $(3); \
  $(CJK2DVI); \
  $(if $(4),$(call DVI2PDF,$(4)),$(call DVI2PDF,letter))

# MULE srcdir targetdir [paper-format]
MULE=\
  cd $(distdir); \
  emacs --batch \
        --load utils/lisp/emacs/cjk-enc.el \
        --funcall batch-cjk-write-file \
        $(1)/$@.tex; \
  mv $(1)/$@.cjk $(2)/cjk; \
  cd $(2); \
  $(CJK2DVI); \
  $(if $(3),$(call DVI2PDF,$(3)),$(call DVI2PDF,letter))

# LATEX srcdir targetdir [paper-format]
LATEX=\
  cd $(distdir); \
  $(call LATEX2DVI,$(1),$(2)); \
  cd $(2); \
  $(if $(3),$(call DVI2PDF,$(3)),$(call DVI2PDF,letter))


DISTTARGETS=\
  READMEb5 \
  READMEgb \
  Big5 \
  Big5vert \
  CEF_test \
  CJKbabel \
  CJKfntef \
  CJKutf8 \
  CJKspace \
  CJKmixed \
  GB \
  JIS \
  KS \
  SJIS \
  UTF8 \
  muletest \
  pytest \
  py_test \
  rubytest \
  thai \
  thai_utf8 \
  c90


all:
	@echo
	@echo "    Say \`make dist' to build the tarballs."
	@echo


READMEb5:
	$(call CONVERT,bg5conv,doc/chinese,doc,a4)
READMEgb:
	$(call LATEX,doc/chinese,doc)
Big5 Big5vert:
	$(call CONVERT,bg5conv,examples,examples)
CEF_test:
	$(call CONVERT,cefconv,examples,examples)
SJIS:
	$(call CONVERT,sjisconv,examples,examples)
CJKbabel muletest rubytest thai thai_utf8:
	$(call MULE,examples,examples)
GB JIS KS UTF8 py_test CJKfntef CJKutf8 CJKspace CJKmixed:
	$(call LATEX,examples,examples)
pytest:
	$(call LATEX,utils/pyhyphen,examples)
c90:
	(cd $(abs-distdir)/utils/thaifont/tools; \
	 ln -s c90.etx c90.tex)
	$(call LATEX,utils/thaifont/tools,doc)


dist: distsrc predistdoc distdoc

distsrc:
	-rm -rf $(distdir)
	rm -f $(distdir).tar.gz
	rm -f $(distdir)-doc.tar.gz
	mkdir $(distdir)
	srcdir=`pwd`; \
	for d in $(DISTDIRS); do \
	  mkdir -p $(distdir)/$$d; \
	  (cd $(distdir)/$$d; \
	   f=`find $$srcdir/$$d -maxdepth 1 -type f`; \
	   test -z "$$f" || ln -s $$f . || true); \
	done
	for f in `find $(abs-distdir)/utils -name '*.w'`; do \
	  ctangle $$f - `echo $$f | sed s/w$$/c/`; \
	done
	tar -H ustar -chf - $(distdir) | gzip -9 -c > $(distdir).tar.gz

predistdoc:
	mkdir -p $(distdir)/doc/{cjk,dvi,pdf}
	mkdir -p $(distdir)/examples/{cjk,dvi,pdf}
	mkdir -p $(distdir)/doc/man/{dvi,html,pdf,txt}
	echo "This directory contains files which are \`preprocessed' with" \
	  > $(distdir)/doc/cjk/README
	echo "cjk-enc.el, bg5conv, etc." \
	  >> $(distdir)/doc/cjk/README
	echo \
	  >> $(distdir)/doc/cjk/README
	echo "You can feed them directly into LaTeX." \
	  >> $(distdir)/doc/cjk/README

distdoc: $(DISTTARGETS) manpages cweb
	for f in `find $(distdir) -type l`; do \
	  rm $$f; \
	done
	for f in `find $(distdir) -name '*.c'`; do \
	  rm $$f; \
	done
	-for d in `find $(distdir) -depth -type d`; do \
	  rmdir --ignore-fail-on-non-empty $$d; \
	done
	tar -H ustar -chf - $(distdir) | gzip -9 -c > $(distdir)-doc.tar.gz
	rm -rf $(distdir)

manpages:
	for f in `find utils -type f -name '*.1'`; do \
	  groff -ww -Tdvi -dpaper=letter -P-pletter -mec -man -rS11 $$f > \
	    $(abs-distdir)/doc/man/dvi/`basename $$f .1`.dvi; \
	  groff -ww -Tps -dpaper=letter -P-pletter -man -rS11 $$f | \
	    ps2pdf - $(abs-distdir)/doc/man/pdf/`basename $$f .1`.pdf; \
	  groff -ww -Tlatin1 -man -P-bcu $$f > \
	    $(abs-distdir)/doc/man/txt/`basename $$f .1`.txt; \
	  groff -ww -Thtml -man $$f > \
	    $(abs-distdir)/doc/man/html/`basename $$f .1`.html; \
	done

cweb:
	for f in `find utils -type f -name '*.w'`; do \
	  cp $$f $(abs-distdir)/doc/dvi; \
	  (cd $(abs-distdir)/doc/dvi; \
	   F=`basename $$f .w`; \
	   cweavex +a $$F.w; \
	   tex $$F; \
	   rm -rf $$F.idx $$F.log $$F.scn $$F.tex $$F.toc $$F.w; \
	   dvipdfmx -v -p letter -o ../pdf/$$F.pdf $$F); \
	done

# EOF


==> cjk-4.8.5/contrib/wadalab/fixwada <==
# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

# This script fixes the Wadalab fonts which have been created with the
# `makefont' script of the CJK package version 4.5.1 or earlier.
#
# It converts all PFB files in the current directory.


for i in *.pfb; do
  echo $i
  mv $i $i.old
  cat $i.old | \
  t1disasm | \
  awk '
    {
      sub(/001\.001/, "001.002")

      if (/%%Creation/) {
        print "%%CreationDate: 2003-Feb-07"
        next
      }

      if (/0 -160 rmoveto/ && last_is_hsbw) {
        last_is_hsbw = 0
        next
      }

      if (/hsbw/) {
        last_is_hsbw = 1
        waiting_for_Xmoveto = 1
      }
      else
        last_is_hsbw = 0

      if (waiting_for_Xmoveto) {
        if (/rmoveto/) {
          printf "\t%d %d rmoveto\n", $1, $2 - 160
          waiting_for_Xmoveto = 0
          next
        }
        else if (/vmoveto/) {
          printf "\t%d vmoveto\n", $1 - 160
          waiting_for_Xmoveto = 0
          next
        }
        else if (/hmoveto/) {
          printf "\t%d %d rmoveto\n", $1, -160
          waiting_for_Xmoveto = 0
          next
        }
      }

      if (/moveto/)
        print "\tclosepath"

      if (/hstem/) {
        printf "\t%d %d hstem\n", $1 - 160, $2
        next
      }

      print
    }
  ' | \
  t1asm > $i
  rm $i.old
done


==> cjk-4.8.5/contrib/wadalab/makefont <==
#!/bin/sh
#
# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

# Version 1.0
#
# This script transforms Wadalab PFA and AFM files created by the
# wftodm program into PFB and TFM files.  All files in the current
# directory and its subdirectories are converted.
#
# Additionally, it normalizes the font matrix so that the subfonts work
# with pdfTeX; for convenience, it also inserts `closepath' commands to
# end subpaths in glyphs.
#
# Note that an older version of this script (without a version number) has
# some flaws; you should either regenerate all Wadalab subfonts or use the
# `fixwada' script to fix PFB fonts which have already been created with
# this older version.
#
# The programs t1asm, t1disasm, and afm2tfm must be in the path.

for f in `find . -name '*.pfa' -print`; do
  echo processing $f
  name=`basename $f .pfa`
  t1disasm < $name.pfa > $name.old

  cat $name.old | \
  awk '
    {
      sub(/001\.001/, "001.002")
      sub(/\[.001 0 0 .001 0 -0.16\]/, "[.001 0 0 .001 0 0]")
      sub(/\[0 0 1000 1000\]/, "[0 -160 1000 840]")

      if (/%%Creation/) {
        print "%%CreationDate: 2003-Feb-07"
        next
      }

      if (/hsbw/)
        waiting_for_Xmoveto = 1

      if (waiting_for_Xmoveto) {
        if (/rmoveto/) {
          printf "\t%d %d rmoveto\n", $1, $2 - 160
          waiting_for_Xmoveto = 0
          next
        }
        if (/vmoveto/) {
          printf "\t%d vmoveto\n", $1 - 160
          waiting_for_Xmoveto = 0
          next
        }
        if (/hmoveto/) {
          printf "\t%d %d rmoveto\n", $1, -160
          waiting_for_Xmoveto = 0
          next
        }
      }

      if (/moveto/)
        print "\tclosepath"

      if (/hstem/) {
        printf "\t%d %d hstem\n", $1 - 160, $2
        next
      }

      print
    }
  ' > $name.asm
  rm $name.old

  t1asm < $name.asm > $name.pfb
  rm $name.asm
done

for f in `find . -name '*.afm' -print`; do
  echo processing $f
  name=`basename $f .afm`
  mv $name.afm $name.old

  cat $name.old | \
  sed -e "
      s/FontBBox 0 0 1000 1000/FontBBox 0 -160 1000 840/
      s/B 0 0 1000 1000/B 0 -160 1000 840/
  " > $name.afm

  rm $name.old

  afm2tfm $name.afm &> /dev/null
done

# EOF


==> cjk-4.8.5/doc/INSTALL <==
This is the file INSTALL of the CJK macro package ver. 4.8.5 (16-Oct-2021).

Installation Guide
==================

It is probably a good idea to get a packaged version of CJK---be warned that
installing CJK is *not* trivial.

The easiest solution is to use the TeX Live CD which is distributed among
members of TeX user groups worldwide. It comes with a ready-to-run CJK setup
together with basic CJK fonts (in outline format if freely available) for
almost all encodings. To get a recent snapshot, try the SVN archive. See

  http://www.tug.org/texlive/svn/

for more details.

. Using web sites like http://rpmseek.com you can find and download CJK
  packages for most GNU/Linux distributions like SuSE or Debian.

. For FreeBSD try this:

    http://www.freebsd.org/ports/chinese.html

. MikTeX also provides packages for CJK.


Here a check list for the impatient (experienced) user which tries to show
whether you've done all steps to install the CJK package and fonts. It is
assumed that you want to install both ttf2pk and hbf2gf.

Detailed explanations can be found below.


--- begin checklist ---------------------------------------------------------

. Have you installed a LaTeX 2e version newer or equal to 2001/06/01? The
  version of LaTeX is given in each log file produced by LaTeX. For using
  CJKutf8.sty you even need version 2003/12/01.

. Have you removed an older version of CJK? If not, do it now but don't
  forget to save your FD and other files which you have changed! Don't
  forget also to remove the ttf2pk and hbf2gf binaries.

. Can the texinput tree of the CJK package be found by your TeX
  implementation? Have you activated subdirectory searching?

. Have you downloaded the needed font packages (either ps, hbf or ttf)? See
  also contrib/wadalab/DNP.txt for the Japanese Wadalab fonts. Have you
  moved the TFM files into your TFM-tree (or updated TFMINPUTS accordingly)?
  Ditto for VF files if needed.

. Have you installed ttf2pk and ttf2tfm from the FreeType 1 package (only
  needed for TrueType fonts)? Note that FreeType 2 won't work.

. Have you run ttf2tfm to create the proper TFM files from your TrueType
  fonts? This won't be done automatically via mktextfm or MakeTeXTFM!

. Have you updated the ttfonts.map file for ttf2pk? Have you updated the
  various hbf2gf config files? Have you copied them to the right places?
  Don't forget to install ttf2pk's SFD and other data files which define the
  various CJK subfonts and encodings.

. Have you modified and installed the script files for automatic font
  generation (not necessary for teTeX 1.0 or newer)?

. If you want Thai support, have you followed the instructions given in
  thaifont.txt?


web2c/teTeX users:

. Do you have a C compiler and a make program available for compilation? GNU
  gcc and GNU make are recommended.

. Have you updated special.map?

. Have you used the options --with-kpathsea-include=... and
  --with-kpathsea-lib=... while calling the configure script of hbf2gf
  (or ttf2pk)? Otherwise no file searching library is used which yields
  surprising results... Note: Don't use `/usr/include/kpathsea', for
  example, but `/usr/include' as an argument to --with-kpathsea-include.

. To check whether kpathsea correctly finds HBF files and configuration
  files for hbf2gf, say:

    kpsewhich -progname=hbf2gf -format='misc fonts' <your_font>.hbf
    kpsewhich -progname=hbf2gf -format='other text files' <your_file>.cfg

  The same for TrueType fonts and the ttf2pk config file:

    kpsewhich -progname=ttf2pk <your_font>.ttf
    kpsewhich -progname=ttf2pk -format='other text files' ttfonts.map

  [Recent kpathsea versions (like 3.5.5) which come with the new teTeX or
   TeXLive distributions have a new variable `TEXFONTMAPS' for map files;
   you should use this test

     kpsewhich -progname=ttf2pk -format=map ttfonts.map

   instead of the last one.]

. Have you compiled the various *conv utility programs (like bg5conv)? Have
  you installed them together with the caller scripts (like bg5latex) in
  your path? FOR BIG 5 ENCODING YOU SHOULD ALWAYS USE bg5latex or
  bg5pdflatex (except if you use cjk-enc.el). FOR SJIS ENCODING YOU SHOULD
  ALWAYS USE sjislatex or sjispdflatex.

. Have you updated and controlled the texmf.cnf configuration file or set
  the various environment variables? (TEXINPUTS, TFMFONTS, PKFONTS,
  MISCFONTS, TTFONTS, probably TTF2PKINPUTS, TTF2TFMINPUTS, HBF2GFINPUTS)

. ttf2pk and hbf2gf should be in the same directory where your TeX binaries
  like `texconfig' or `gftopk' are (or you must set TEXMFCNF and probably
  TEXMF in the environment). Soft links won't work!

. Finally, have you run texhash (or mktexlsr) after finishing all other
  things?


emTeX users:

. Have you created a LaTeX format file which allows plain 8bit input and
  output without using any TeX Code Page (tcp)?

. Have you installed 4DOS (4OS2 or Take Command) for running the file
  dvidrv.btm?

. Have you configured dvidrv.btm?

. Have you installed the various *conv utility programs (like bg5conv)?
  together with the caller scripts (like bg5latex.bat)? FOR BIG 5 ENCODING
  YOU SHOULD ALWAYS USE bg5latex.bat . FOR SJIS ENCODING YOU SHOULD ALWAYS
  USE sjisltx.bat .

. Have you created and installed TFM files for fonts not in a CJK font
  package?

. Check whether you have updated all needed environment variables (TEXINPUT,
  TEXTFM, TTFONTS, TTFCFG, HBFONTS, HBFCFG) and your dvidrv configuration
  file or files (+font-files, +virtual-fonts).


In case of errors, verify the list step by step. Detailed information for
each step can be found in the documentation files of CJK. Under web2c or
teTeX, you can set the KPATHSEA_DEBUG environment variable to -1, then all
debugging info is shown and sent to stderr; it is *highly* recommended that
you read the kpathsea.info files. Under emTeX, read the various
documentation files, especially dvidrv.doc and tex.doc, and check the log
file of your dvi driver.

For hbf2gf, read hbf2gf.txt and its manual page (hbf2gf.1 or a formatted
version of it). Similarly, more info on ttf2tfm and ttf2pk can be found in
ttf2pk.doc and the manual pages ttf2pk.1 and ttf2tfm.1 (or a formatted
version).

--- end checklist -----------------------------------------------------------



Unix (web2c and teTeX)
----------------------

. If you can become root, rename the `texinput' directory tree of CJK into
  `CJK' or something else and add it to your (local) web2c texinput tree
  (for example, /usr/local/share/texmf.local/tex/latex/CJK).

. If you can't become root, modify the TEXINPUTS environment variable
  instead so that it includes the CJK directory; use a command similar to

    setenv TEXINPUTS :<your CJK directory>//

  to let TeX search the standard directories and your CJK tree, e.g.,

    setenv TEXINPUTS :/home/joe_user/CJK/4_3.0/texinput//

  (Note the leading double colon to append a path, and the double slash to
  activate subdirectory searching---for details see the kpathsea info
  files.)

  [Recent teTeX and TeXLive versions automatically search a TEXMF tree in
   your home directory called `texmf'.]

  See contrib/wadalab/DNP.txt for the Japanese Wadalab fonts.

. Edit the FD files of the encodings you want to use to specify the fonts
  you have. An explanation of the additional size commands CJK provides can
  be found in fonts.txt .

  Note: Most FD example files from the CJK package are set up for PS fonts
  from the TeXLive distribution.

  If you use the CJK font packages (see below) no changes are needed.

. [In case you plan to use only outline fonts (PFB, TTF) you can omit the
   installation of hbf2gf and HBF fonts.]

  If necessary, create TFM (and PK) files from CJK bitmaps with hbf2gf
  (found in utils/hbf2gf). This program comes with a configure script; say
  `./configure --help' in the utils/hbf2gf directory for configuration
  options. You need a compiled kpathsea library and its header files; in
  most cases you say

    ./configure --prefix=/usr/local/TeX \
                --with-kpathsea-include=<INCLUDEDIR> \
                --with-kpathsea-lib=<LIBDIR>
    make
    make install

  for a normal compilation and installation. Replace `/usr/local/TeX' with a
  path to your TeX distribution, and <DIR> with the directory one level
  higher than the library and the include files themselves. Example:
  libkpathsea.a is in /usr/local/TeX/lib/i686-linux, kpathsea.h is in
  /usr/local/TeX/include/kpathsea; then <LIBDIR> should be
  `/usr/local/TeX/TeX/lib/i686-linux', and <INCLUDEDIR> should be
  `/usr/local/TeX/include' (and not `/usr/local/TeX/include/kpathsea).

  See hbf2gf.txt, the man page (hbf2gf.1), and the documentation of the
  source file (hbf2gf.dvi) for further details. Usually it is sufficient to
  let hbf2gf create a complete set of TFM files; PK fonts are then created
  on demand.

  Older kpathsea versions need a patched MakeTeXPK or mktexpk script; you
  should apply the proper patch(es) from utils/hbf2gf/scripts. No changes to
  the script files are necessary for teTeX 1.0 and newer.

  The CJK font packages already contain TFM (and VF) files arranged for the
  (new) TDS directory structure; add it directly to your TEXMF tree.

. Free Chinese TrueType fonts (for both simplified and traditional Chinese)
  with a license similar to the GPL can be found on

    ftp://ftp.gnu.org/gnu/nongnu

  and its mirrors worldwide. You might also search websites of companies
  offering WWW browser; they often come with CJK language packs which
  contain CJK TrueType fonts.

  Please note that many CJK TrueType fonts only have a Unicode mapping
  table. You should use the SFD files from the ttf2pk package starting with
  the letter `U' (e.g., UKS.sfd) which maps Unicode fonts to language
  specific encoded subfonts as needed by the CJK package.

  The ttf2pk package found in the contrib/ttf2pk directory of

    ftp://ftp.freetype.org/pub/
            freetype/unstable/freetype1-contrib-current.tar.gz

  contains the two programs ttf2tfm and ttf2pk for converting TrueType fonts
  into TFM and PK fonts, respectively. By the way, this package is not
  restricted to CJK TrueType fonts; it works with other TrueType fonts too.
  Read the manual pages and the documentation for further information. For
  compilation you also need the FreeType 1 package:

    ftp://ftp.freetype.org/pub/freetype/unstable/freetype-current.tar.gz

. The font editor `fontforge' (available from http://fontforge.sf.net) is
  capable of generating Type 1 subfonts as needed by CJK from other formats
  like TTF, OTF or CID (using the subfont definition files from ttf2pk).
  Such subfonts should be usable by virtually all platforms.

  (Funnnily, fontforge uses the `.sfd' extension also for saving font files
  it creates.)

  Although fontforge needs the X Window System, it can be compiled without a
  graphical interface, using a scripting language to control font
  conversion. The directory `utils/subfonts' of the CJK package contains
  useful scripts for manipulating subfonts.

. It is recommended to add all CJK fonts which are converted to the PK font
  format (either with hbf2gf or ttf2pk) to the file special.map: Assuming
  that your PK fonts should be generated in

    $TEXMF/fonts/pk/modeless/gb2312/gsfs14/

  the proper entries would be

    gsfs1401  gb2312  gsfs14
    gsfs1402  gs2312  gsfs14
    ...

. Compile the small preprocessors in the utils subdirectories with

    cc -O -s -o bg5conv bg5conv.c
    cc -O -s -o sjisconv sjisconv.c
    cc -O -s -o cefconv cefconv.c
    cc -O -s -o cef5conv cef5conv.c
    cc -O -s -o cefsconv cefsconv.c
    cc -O -s -o extconv extconv.c

  and move them into TeX's bin directory (together with the shell scripts)
  or modify the PATH environment variable appropriately. (`cc' can be any C
  compiler.)

  The script files `...latex' make the use of these programs transparent.

. Move the man pages into your man1 directory tree.

. If you want to use Mule, emacs, or XEmacs together with the CJK package,
  you should install cjk-enc.el (in utils/lisp). See cjk-enc.txt for
  documentation. Choose the correct cjk-enc.el version---note that the Mule
  version has limited capabilities compared to the Emacs version.

  Move cjk-enc.el to a place which is searched by Mule (e.g.,
  /usr/local/lib/mule/site-lisp) and put the following line into your emacs
  file:

    (load-library "cjk-enc")

  The default directory for emacs is /usr/local/share/emacs/site-lisp.

  Note that you don't need cjk-enc.el in case you are editing UTF-8 encoded
  files only.

. If you mainly write Chinese or Japanese with Emacs or Mule, consider the
  use of cjktilde.el (in utils/lisp). This file contains a minor mode which
  exchanges the tilde key with the space key. See the documentation of
  \CJKtilde in CJK.txt for the reasons to use `~' in most cases instead of
  a space character.

  To install, move cjktilde.el to a place which is searched by Emacs or Mule
  (e.g., /usr/local/share/emacs/site-lisp) and put the following line into
  your .emacs file:

    (load-library "cjktilde")

  To toggle the CJK tilde mode say

    M-x cjk-tilde-mode

  You can then assign cjk-tilde-mode to a key, e.g., shift-insert.

. If you use AUCTeX you can try cjkspace.el instead of cjktilde.el; it works
  in a similar (but not identical) way and is special to LaTeX buffers. Move
  the file to the local lisp directory and put the following lines into your
  .emacs file:

    (autoload 'CJK-insert-space "cjkspace"
      "Insert tildes appropriately in CJK document." t)
    (defun my-LaTeX-mode-hook ()
      "My personal key definitions for LaTeX mode."
      (define-key LaTeX-mode-map " " 'CJK-insert-space))
    (add-hook 'LaTeX-mode-hook 'my-LaTeX-mode-hook)

  Please read the documentation in the file cjkspace.el .

. For Thai support please follow the instructions given in `thaifont.txt'.


DOS and OS/2 (emTeX)
--------------------

web2c has been ported to MS-DOS. If you use this (which I recommend), follow
the instructions above.

. Note that some Unix specific shell scripts and other files have names
  longer than 8 characters. You don't need them. Some of the TeX input files
  have lower and uppercase characters in its filenames, but none of the
  filenames collide under DOS.

. Move the `texinput' directory tree to a place where TeX scans for input
  files (and rename it to `cjk' or something else). Note that its
  subdirectories are specific to encoding schemes. emTeX allows for
  recursively scanned search paths, thus retaining the directory tree is
  possible.

  Example:

    CJK files:      c:\emtex\texinput\cjk\...
    environment:    set emtexdir=c:\emtex
                    set texinput=%emtexdir%\texinput!!

  See contrib/wadalab/DNP.txt for the Japanese Wadalab fonts.

. [In case you plan to use only outline fonts (PFB, TTF) you can omit
   this step.]

  Compile hbf2gf. You need GNU make and either the emx (DOS and OS/2) or
  the djgpp (DOS and Windows) compiler.

  Say `make -f Makefile.gnu' to see the possible options; more info can be
  found in hbf2gf.txt .

. Compile the utility programs.

    cc -O -s -o bg5conv bg5conv.c
    cc -O -s -o sjisconv sjisconv.c
    cc -O -s -o cefconv cefconv.c
    cc -O -s -o cef5conv cef5conv.c
    cc -O -s -o cefsconv cefsconv.c
    cc -O -s -o extconv extconv.c

. Move the various BAT files (for DOS) and/or the CMD REXX scripts (for
  OS/2) into a directory in the path (e.g., c:\emtex\bin).

. Edit the FD files of your encoding(s) to specify the fonts you have. An
  explanation of the additional size commands CJK provides can be found in
  fonts.txt .

  Note: Most FD example files from the CJK package are set up for PS fonts
  from the TeXLive distribution.

  If you use the CJK font packages (see below) no changes are needed.

. [In case you plan to use only outline fonts (PFB, TTF) you can omit this
   step.]

  If necessary, create TFM (and PK) files from CJK bitmaps with hbf2gf
  (found in utils\hbf2gf). See hbf2gf.txt and the documentation of the
  source file (hbf2gf.dvi) for explanation. Usually it is sufficient to let
  hbf2gf create a complete set of TFM files; PK fonts are then created on
  demand (this is done with the dvidrv.btm shell script of the CJK package).

  You need 4DOS or 4OS/2 (these are shareware replacements for command.com)
  to run dvidrv.btm.

  dvidrv.btm should also work with Take Command/16, Take Command/32, or Take
  Command for OS/2.

  The CJK font packages already contain TFM (and VF) files (arranged for the
  (new) TDS directory structure; unpack the font packages in the root
  directory with

    gzip -d CJK_font_archive.tgz
    tar xvf CJK_font_archive.tar

  Rearrange the directory structure as suggested below (to make the file
  search mechanism of emTeX faster) and modify the appropriate environment
  variables to include the additional directories. The same holds for the
  CJK bitmap fonts, its HBF header files and the hbf2gf configuration files.

  [Note: Binaries for the gzip and tar archive programs can be found on CTAN
   in the `utils' subdirectory.]

  Example:

      jfs56.tar.gz (should be ftp'ed as jfs56.tgz if you work under DOS
                    since two dots are not allowed)

    suggested final directory structure (after unpacking and rearranging):

      c:\texmf\fonts\tfm\gsfs1401.tfm ...
      c:\texmf\hbf2gf\gsfs14.cfg
      c:\texmf\fonts\hbf\gb2312\jfs56\jfs56.a ...
    [ c:\texmf\fonts\pk\modeless\XXXdpi\gsfs1401.pk ... ]

    Add these lines to the end of autoexec.bat:

      set texmfdir=c:\texmf
      set cjkpk=%texmfdir%\fonts\pk
      set textfm=%textfm%;%texmfdir%\fonts\tfm

    Under OS/2, add similar lines (but with expanded pathnames) to the end
    of config.sys:

      set texmfdir=c:\texmf
      set cjkpk=c:\texmf\fonts\pk
      set textfm=<your old textfm path>;c:\texmf\fonts\tfm

    Changes in gsfs14.cfg:

      pk_directory  $texmfdir\fonts\pk\modeless\432dpi\
      tfm_directory $texmfdir\fonts\tfm\

    Changes in dvidrv.btm:

      set pkdir=%texmfdir%\fonts\pk
      set ttfcfg=%texmfdir%\ttf2pk
      set hbfcfg=%texmfdir%\hbf2gf

      set pre_dpi=
      set post_dpi=dpi

    Changes in a dvi driver configuration file (.cnf) for emTeX:

      +font-files:{<your old pk path>,$texmfdir:fonts\modeless}\@Rrdpi\@f.pk

. Free Chinese TrueType fonts (for both simplified and traditiional Chinese)
  with a license similar to the GPL can be found on
  ftp://ftp.gnu.org/gnu/nongnu and its mirrors worldwide. You might also
  search websites of companies offering WWW browser; they often come with
  CJK language packs which contain CJK TrueType fonts.

  Please note that many CJK TrueType fonts only have a Unicode mapping
  table. You should use the SFD files from the ttf2pk package starting with
  the letter `U' (e.g., UKS.sfd) which maps Unicode fonts to language
  specific encoded subfonts as needed by the CJK package.

  The ttf2pk package can be found in the contrib/ttf2pk directory of

    ftp://ftp.freetype.org/
            freetype/unstable/freetype1-contrib-current.tar.gz

  contains the two programs ttf2tfm and ttf2pk for converting TrueType fonts
  into TFM and PK fonts, respectively. By the way, this package is not
  restricted to CJK TrueType fonts; it works with other TrueType fonts too.
  Read the manual pages and the documentation for further information. For
  compilation you also need the FreeType 1 package:

    ftp://ftp.freetype.org/pub/freetype/unstable/freetype-current.tar.gz

. The font editor `fontforge' (available from http://fontforge.sf.net) is
  capable to generate Type 1 subfonts as needed by CJK from other formats
  like TTF, OTF or CID (using the subfont definition files from ttf2pk).
  Such subfonts should be usable by virtually all platforms.

  (Funnnily, fontforge uses the `.sfd' extension also for saving font files
  it creates.)

  Although fontforge needs the X Window System, it can be compiled without a
  graphical interface, using a scripting language to control font
  conversion. The directory `utils/subfonts' of the CJK package contains
  useful scripts for manipulating subfonts.

. You find the some standard Hangul PK fonts for 300dpi (cx) and 600dpi
  (ljfour) resolution in the following archives:

    han.300.tar.gz
    han1.300.tar.gz
    han.600.tar.gz
    han1.600.tar.gz
    han.tfmvf.tar.gz
    han1.tfmvf.tar.gz

  It is necessary to rearrange not only the directory structure but the
  names of the dpi directories too: The TeX directory standards specifies
  `dpiXXX', but emTeX provides by default `XXXdpi'.

  The final locations of the packages' files should be

    c:\texmf\fonts\tfm\
    c:\texmf\fonts\vf\
    c:\texmf\fonts\pk\{cx,ljfour}\XXXdpi\

  Additionally to the above example you should add this to the end of
  autoexec.bat:

    set cjkvf=%texmfdir%\fonts\vf

  or config.sys for OS/2:

    set cjkvf=c:\texmf\fonts\vf

  Assuming that you use the 300dpi Hangul PK fonts (for a cx printer) you
  should do the following changes in your dvi driver configuration file
  (suffix `.cnf') for emTeX (still continuing the above example):

    +font-files:{<your old pk path>,$texmfdir:fonts\{modeless,cx}}\@Rrdpi\@f.pk
    +virtual-fonts:{<your old vf path>,$texmfdir:fonts}\@f.vf

. For Thai support please follow the instructions given in `thaifont.txt'.


Other systems
-------------

Recent versions of CJK have only been tested with web2c; nevertheless, it
should run on other systems too:

  The font editor `fontforge' (available from http://fontforge.sf.net) is
  capable to generate Type 1 subfonts as needed by CJK from other formats
  like TTF, OTF or CID (using the subfont definition files from ttf2pk).
  Such subfonts should be usable by virtually all platforms.

  (Funnnily, fontforge uses the `.sfd' extension also for saving font files
  it creates.)

  Although fontforge needs the X Window System, it can be compiled without a
  graphical interface, using a scripting language to control font
  conversion. The directory `utils/subfonts' of the CJK package contains
  useful scripts for manipulating subfonts.

  If no outline fonts are available and you have to use HBF fonts, try to
  compile hbf2gf. Since it is written in ANSI C it should be fairly portable
  (if patches are needed please send them to the author; most likely you
  have to modify the file operating routines). If this fails it is necessary
  to build the various PK fonts on a different machine. It has been reported
  that older GNU compilers on the NeXT have difficulties with `%i'
  formatting parameters in the HBF API (hbf.c): replace all occurrences of
  `%i' with `%d'.

  If there exists an equivalent to mktexpk (or dvidrv.btm), try to modify it
  similar to CJK's changes so that CJK fonts can be created on the fly. If
  this fails you can only use precompiled sets of CJK fonts (this is, using
  PK fonts generated on another platform).

  The rest should be rather trivial for the experienced user; again, please
  write the author if you have successfully installed the package and send a
  report how to install.


How to get CJK and related software
-----------------------------------

. You find CJK and software related to TeX at the CTAN hosts (Comprehensive
  TeX Archive Network). These completely identical ftp servers (concerning
  TeX software) are

    ftp.dante.de    DANTE (Deutsche Anwendervereinigung fuer TeX)
                    Hamburg (Germany)
    ftp.tex.ac.uk   Cambridge University
                    Cambridge (England)
    ctan.tug.org    TUG (TeX Users Group)
                    Massachusetts (USA)

  You should use the nearest one, or even better, a local mirror of a CTAN
  host: The file `CTAN.sites' on CTAN contains a list.

  On CTAN, the CJK package itself is unpacked. To receive the complete
  package, go to the parent directory of CJK and say

    get CJK.zip

  or

    get CJK.tar.gz

  whatever is appropriate for your system.

  The CJK directory and all its subdirectories are sent to you in compressed
  form. Be aware that not all mirrors of CTAN sites support compression of
  directories.

. The documentation bundle of the CJK package is not unpackaged; download it
  as

    get cjk-4.8.5-doc.tar.gz

  or

    get cjk-4.8.5-doc.tar.gz cjkdoc.tgz

  whatever is appropriate for your system. It contains precompiled versions
  (in DVI, PDF, text format) of all documentation and example files.

. PostScript font packages with subfonts which can be directly used by the
  CJK package are already available on CTAN:

    traditional Chinese:
      fonts/arphic/bkai00mp-<version>.tar.gz
      fonts/arphic/bsmi00lp-<version>.tar.gz

    simplified Chinese:
      fonts/arphic/gbsn00lp-<version>.tar.gz
      fonts/arphic/gkai00mp-<version>.tar.gz

    Japanese:
      fonts/wadalab/gothic-0-13-<version>.tar.gz
      fonts/wadalab/maru-0-8-<version>.tar.gz
      fonts/wadalab/maru-1-8-<version>.tar.gz
      fonts/wadalab/mincho-0-12-<version>.tar.gz
      fonts/wadalab/mincho-0-8-<version>.tar.gz
      fonts/wadalab/mincho-1-8-<version>.tar.gz

    Korean:
      fonts/korean/HLaTeX/uhc-bom.tar.gz
      fonts/korean/HLaTeX/uhc-dinaru.tar.gz
      fonts/korean/HLaTeX/uhc-fonts.tar.gz
      fonts/korean/HLaTeX/uhc-gothic.tar.gz
      fonts/korean/HLaTeX/uhc-graphic.tar.gz
      fonts/korean/HLaTeX/uhc-gungseo.tar.gz
      fonts/korean/HLaTeX/uhc-jamo.tar.gz
      fonts/korean/HLaTeX/uhc-myoungjo.tar.gz
      fonts/korean/HLaTeX/uhc-pen.tar.gz
      fonts/korean/HLaTeX/uhc-pilgi.tar.gz
      fonts/korean/HLaTeX/uhc-pilgia.tar.gz
      fonts/korean/HLaTeX/uhc-shinmun.tar.gz
      fonts/korean/HLaTeX/uhc-taza.tar.gz
      fonts/korean/HLaTeX/uhc-vada.tar.gz
      fonts/korean/HLaTeX/uhc-yetgul.tar.gz

  You should consult the documentation and the font samplers of those
  packages (if available) for more informations.

. Mule 2.3 can be downloaded from this Japanese host:

    ftp://ftp.m17n.org/pub/mule/mule-2.3.tar.gz

  [Note: You need Mule 2.3 only for right-to-left scripts like Arabic or
   Hebrew which aren't yet supported in emacs. Otherwise, I strongly
   recommend to get FSF emacs 22 or newer, or XEmacs 21.1 or newer which is
   available from ftp.gnu.org (USA) and ftp.xemacs.org, respectively, and
   its many mirrors.]


---End of INSTALL---


==> cjk-4.8.5/utils/Bg5conv/bg5conv.1 <==
.\" man page for bg5conv
.\" Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
.\"
.\" This program is free software; you can redistribute it and/or modify
.\" it under the terms of the GNU General Public License as published by
.\" the Free Software Foundation; either version 2 of the License, or
.\" (at your option) any later version.
.\"
.\" This program is distributed in the hope that it will be useful,
.\" but WITHOUT ANY WARRANTY; without even the implied warranty of
.\" MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
.\" GNU General Public License for more details.
.\"
.\" You should have received a copy of the GNU General Public License
.\" along with this program in doc/COPYING; if not, write to the Free
.\" Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
.\" MA 02110-1301 USA
.
.TH BG5CONV 1 16-Oct-2021 "CJK Version 4.8.5"
.
.\" ====
.\" ==== macro definitions
.\" ====
.
.\" here we define \TeX for troff and nroff
.if t .ds TX \fRT\\h'-0.1667m'\\v'0.20v'E\\v'-0.20v'\\h'-0.125m'X\fP
.if n .ds TX TeX
.
.\" and here the same for \LaTeX
.if t \{\
.ie '\*(.T'dvi' \
.ds LX \fRL\h'-0.36m'\v'-0.15v'\s-3A\s0\h'-0.15m'\v'0.15v'\fP\*(TX
.el .ds LX \fRL\h'-0.36m'\v'-0.22v'\s-2A\s0\h'-0.15m'\v'0.22v'\fP\*(TX
.\}
.if n .ds LX LaTeX
.
.\" \LaTeXe
.\" note that we need \vareps for TeX instead of \eps which can only be
.\" accessed with the \N escape sequence (in the Math Italic font)
.if t \{\
.ie '\*(.T'dvi' .ds LE \*(LX\h'0.15m'2\v'0.20v'\f(MI\N'34'\fP\v'-0.20v'
.el .ds LE \*(LX\h'0.15m'2\v'0.20v'\(*e\v'-0.20v'
.\}
.if n .ds LE LaTeX\ 2e
.
.\" a typewriter font
.if t \{\
.de C
\fC\\$1\fP\\$2
..
.\}
.if n \{\
.de C
\\$1\\$2
..
.\}
.
.\" ====
.\" ==== end of macro definitions
.\" ====
.
.
.
.SH NAME
bg5conv \- convert a TeX document in Big\ 5 encoding into `preprocessed'
form.
.
.
.SH SYNOPSIS
.B bg5conv
<
.I infile
>
.I outfile
.
.
.SH DESCRIPTION
Big\ 5 encoding for traditional Chinese uses the characters
.C { ,
.C } ,
and
.C \e
which have special meanings in \*(TX
documents.
.PP
After processing a \*(LE
document which contains Big\ 5 characters with
.B bg5conv
you need not care about these special characters.
.PP
This filter is part of the
.B CJK
macro package for \*(LE.
.
.
.SH "SEE ALSO"
.BR \%sjisconv (1),
.BR \%cefconv (1),
.BR cef5conv (1),
.BR \%cefsconv (1),
.BR \%extconv (1),
.br
the
.B CJK
documentation files.
.
.
.SH AUTHOR
Werner Lemberg
.C <wl@gnu.org>


==> cjk-4.8.5/utils/Bg5conv/bg5latex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

bg5conv < "$tex" > "$aux" && eval latex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/Bg5conv/bg5pdflatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] pdflatex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

bg5conv < "$tex" > "$aux" && eval pdflatex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/CEFconv/cef5conv.1 <==
.\" man page for cef5conv
.\" Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
.\"
.\" This program is free software; you can redistribute it and/or modify
.\" it under the terms of the GNU General Public License as published by
.\" the Free Software Foundation; either version 2 of the License, or
.\" (at your option) any later version.
.\"
.\" This program is distributed in the hope that it will be useful,
.\" but WITHOUT ANY WARRANTY; without even the implied warranty of
.\" MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
.\" GNU General Public License for more details.
.\"
.\" You should have received a copy of the GNU General Public License
.\" along with this program in doc/COPYING; if not, write to the Free
.\" Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
.\" MA 02110-1301 USA
.
.TH CEF5CONV 1 16-Oct-2021 "CJK Version 4.8.5"
.
.\" ====
.\" ==== macro definitions
.\" ====
.
.\" here we define \TeX for troff and nroff
.if t .ds TX \fRT\\h'-0.1667m'\\v'0.20v'E\\v'-0.20v'\\h'-0.125m'X\fP
.if n .ds TX TeX
.
.\" and here the same for \LaTeX
.if t \{\
.ie '\*(.T'dvi' \
.ds LX \fRL\h'-0.36m'\v'-0.15v'\s-3A\s0\h'-0.15m'\v'0.15v'\fP\*(TX
.el .ds LX \fRL\h'-0.36m'\v'-0.22v'\s-2A\s0\h'-0.15m'\v'0.22v'\fP\*(TX
.\}
.if n .ds LX LaTeX
.
.\" \LaTeXe
.\" note that we need \vareps for TeX instead of \eps which can only be
.\" accessed with the \N escape sequence (in the Math Italic font)
.if t \{\
.ie '\*(.T'dvi' .ds LE \*(LX\h'0.15m'2\v'0.20v'\f(MI\N'34'\fP\v'-0.20v'
.el .ds LE \*(LX\h'0.15m'2\v'0.20v'\(*e\v'-0.20v'
.\}
.if n .ds LE LaTeX\ 2e
.
.\" a typewriter font
.if t \{\
.de C
\fC\\$1\fP
..
.\}
.if n \{\
.de C
\\$1
..
.\}
.
.\" ====
.\" ==== end of macro definitions
.\" ====
.
.
.
.SH NAME
cef5conv \- convert a TeX document in Big\ 5 encoding containing CEF macros
into `preprocessed' form.
.
.
.SH SYNOPSIS
.B cef5conv
<
.I infile
>
.I outfile
.
.
.SH DESCRIPTION
The
.B Chinese Encoding Framework
.RB ( CEF )
developed by Christian Wittern
.C <cwittern@conline.central.de>
makes it possible to include CJK characters in various encodings using the
SGML macros
.B &CX-aabb;
for Big\ 5 and CNS encoding and
.B &U-aabb;
for Unicode
.RB ( X
denotes a number between 0 and 7; 0 represents Big\ 5 encoding, 1-7 CNS
encoding planes 1-7.
.B aabb
is either a decimal or hexadecimal number).
.PP
.B cef5conv
converts the CEF macros of a Big\ 5 encoded document together with the Big\
5 encoding itself into a form which can directly processed with \*(LE.
It is identical to
.IP
.B bg5conv
<
.I infile
|
.B cefconv
>
.I outfile
.PP
This filter is part of the
.B CJK
macro package for \*(LE.
.
.
.SH "SEE ALSO"
.BR \%sjisconv (1),
.BR bg5conv (1),
.BR \%cefconv (1),
.BR \%cefsconv (1),
.BR \%extconv (1),
.br
the
.B CJK
documentation files.
.
.
.SH AUTHOR
Werner Lemberg
.C <wl@gnu.org>


==> cjk-4.8.5/utils/CEFconv/cef5latex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

cef5conv < "$tex" > "$aux" && eval latex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/CEFconv/cef5pdflatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] pdflatex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

cef5conv < "$tex" > "$aux" && eval pdflatex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/CEFconv/cefconv.1 <==
.\" man page for cefconv
.\" Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
.\"
.\" This program is free software; you can redistribute it and/or modify
.\" it under the terms of the GNU General Public License as published by
.\" the Free Software Foundation; either version 2 of the License, or
.\" (at your option) any later version.
.\"
.\" This program is distributed in the hope that it will be useful,
.\" but WITHOUT ANY WARRANTY; without even the implied warranty of
.\" MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
.\" GNU General Public License for more details.
.\"
.\" You should have received a copy of the GNU General Public License
.\" along with this program in doc/COPYING; if not, write to the Free
.\" Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
.\" MA 02110-1301 USA
.
.TH CEFCONV 1 16-Oct-2021 "CJK Version 4.8.5"
.
.\" ====
.\" ==== macro definitions
.\" ====
.
.\" here we define \TeX for troff and nroff
.if t .ds TX \fRT\\h'-0.1667m'\\v'0.20v'E\\v'-0.20v'\\h'-0.125m'X\fP
.if n .ds TX TeX
.
.\" and here the same for \LaTeX
.if t \{\
.ie '\*(.T'dvi' \
.ds LX \fRL\h'-0.36m'\v'-0.15v'\s-3A\s0\h'-0.15m'\v'0.15v'\fP\*(TX
.el .ds LX \fRL\h'-0.36m'\v'-0.22v'\s-2A\s0\h'-0.15m'\v'0.22v'\fP\*(TX
.\}
.if n .ds LX LaTeX
.
.\" \LaTeXe
.\" note that we need \vareps for TeX instead of \eps which can only be
.\" accessed with the \N escape sequence (in the Math Italic font)
.if t \{\
.ie '\*(.T'dvi' .ds LE \*(LX\h'0.15m'2\v'0.20v'\f(MI\N'34'\fP\v'-0.20v'
.el .ds LE \*(LX\h'0.15m'2\v'0.20v'\(*e\v'-0.20v'
.\}
.if n .ds LE LaTeX\ 2e
.
.\" a typewriter font
.if t \{\
.de C
\fC\\$1\fP
..
.\}
.if n \{\
.de C
\\$1
..
.\}
.
.\" ====
.\" ==== end of macro definitions
.\" ====
.
.
.
.SH NAME
cefconv \- convert a TeX document containing CEF macros into `preprocessed'
form.
.
.
.SH SYNOPSIS
.B cefconv
<
.I infile
>
.I outfile
.
.
.SH DESCRIPTION
The
.B Chinese Encoding Framework
.RB ( CEF )
developed by Christian Wittern
.C <cwittern@conline.central.de>
makes it possible to include CJK characters in various encodings using the
SGML macros
.B &CX-aabb;
for Big\ 5 and CNS encoding and
.B &U-aabb;
for Unicode
.RB ( X
denotes a number between 0 and 7; 0 represents Big\ 5 encoding, 1-7 CNS
encoding planes 1-7.
.B aabb
is either a decimal or hexadecimal number)
.PP
.B \%cefconv
converts the CEF macros into a form which can directly processed with \*(LE.
.PP
This filter is part of the
.B CJK
macro package for \*(LE.
.
.
.SH "SEE ALSO"
.BR \%sjisconv (1),
.BR bg5conv (1),
.BR cef5conv (1),
.BR \%cefsconv (1),
.BR \%extconv (1),
.br
the
.B CJK
documentation files.
.
.
.SH AUTHOR
Werner Lemberg
.C <wl@gnu.org>


==> cjk-4.8.5/utils/CEFconv/ceflatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

cefconv < "$tex" > "$aux" && eval latex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/CEFconv/cefpdflatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] pdflatex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

cefconv < "$tex" > "$aux" && eval pdflatex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/CEFconv/cefsconv.1 <==
.\" man page for cefsconv
.\" Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
.\"
.\" This program is free software; you can redistribute it and/or modify
.\" it under the terms of the GNU General Public License as published by
.\" the Free Software Foundation; either version 2 of the License, or
.\" (at your option) any later version.
.\"
.\" This program is distributed in the hope that it will be useful,
.\" but WITHOUT ANY WARRANTY; without even the implied warranty of
.\" MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
.\" GNU General Public License for more details.
.\"
.\" You should have received a copy of the GNU General Public License
.\" along with this program in doc/COPYING; if not, write to the Free
.\" Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
.\" MA 02110-1301 USA
.
.TH CEFSCONV 1 16-Oct-2021 "CJK Version 4.8.5"
.
.\" ====
.\" ==== macro definitions
.\" ====
.
.\" here we define \TeX for troff and nroff
.if t .ds TX \fRT\\h'-0.1667m'\\v'0.20v'E\\v'-0.20v'\\h'-0.125m'X\fP
.if n .ds TX TeX
.
.\" and here the same for \LaTeX
.if t \{\
.ie '\*(.T'dvi' \
.ds LX \fRL\h'-0.36m'\v'-0.15v'\s-3A\s0\h'-0.15m'\v'0.15v'\fP\*(TX
.el .ds LX \fRL\h'-0.36m'\v'-0.22v'\s-2A\s0\h'-0.15m'\v'0.22v'\fP\*(TX
.\}
.if n .ds LX LaTeX
.
.\" \LaTeXe
.\" note that we need \vareps for TeX instead of \eps which can only be
.\" accessed with the \N escape sequence (in the Math Italic font)
.if t \{\
.ie '\*(.T'dvi' .ds LE \*(LX\h'0.15m'2\v'0.20v'\f(MI\N'34'\fP\v'-0.20v'
.el .ds LE \*(LX\h'0.15m'2\v'0.20v'\(*e\v'-0.20v'
.\}
.if n .ds LE LaTeX\ 2e
.
.\" a typewriter font
.if t \{\
.de C
\fC\\$1\fP
..
.\}
.if n \{\
.de C
\\$1
..
.\}
.
.\" ====
.\" ==== end of macro definitions
.\" ====
.
.
.
.SH NAME
cefsconv \- convert a TeX document in SJIS encoding containing CEF macros
into `preprocessed' form.
.
.
.SH SYNOPSIS
.B cefsconv
<
.I infile
>
.I outfile
.
.
.SH DESCRIPTION
The
.B Chinese Encoding Framework
.RB ( CEF )
developed by Christian Wittern
.C <cwittern@conline.central.de>
makes it possible to include CJK characters in various encodings using the
SGML macros
.B &CX-aabb;
for Big\ 5 and CNS encoding and
.B &U-aabb;
for Unicode
.RB ( X
denotes a number between 0 and 7; 0 represents Big\ 5 encoding, 1-7 CNS
encoding planes 1-7.
.B aabb
is either a decimal or hexadecimal number).
.PP
.B \%cefsconv
converts the CEF macros of a SJIS encoded document together with the SJIS
encoding itself into a form which can directly processed with \*(LE.
It is identical to
.IP
.B sjisconv
<
.I infile
|
.B cefconv
>
.I outfile
.PP
This filter is part of the
.B CJK
macro package for \*(LE.
.
.
.SH "SEE ALSO"
.BR \%sjisconv (1),
.BR bg5conv (1),
.BR \%cefconv (1),
.BR cef5conv (1),
.BR \%extconv (1),
.br
the
.B CJK
documentation files.
.
.
.SH AUTHOR
Werner Lemberg
.C <wl@gnu.org>


==> cjk-4.8.5/utils/CEFconv/cefslatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

cefsconv < "$tex" > "$aux" && eval latex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/CEFconv/cefspdflatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

cefsconv < "$tex" > "$aux" && eval pdflatex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/SJISconv/sjisconv.1 <==
.\" man page for sjisconv
.\" Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
.\"
.\" This program is free software; you can redistribute it and/or modify
.\" it under the terms of the GNU General Public License as published by
.\" the Free Software Foundation; either version 2 of the License, or
.\" (at your option) any later version.
.\"
.\" This program is distributed in the hope that it will be useful,
.\" but WITHOUT ANY WARRANTY; without even the implied warranty of
.\" MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
.\" GNU General Public License for more details.
.\"
.\" You should have received a copy of the GNU General Public License
.\" along with this program in doc/COPYING; if not, write to the Free
.\" Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
.\" MA 02110-1301 USA
.
.TH SJISCONV 1 16-Oct-2021 "CJK Version 4.8.5"
.
.\" ====
.\" ==== macro definitions
.\" ====
.
.\" here we define \TeX for troff and nroff
.if t .ds TX \fRT\\h'-0.1667m'\\v'0.20v'E\\v'-0.20v'\\h'-0.125m'X\fP
.if n .ds TX TeX
.
.\" and here the same for \LaTeX
.if t \{\
.ie '\*(.T'dvi' \
.ds LX \fRL\h'-0.36m'\v'-0.15v'\s-3A\s0\h'-0.15m'\v'0.15v'\fP\*(TX
.el .ds LX \fRL\h'-0.36m'\v'-0.22v'\s-2A\s0\h'-0.15m'\v'0.22v'\fP\*(TX
.\}
.if n .ds LX LaTeX
.
.\" \LaTeXe
.\" note that we need \vareps for TeX instead of \eps which can only be
.\" accessed with the \N escape sequence (in the Math Italic font)
.if t \{\
.ie '\*(.T'dvi' .ds LE \*(LX\h'0.15m'2\v'0.20v'\f(MI\N'34'\fP\v'-0.20v'
.el .ds LE \*(LX\h'0.15m'2\v'0.20v'\(*e\v'-0.20v'
.\}
.if n .ds LE LaTeX\ 2e
.
.\" a typewriter font
.if t \{\
.de C
\fC\\$1\fP\\$2
..
.\}
.if n \{\
.de C
\\$1\\$2
..
.\}
.
.\" ====
.\" ==== end of macro definitions
.\" ====
.
.
.
.SH NAME
sjisconv \- convert a TeX document in SJIS encoding into `preprocessed'
form.
.
.
.SH SYNOPSIS
.B sjisconv
<
.I infile
>
.I outfile
.
.
.SH DESCRIPTION
SJIS encoding for Japanese uses the characters
.C { ,
.C } ,
and
.C \e
which have special meanings in \*(TX
documents.
.PP
After processing a \*(LE
document which contains SJIS characters with
.B \%sjisconv
you need not care about these special characters.
.PP
This filter is part of the
.B CJK
macro package for \*(LE.
.
.
.SH "SEE ALSO"
.BR bg5conv (1),
.BR \%cefconv (1),
.BR cef5conv (1),
.BR \%cefsconv (1),
.BR \%extconv (1),
.br
the
.B CJK
documentation files.
.
.
.SH AUTHOR
Werner Lemberg
.C <wl@gnu.org>


==> cjk-4.8.5/utils/SJISconv/sjislatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

sjisconv < "$tex" > "$aux" && eval latex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/SJISconv/sjispdflatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

sjisconv < "$tex" > "$aux" && eval pdflatex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/extconv/bg5+latex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

extconv < "$tex" > "$aux" && eval latex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/extconv/bg5+pdflatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] pdflatex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

extconv < "$tex" > "$aux" && eval pdflatex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/extconv/extconv.1 <==
.\" man page for bg5conv
.\"
.\" Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
.\"
.\" This program is free software; you can redistribute it and/or modify
.\" it under the terms of the GNU General Public License as published by
.\" the Free Software Foundation; either version 2 of the License, or
.\" (at your option) any later version.
.\"
.\" This program is distributed in the hope that it will be useful,
.\" but WITHOUT ANY WARRANTY; without even the implied warranty of
.\" MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
.\" GNU General Public License for more details.
.\"
.\" You should have received a copy of the GNU General Public License
.\" along with this program in doc/COPYING; if not, write to the Free
.\" Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
.\" MA 02110-1301 USA
.
.TH EXTCONV 1 16-Oct-2021 "CJK Version 4.8.5"
.
.\" ====
.\" ==== macro definitions
.\" ====
.
.\" here we define \TeX for troff and nroff
.if t .ds TX \fRT\\h'-0.1667m'\\v'0.20v'E\\v'-0.20v'\\h'-0.125m'X\fP
.if n .ds TX TeX
.
.\" and here the same for \LaTeX
.if t \{\
.ie '\*(.T'dvi' \
.ds LX \fRL\h'-0.36m'\v'-0.15v'\s-3A\s0\h'-0.15m'\v'0.15v'\fP\*(TX
.el .ds LX \fRL\h'-0.36m'\v'-0.22v'\s-2A\s0\h'-0.15m'\v'0.22v'\fP\*(TX
.\}
.if n .ds LX LaTeX
.
.\" \LaTeXe
.\" note that we need \vareps for TeX instead of \eps which can only be
.\" accessed with the \N escape sequence (in the Math Italic font)
.if t \{\
.ie '\*(.T'dvi' .ds LE \*(LX\h'0.15m'2\v'0.20v'\f(MI\N'34'\fP\v'-0.20v'
.el .ds LE \*(LX\h'0.15m'2\v'0.20v'\(*e\v'-0.20v'
.\}
.if n .ds LE LaTeX\ 2e
.
.\" a typewriter font
.if t \{\
.de C
\fC\\$1\fP\\$2
..
.\}
.if n \{\
.de C
\\$1\\$2
..
.\}
.
.\" ====
.\" ==== end of macro definitions
.\" ====
.
.
.
.SH NAME
extconv \- convert a TeX document in either Big\ 5+ or GBK encoding into
`preprocessed' form.
.
.
.SH SYNOPSIS
.B extconv
<
.I infile
>
.I outfile
.
.
.SH DESCRIPTION
Big\ 5+ and GBK encodings use the characters
.C { ,
.C } ,
and
.C \e
which have special meanings in \*(TX
documents.
.PP
After processing a \*(LE
document which contains such characters with
.B \%extconv
you need not care about these special characters.
.PP
This filter is part of the
.B CJK
macro package for \*(LE.
.
.
.SH "SEE ALSO"
.BR bg5conv (1),
.BR \%sjisconv (1),
.BR \%cefconv (1),
.BR cef5conv (1),
.BR \%cefsconv (1),
.br
the
.B CJK
documentation files.
.
.
.SH AUTHOR
Werner Lemberg
.C <wl@gnu.org>


==> cjk-4.8.5/utils/extconv/gbklatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] latex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

extconv < "$tex" > "$aux" && eval latex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/extconv/gbkpdflatex <==
#! /bin/sh

# Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
#
# This program is free software; you can redistribute it and/or modify
# it under the terms of the GNU General Public License as published by
# the Free Software Foundation; either version 2 of the License, or
# (at your option) any later version.
#
# This program is distributed in the hope that it will be useful,
# but WITHOUT ANY WARRANTY; without even the implied warranty of
# MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
# GNU General Public License for more details.
#
# You should have received a copy of the GNU General Public License
# along with this program in doc/COPYING; if not, write to the Free
# Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
# MA 02110-1301 USA

n=1
argv=

# get last argument
while test 1 -lt $#; do
  eval argv$n=\$1
  argv="$argv \"\$argv$n\""
  n=`expr $n + 1`
  shift
done

# replace extension with .cjk or append .cjk if there is no extension
tex=$1
case $tex in
""|*.cjk)
  echo >&2 "Usage: $0 [options] pdflatex-file"
  exit 1;;
*)
  aux=`expr "X$tex" : 'X\(.*\)\.[^/]*$' \| "X$tex" : 'X\(.*\)'`.cjk;;
esac

extconv < "$tex" > "$aux" && eval pdflatex "$argv" "\$aux"

# EOF


==> cjk-4.8.5/utils/hbf2gf/configure <==
#! /bin/sh
# Guess values for system-dependent variables and create Makefiles.
# Generated by GNU Autoconf 2.71.
#
#
# Copyright (C) 1992-1996, 1998-2017, 2020-2021 Free Software Foundation,
# Inc.
#
#
# This configure script is free software; the Free Software Foundation
# gives unlimited permission to copy, distribute and modify it.
## -------------------- ##
## M4sh Initialization. ##
## -------------------- ##

# Be more Bourne compatible
DUALCASE=1; export DUALCASE # for MKS sh
as_nop=:
if test ${ZSH_VERSION+y} && (emulate sh) >/dev/null 2>&1
then :
  emulate sh
  NULLCMD=:
  # Pre-4.2 versions of Zsh do word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else $as_nop
  case `(set -o) 2>/dev/null` in #(
  *posix*) :
    set -o posix ;; #(
  *) :
     ;;
esac
fi



# Reset variables that may have inherited troublesome values from
# the environment.

# IFS needs to be set, to space, tab, and newline, in precisely that order.
# (If _AS_PATH_WALK were called with IFS unset, it would have the
# side effect of setting IFS to empty, thus disabling word splitting.)
# Quoting is to prevent editors from complaining about space-tab.
as_nl='
'
export as_nl
IFS=" ""	$as_nl"

PS1='$ '
PS2='> '
PS4='+ '

# Ensure predictable behavior from utilities with locale-dependent output.
LC_ALL=C
export LC_ALL
LANGUAGE=C
export LANGUAGE

# We cannot yet rely on "unset" to work, but we need these variables
# to be unset--not just set to an empty or harmless value--now, to
# avoid bugs in old shells (e.g. pre-3.0 UWIN ksh).  This construct
# also avoids known problems related to "unset" and subshell syntax
# in other old shells (e.g. bash 2.01 and pdksh 5.2.14).
for as_var in BASH_ENV ENV MAIL MAILPATH CDPATH
do eval test \${$as_var+y} \
  && ( (unset $as_var) || exit 1) >/dev/null 2>&1 && unset $as_var || :
done

# Ensure that fds 0, 1, and 2 are open.
if (exec 3>&0) 2>/dev/null; then :; else exec 0</dev/null; fi
if (exec 3>&1) 2>/dev/null; then :; else exec 1>/dev/null; fi
if (exec 3>&2)            ; then :; else exec 2>/dev/null; fi

# The user is always right.
if ${PATH_SEPARATOR+false} :; then
  PATH_SEPARATOR=:
  (PATH='/bin;/bin'; FPATH=$PATH; sh -c :) >/dev/null 2>&1 && {
    (PATH='/bin:/bin'; FPATH=$PATH; sh -c :) >/dev/null 2>&1 ||
      PATH_SEPARATOR=';'
  }
fi


# Find who we are.  Look in the path if we contain no directory separator.
as_myself=
case $0 in #((
  *[\\/]* ) as_myself=$0 ;;
  *) as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    test -r "$as_dir$0" && as_myself=$as_dir$0 && break
  done
IFS=$as_save_IFS

     ;;
esac
# We did not find ourselves, most probably we were run as `sh COMMAND'
# in which case we are not to be found in the path.
if test "x$as_myself" = x; then
  as_myself=$0
fi
if test ! -f "$as_myself"; then
  printf "%s\n" "$as_myself: error: cannot find myself; rerun with an absolute file name" >&2
  exit 1
fi


# Use a proper internal environment variable to ensure we don't fall
  # into an infinite loop, continuously re-executing ourselves.
  if test x"${_as_can_reexec}" != xno && test "x$CONFIG_SHELL" != x; then
    _as_can_reexec=no; export _as_can_reexec;
    # We cannot yet assume a decent shell, so we have to provide a
# neutralization value for shells without unset; and this also
# works around shells that cannot unset nonexistent variables.
# Preserve -v and -x to the replacement shell.
BASH_ENV=/dev/null
ENV=/dev/null
(unset BASH_ENV) >/dev/null 2>&1 && unset BASH_ENV ENV
case $- in # ((((
  *v*x* | *x*v* ) as_opts=-vx ;;
  *v* ) as_opts=-v ;;
  *x* ) as_opts=-x ;;
  * ) as_opts= ;;
esac
exec $CONFIG_SHELL $as_opts "$as_myself" ${1+"$@"}
# Admittedly, this is quite paranoid, since all the known shells bail
# out after a failed `exec'.
printf "%s\n" "$0: could not re-execute with $CONFIG_SHELL" >&2
exit 255
  fi
  # We don't want this to propagate to other subprocesses.
          { _as_can_reexec=; unset _as_can_reexec;}
if test "x$CONFIG_SHELL" = x; then
  as_bourne_compatible="as_nop=:
if test \${ZSH_VERSION+y} && (emulate sh) >/dev/null 2>&1
then :
  emulate sh
  NULLCMD=:
  # Pre-4.2 versions of Zsh do word splitting on \${1+\"\$@\"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '\${1+\"\$@\"}'='\"\$@\"'
  setopt NO_GLOB_SUBST
else \$as_nop
  case \`(set -o) 2>/dev/null\` in #(
  *posix*) :
    set -o posix ;; #(
  *) :
     ;;
esac
fi
"
  as_required="as_fn_return () { (exit \$1); }
as_fn_success () { as_fn_return 0; }
as_fn_failure () { as_fn_return 1; }
as_fn_ret_success () { return 0; }
as_fn_ret_failure () { return 1; }

exitcode=0
as_fn_success || { exitcode=1; echo as_fn_success failed.; }
as_fn_failure && { exitcode=1; echo as_fn_failure succeeded.; }
as_fn_ret_success || { exitcode=1; echo as_fn_ret_success failed.; }
as_fn_ret_failure && { exitcode=1; echo as_fn_ret_failure succeeded.; }
if ( set x; as_fn_ret_success y && test x = \"\$1\" )
then :

else \$as_nop
  exitcode=1; echo positional parameters were not saved.
fi
test x\$exitcode = x0 || exit 1
blah=\$(echo \$(echo blah))
test x\"\$blah\" = xblah || exit 1
test -x / || exit 1"
  as_suggested="  as_lineno_1=";as_suggested=$as_suggested$LINENO;as_suggested=$as_suggested" as_lineno_1a=\$LINENO
  as_lineno_2=";as_suggested=$as_suggested$LINENO;as_suggested=$as_suggested" as_lineno_2a=\$LINENO
  eval 'test \"x\$as_lineno_1'\$as_run'\" != \"x\$as_lineno_2'\$as_run'\" &&
  test \"x\`expr \$as_lineno_1'\$as_run' + 1\`\" = \"x\$as_lineno_2'\$as_run'\"' || exit 1"
  if (eval "$as_required") 2>/dev/null
then :
  as_have_required=yes
else $as_nop
  as_have_required=no
fi
  if test x$as_have_required = xyes && (eval "$as_suggested") 2>/dev/null
then :

else $as_nop
  as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
as_found=false
for as_dir in /bin$PATH_SEPARATOR/usr/bin$PATH_SEPARATOR$PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
  as_found=:
  case $as_dir in #(
	 /*)
	   for as_base in sh bash ksh sh5; do
	     # Try only shells that exist, to save several forks.
	     as_shell=$as_dir$as_base
	     if { test -f "$as_shell" || test -f "$as_shell.exe"; } &&
		    as_run=a "$as_shell" -c "$as_bourne_compatible""$as_required" 2>/dev/null
then :
  CONFIG_SHELL=$as_shell as_have_required=yes
		   if as_run=a "$as_shell" -c "$as_bourne_compatible""$as_suggested" 2>/dev/null
then :
  break 2
fi
fi
	   done;;
       esac
  as_found=false
done
IFS=$as_save_IFS
if $as_found
then :

else $as_nop
  if { test -f "$SHELL" || test -f "$SHELL.exe"; } &&
	      as_run=a "$SHELL" -c "$as_bourne_compatible""$as_required" 2>/dev/null
then :
  CONFIG_SHELL=$SHELL as_have_required=yes
fi
fi


      if test "x$CONFIG_SHELL" != x
then :
  export CONFIG_SHELL
             # We cannot yet assume a decent shell, so we have to provide a
# neutralization value for shells without unset; and this also
# works around shells that cannot unset nonexistent variables.
# Preserve -v and -x to the replacement shell.
BASH_ENV=/dev/null
ENV=/dev/null
(unset BASH_ENV) >/dev/null 2>&1 && unset BASH_ENV ENV
case $- in # ((((
  *v*x* | *x*v* ) as_opts=-vx ;;
  *v* ) as_opts=-v ;;
  *x* ) as_opts=-x ;;
  * ) as_opts= ;;
esac
exec $CONFIG_SHELL $as_opts "$as_myself" ${1+"$@"}
# Admittedly, this is quite paranoid, since all the known shells bail
# out after a failed `exec'.
printf "%s\n" "$0: could not re-execute with $CONFIG_SHELL" >&2
exit 255
fi

    if test x$as_have_required = xno
then :
  printf "%s\n" "$0: This script requires a shell more modern than all"
  printf "%s\n" "$0: the shells that I found on your system."
  if test ${ZSH_VERSION+y} ; then
    printf "%s\n" "$0: In particular, zsh $ZSH_VERSION has bugs and should"
    printf "%s\n" "$0: be upgraded to zsh 4.3.4 or later."
  else
    printf "%s\n" "$0: Please tell bug-autoconf@gnu.org about your system,
$0: including any error possibly output before this
$0: message. Then install a modern shell, or manually run
$0: the script under such a shell if you do have one."
  fi
  exit 1
fi
fi
fi
SHELL=${CONFIG_SHELL-/bin/sh}
export SHELL
# Unset more variables known to interfere with behavior of common tools.
CLICOLOR_FORCE= GREP_OPTIONS=
unset CLICOLOR_FORCE GREP_OPTIONS

## --------------------- ##
## M4sh Shell Functions. ##
## --------------------- ##
# as_fn_unset VAR
# ---------------
# Portably unset VAR.
as_fn_unset ()
{
  { eval $1=; unset $1;}
}
as_unset=as_fn_unset


# as_fn_set_status STATUS
# -----------------------
# Set $? to STATUS, without forking.
as_fn_set_status ()
{
  return $1
} # as_fn_set_status

# as_fn_exit STATUS
# -----------------
# Exit the shell with STATUS, even in a "trap 0" or "set -e" context.
as_fn_exit ()
{
  set +e
  as_fn_set_status $1
  exit $1
} # as_fn_exit
# as_fn_nop
# ---------
# Do nothing but, unlike ":", preserve the value of $?.
as_fn_nop ()
{
  return $?
}
as_nop=as_fn_nop

# as_fn_mkdir_p
# -------------
# Create "$as_dir" as a directory, including parents if necessary.
as_fn_mkdir_p ()
{

  case $as_dir in #(
  -*) as_dir=./$as_dir;;
  esac
  test -d "$as_dir" || eval $as_mkdir_p || {
    as_dirs=
    while :; do
      case $as_dir in #(
      *\'*) as_qdir=`printf "%s\n" "$as_dir" | sed "s/'/'\\\\\\\\''/g"`;; #'(
      *) as_qdir=$as_dir;;
      esac
      as_dirs="'$as_qdir' $as_dirs"
      as_dir=`$as_dirname -- "$as_dir" ||
$as_expr X"$as_dir" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$as_dir" : 'X\(//\)[^/]' \| \
	 X"$as_dir" : 'X\(//\)$' \| \
	 X"$as_dir" : 'X\(/\)' \| . 2>/dev/null ||
printf "%s\n" X"$as_dir" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
      test -d "$as_dir" && break
    done
    test -z "$as_dirs" || eval "mkdir $as_dirs"
  } || test -d "$as_dir" || as_fn_error $? "cannot create directory $as_dir"


} # as_fn_mkdir_p

# as_fn_executable_p FILE
# -----------------------
# Test if FILE is an executable regular file.
as_fn_executable_p ()
{
  test -f "$1" && test -x "$1"
} # as_fn_executable_p
# as_fn_append VAR VALUE
# ----------------------
# Append the text in VALUE to the end of the definition contained in VAR. Take
# advantage of any shell optimizations that allow amortized linear growth over
# repeated appends, instead of the typical quadratic growth present in naive
# implementations.
if (eval "as_var=1; as_var+=2; test x\$as_var = x12") 2>/dev/null
then :
  eval 'as_fn_append ()
  {
    eval $1+=\$2
  }'
else $as_nop
  as_fn_append ()
  {
    eval $1=\$$1\$2
  }
fi # as_fn_append

# as_fn_arith ARG...
# ------------------
# Perform arithmetic evaluation on the ARGs, and store the result in the
# global $as_val. Take advantage of shells that can avoid forks. The arguments
# must be portable across $(()) and expr.
if (eval "test \$(( 1 + 1 )) = 2") 2>/dev/null
then :
  eval 'as_fn_arith ()
  {
    as_val=$(( $* ))
  }'
else $as_nop
  as_fn_arith ()
  {
    as_val=`expr "$@" || test $? -eq 1`
  }
fi # as_fn_arith

# as_fn_nop
# ---------
# Do nothing but, unlike ":", preserve the value of $?.
as_fn_nop ()
{
  return $?
}
as_nop=as_fn_nop

# as_fn_error STATUS ERROR [LINENO LOG_FD]
# ----------------------------------------
# Output "`basename $0`: error: ERROR" to stderr. If LINENO and LOG_FD are
# provided, also output the error to LOG_FD, referencing LINENO. Then exit the
# script with STATUS, using 1 if that was 0.
as_fn_error ()
{
  as_status=$1; test $as_status -eq 0 && as_status=1
  if test "$4"; then
    as_lineno=${as_lineno-"$3"} as_lineno_stack=as_lineno_stack=$as_lineno_stack
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: $2" >&$4
  fi
  printf "%s\n" "$as_me: error: $2" >&2
  as_fn_exit $as_status
} # as_fn_error

if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

if (basename -- /) >/dev/null 2>&1 && test "X`basename -- / 2>&1`" = "X/"; then
  as_basename=basename
else
  as_basename=false
fi

if (as_dir=`dirname -- /` && test "X$as_dir" = X/) >/dev/null 2>&1; then
  as_dirname=dirname
else
  as_dirname=false
fi

as_me=`$as_basename -- "$0" ||
$as_expr X/"$0" : '.*/\([^/][^/]*\)/*$' \| \
	 X"$0" : 'X\(//\)$' \| \
	 X"$0" : 'X\(/\)' \| . 2>/dev/null ||
printf "%s\n" X/"$0" |
    sed '/^.*\/\([^/][^/]*\)\/*$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`

# Avoid depending upon Character Ranges.
as_cr_letters='abcdefghijklmnopqrstuvwxyz'
as_cr_LETTERS='ABCDEFGHIJKLMNOPQRSTUVWXYZ'
as_cr_Letters=$as_cr_letters$as_cr_LETTERS
as_cr_digits='0123456789'
as_cr_alnum=$as_cr_Letters$as_cr_digits


  as_lineno_1=$LINENO as_lineno_1a=$LINENO
  as_lineno_2=$LINENO as_lineno_2a=$LINENO
  eval 'test "x$as_lineno_1'$as_run'" != "x$as_lineno_2'$as_run'" &&
  test "x`expr $as_lineno_1'$as_run' + 1`" = "x$as_lineno_2'$as_run'"' || {
  # Blame Lee E. McMahon (1931-1989) for sed's syntax.  :-)
  sed -n '
    p
    /[$]LINENO/=
  ' <$as_myself |
    sed '
      s/[$]LINENO.*/&-/
      t lineno
      b
      :lineno
      N
      :loop
      s/[$]LINENO\([^'$as_cr_alnum'_].*\n\)\(.*\)/\2\1\2/
      t loop
      s/-\n.*//
    ' >$as_me.lineno &&
  chmod +x "$as_me.lineno" ||
    { printf "%s\n" "$as_me: error: cannot create $as_me.lineno; rerun with a POSIX shell" >&2; as_fn_exit 1; }

  # If we had to re-execute with $CONFIG_SHELL, we're ensured to have
  # already done that, so ensure we don't try to do so again and fall
  # in an infinite loop.  This has already happened in practice.
  _as_can_reexec=no; export _as_can_reexec
  # Don't try to exec as it changes $[0], causing all sort of problems
  # (the dirname of $[0] is not the place where we might find the
  # original and so on.  Autoconf is especially sensitive to this).
  . "./$as_me.lineno"
  # Exit status is that of the last command.
  exit
}


# Determine whether it's possible to make 'echo' print without a newline.
# These variables are no longer used directly by Autoconf, but are AC_SUBSTed
# for compatibility with existing Makefiles.
ECHO_C= ECHO_N= ECHO_T=
case `echo -n x` in #(((((
-n*)
  case `echo 'xy\c'` in
  *c*) ECHO_T='	';;	# ECHO_T is single tab character.
  xy)  ECHO_C='\c';;
  *)   echo `echo ksh88 bug on AIX 6.1` > /dev/null
       ECHO_T='	';;
  esac;;
*)
  ECHO_N='-n';;
esac

# For backward compatibility with old third-party macros, we provide
# the shell variables $as_echo and $as_echo_n.  New code should use
# AS_ECHO(["message"]) and AS_ECHO_N(["message"]), respectively.
as_echo='printf %s\n'
as_echo_n='printf %s'


rm -f conf$$ conf$$.exe conf$$.file
if test -d conf$$.dir; then
  rm -f conf$$.dir/conf$$.file
else
  rm -f conf$$.dir
  mkdir conf$$.dir 2>/dev/null
fi
if (echo >conf$$.file) 2>/dev/null; then
  if ln -s conf$$.file conf$$ 2>/dev/null; then
    as_ln_s='ln -s'
    # ... but there are two gotchas:
    # 1) On MSYS, both `ln -s file dir' and `ln file dir' fail.
    # 2) DJGPP < 2.04 has no symlinks; `ln -s' creates a wrapper executable.
    # In both cases, we have to default to `cp -pR'.
    ln -s conf$$.file conf$$.dir 2>/dev/null && test ! -f conf$$.exe ||
      as_ln_s='cp -pR'
  elif ln conf$$.file conf$$ 2>/dev/null; then
    as_ln_s=ln
  else
    as_ln_s='cp -pR'
  fi
else
  as_ln_s='cp -pR'
fi
rm -f conf$$ conf$$.exe conf$$.dir/conf$$.file conf$$.file
rmdir conf$$.dir 2>/dev/null

if mkdir -p . 2>/dev/null; then
  as_mkdir_p='mkdir -p "$as_dir"'
else
  test -d ./-p && rmdir ./-p
  as_mkdir_p=false
fi

as_test_x='test -x'
as_executable_p=as_fn_executable_p

# Sed expression to map a string onto a valid CPP name.
as_tr_cpp="eval sed 'y%*$as_cr_letters%P$as_cr_LETTERS%;s%[^_$as_cr_alnum]%_%g'"

# Sed expression to map a string onto a valid variable name.
as_tr_sh="eval sed 'y%*+%pp%;s%[^_$as_cr_alnum]%_%g'"


test -n "$DJDIR" || exec 7<&0 </dev/null
exec 6>&1

# Name of the host.
# hostname on some systems (SVR3.2, old GNU/Linux) returns a bogus exit status,
# so uname gets run too.
ac_hostname=`(hostname || uname -n) 2>/dev/null | sed 1q`

#
# Initializations.
#
ac_default_prefix=/usr/local
ac_clean_files=
ac_config_libobj_dir=.
LIBOBJS=
cross_compiling=no
subdirs=
MFLAGS=
MAKEFLAGS=

# Identity of this package.
PACKAGE_NAME=''
PACKAGE_TARNAME=''
PACKAGE_VERSION=''
PACKAGE_STRING=''
PACKAGE_BUGREPORT=''
PACKAGE_URL=''

ac_unique_file="hbf.h"
# Factoring default headers for most tests.
ac_includes_default="\
#include <stddef.h>
#ifdef HAVE_STDIO_H
# include <stdio.h>
#endif
#ifdef HAVE_STDLIB_H
# include <stdlib.h>
#endif
#ifdef HAVE_STRING_H
# include <string.h>
#endif
#ifdef HAVE_INTTYPES_H
# include <inttypes.h>
#endif
#ifdef HAVE_STDINT_H
# include <stdint.h>
#endif
#ifdef HAVE_STRINGS_H
# include <strings.h>
#endif
#ifdef HAVE_SYS_TYPES_H
# include <sys/types.h>
#endif
#ifdef HAVE_SYS_STAT_H
# include <sys/stat.h>
#endif
#ifdef HAVE_UNISTD_H
# include <unistd.h>
#endif"

ac_header_c_list=
ac_func_c_list=
ac_subst_vars='LTLIBOBJS
LIBOBJS
INSTALL_DATA
INSTALL_SCRIPT
INSTALL_PROGRAM
RM
no_strdup
XX_CFLAGS
OBJEXT
EXEEXT
ac_ct_CC
CPPFLAGS
LDFLAGS
CFLAGS
CC
target_os
target_vendor
target_cpu
target
host_os
host_vendor
host_cpu
host
build_os
build_vendor
build_cpu
build
target_alias
host_alias
build_alias
LIBS
ECHO_T
ECHO_N
ECHO_C
DEFS
mandir
localedir
libdir
psdir
pdfdir
dvidir
htmldir
infodir
docdir
oldincludedir
includedir
runstatedir
localstatedir
sharedstatedir
sysconfdir
datadir
datarootdir
libexecdir
sbindir
bindir
program_transform_name
prefix
exec_prefix
PACKAGE_URL
PACKAGE_BUGREPORT
PACKAGE_STRING
PACKAGE_VERSION
PACKAGE_TARNAME
PACKAGE_NAME
PATH_SEPARATOR
SHELL'
ac_subst_files=''
ac_user_opts='
enable_option_checking
with_kpathsea_include
with_kpathsea_lib
'
      ac_precious_vars='build_alias
host_alias
target_alias
CC
CFLAGS
LDFLAGS
LIBS
CPPFLAGS'


# Initialize some variables set by options.
ac_init_help=
ac_init_version=false
ac_unrecognized_opts=
ac_unrecognized_sep=
# The variables have the same names as the options, with
# dashes changed to underlines.
cache_file=/dev/null
exec_prefix=NONE
no_create=
no_recursion=
prefix=NONE
program_prefix=NONE
program_suffix=NONE
program_transform_name=s,x,x,
silent=
site=
srcdir=
verbose=
x_includes=NONE
x_libraries=NONE

# Installation directory options.
# These are left unexpanded so users can "make install exec_prefix=/foo"
# and all the variables that are supposed to be based on exec_prefix
# by default will actually change.
# Use braces instead of parens because sh, perl, etc. also accept them.
# (The list follows the same order as the GNU Coding Standards.)
bindir='${exec_prefix}/bin'
sbindir='${exec_prefix}/sbin'
libexecdir='${exec_prefix}/libexec'
datarootdir='${prefix}/share'
datadir='${datarootdir}'
sysconfdir='${prefix}/etc'
sharedstatedir='${prefix}/com'
localstatedir='${prefix}/var'
runstatedir='${localstatedir}/run'
includedir='${prefix}/include'
oldincludedir='/usr/include'
docdir='${datarootdir}/doc/${PACKAGE}'
infodir='${datarootdir}/info'
htmldir='${docdir}'
dvidir='${docdir}'
pdfdir='${docdir}'
psdir='${docdir}'
libdir='${exec_prefix}/lib'
localedir='${datarootdir}/locale'
mandir='${datarootdir}/man'

ac_prev=
ac_dashdash=
for ac_option
do
  # If the previous option needs an argument, assign it.
  if test -n "$ac_prev"; then
    eval $ac_prev=\$ac_option
    ac_prev=
    continue
  fi

  case $ac_option in
  *=?*) ac_optarg=`expr "X$ac_option" : '[^=]*=\(.*\)'` ;;
  *=)   ac_optarg= ;;
  *)    ac_optarg=yes ;;
  esac

  case $ac_dashdash$ac_option in
  --)
    ac_dashdash=yes ;;

  -bindir | --bindir | --bindi | --bind | --bin | --bi)
    ac_prev=bindir ;;
  -bindir=* | --bindir=* | --bindi=* | --bind=* | --bin=* | --bi=*)
    bindir=$ac_optarg ;;

  -build | --build | --buil | --bui | --bu)
    ac_prev=build_alias ;;
  -build=* | --build=* | --buil=* | --bui=* | --bu=*)
    build_alias=$ac_optarg ;;

  -cache-file | --cache-file | --cache-fil | --cache-fi \
  | --cache-f | --cache- | --cache | --cach | --cac | --ca | --c)
    ac_prev=cache_file ;;
  -cache-file=* | --cache-file=* | --cache-fil=* | --cache-fi=* \
  | --cache-f=* | --cache-=* | --cache=* | --cach=* | --cac=* | --ca=* | --c=*)
    cache_file=$ac_optarg ;;

  --config-cache | -C)
    cache_file=config.cache ;;

  -datadir | --datadir | --datadi | --datad)
    ac_prev=datadir ;;
  -datadir=* | --datadir=* | --datadi=* | --datad=*)
    datadir=$ac_optarg ;;

  -datarootdir | --datarootdir | --datarootdi | --datarootd | --dataroot \
  | --dataroo | --dataro | --datar)
    ac_prev=datarootdir ;;
  -datarootdir=* | --datarootdir=* | --datarootdi=* | --datarootd=* \
  | --dataroot=* | --dataroo=* | --dataro=* | --datar=*)
    datarootdir=$ac_optarg ;;

  -disable-* | --disable-*)
    ac_useropt=`expr "x$ac_option" : 'x-*disable-\(.*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_useropt" : ".*[^-+._$as_cr_alnum]" >/dev/null &&
      as_fn_error $? "invalid feature name: \`$ac_useropt'"
    ac_useropt_orig=$ac_useropt
    ac_useropt=`printf "%s\n" "$ac_useropt" | sed 's/[-+.]/_/g'`
    case $ac_user_opts in
      *"
"enable_$ac_useropt"
"*) ;;
      *) ac_unrecognized_opts="$ac_unrecognized_opts$ac_unrecognized_sep--disable-$ac_useropt_orig"
	 ac_unrecognized_sep=', ';;
    esac
    eval enable_$ac_useropt=no ;;

  -docdir | --docdir | --docdi | --doc | --do)
    ac_prev=docdir ;;
  -docdir=* | --docdir=* | --docdi=* | --doc=* | --do=*)
    docdir=$ac_optarg ;;

  -dvidir | --dvidir | --dvidi | --dvid | --dvi | --dv)
    ac_prev=dvidir ;;
  -dvidir=* | --dvidir=* | --dvidi=* | --dvid=* | --dvi=* | --dv=*)
    dvidir=$ac_optarg ;;

  -enable-* | --enable-*)
    ac_useropt=`expr "x$ac_option" : 'x-*enable-\([^=]*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_useropt" : ".*[^-+._$as_cr_alnum]" >/dev/null &&
      as_fn_error $? "invalid feature name: \`$ac_useropt'"
    ac_useropt_orig=$ac_useropt
    ac_useropt=`printf "%s\n" "$ac_useropt" | sed 's/[-+.]/_/g'`
    case $ac_user_opts in
      *"
"enable_$ac_useropt"
"*) ;;
      *) ac_unrecognized_opts="$ac_unrecognized_opts$ac_unrecognized_sep--enable-$ac_useropt_orig"
	 ac_unrecognized_sep=', ';;
    esac
    eval enable_$ac_useropt=\$ac_optarg ;;

  -exec-prefix | --exec_prefix | --exec-prefix | --exec-prefi \
  | --exec-pref | --exec-pre | --exec-pr | --exec-p | --exec- \
  | --exec | --exe | --ex)
    ac_prev=exec_prefix ;;
  -exec-prefix=* | --exec_prefix=* | --exec-prefix=* | --exec-prefi=* \
  | --exec-pref=* | --exec-pre=* | --exec-pr=* | --exec-p=* | --exec-=* \
  | --exec=* | --exe=* | --ex=*)
    exec_prefix=$ac_optarg ;;

  -gas | --gas | --ga | --g)
    # Obsolete; use --with-gas.
    with_gas=yes ;;

  -help | --help | --hel | --he | -h)
    ac_init_help=long ;;
  -help=r* | --help=r* | --hel=r* | --he=r* | -hr*)
    ac_init_help=recursive ;;
  -help=s* | --help=s* | --hel=s* | --he=s* | -hs*)
    ac_init_help=short ;;

  -host | --host | --hos | --ho)
    ac_prev=host_alias ;;
  -host=* | --host=* | --hos=* | --ho=*)
    host_alias=$ac_optarg ;;

  -htmldir | --htmldir | --htmldi | --htmld | --html | --htm | --ht)
    ac_prev=htmldir ;;
  -htmldir=* | --htmldir=* | --htmldi=* | --htmld=* | --html=* | --htm=* \
  | --ht=*)
    htmldir=$ac_optarg ;;

  -includedir | --includedir | --includedi | --included | --include \
  | --includ | --inclu | --incl | --inc)
    ac_prev=includedir ;;
  -includedir=* | --includedir=* | --includedi=* | --included=* | --include=* \
  | --includ=* | --inclu=* | --incl=* | --inc=*)
    includedir=$ac_optarg ;;

  -infodir | --infodir | --infodi | --infod | --info | --inf)
    ac_prev=infodir ;;
  -infodir=* | --infodir=* | --infodi=* | --infod=* | --info=* | --inf=*)
    infodir=$ac_optarg ;;

  -libdir | --libdir | --libdi | --libd)
    ac_prev=libdir ;;
  -libdir=* | --libdir=* | --libdi=* | --libd=*)
    libdir=$ac_optarg ;;

  -libexecdir | --libexecdir | --libexecdi | --libexecd | --libexec \
  | --libexe | --libex | --libe)
    ac_prev=libexecdir ;;
  -libexecdir=* | --libexecdir=* | --libexecdi=* | --libexecd=* | --libexec=* \
  | --libexe=* | --libex=* | --libe=*)
    libexecdir=$ac_optarg ;;

  -localedir | --localedir | --localedi | --localed | --locale)
    ac_prev=localedir ;;
  -localedir=* | --localedir=* | --localedi=* | --localed=* | --locale=*)
    localedir=$ac_optarg ;;

  -localstatedir | --localstatedir | --localstatedi | --localstated \
  | --localstate | --localstat | --localsta | --localst | --locals)
    ac_prev=localstatedir ;;
  -localstatedir=* | --localstatedir=* | --localstatedi=* | --localstated=* \
  | --localstate=* | --localstat=* | --localsta=* | --localst=* | --locals=*)
    localstatedir=$ac_optarg ;;

  -mandir | --mandir | --mandi | --mand | --man | --ma | --m)
    ac_prev=mandir ;;
  -mandir=* | --mandir=* | --mandi=* | --mand=* | --man=* | --ma=* | --m=*)
    mandir=$ac_optarg ;;

  -nfp | --nfp | --nf)
    # Obsolete; use --without-fp.
    with_fp=no ;;

  -no-create | --no-create | --no-creat | --no-crea | --no-cre \
  | --no-cr | --no-c | -n)
    no_create=yes ;;

  -no-recursion | --no-recursion | --no-recursio | --no-recursi \
  | --no-recurs | --no-recur | --no-recu | --no-rec | --no-re | --no-r)
    no_recursion=yes ;;

  -oldincludedir | --oldincludedir | --oldincludedi | --oldincluded \
  | --oldinclude | --oldinclud | --oldinclu | --oldincl | --oldinc \
  | --oldin | --oldi | --old | --ol | --o)
    ac_prev=oldincludedir ;;
  -oldincludedir=* | --oldincludedir=* | --oldincludedi=* | --oldincluded=* \
  | --oldinclude=* | --oldinclud=* | --oldinclu=* | --oldincl=* | --oldinc=* \
  | --oldin=* | --oldi=* | --old=* | --ol=* | --o=*)
    oldincludedir=$ac_optarg ;;

  -prefix | --prefix | --prefi | --pref | --pre | --pr | --p)
    ac_prev=prefix ;;
  -prefix=* | --prefix=* | --prefi=* | --pref=* | --pre=* | --pr=* | --p=*)
    prefix=$ac_optarg ;;

  -program-prefix | --program-prefix | --program-prefi | --program-pref \
  | --program-pre | --program-pr | --program-p)
    ac_prev=program_prefix ;;
  -program-prefix=* | --program-prefix=* | --program-prefi=* \
  | --program-pref=* | --program-pre=* | --program-pr=* | --program-p=*)
    program_prefix=$ac_optarg ;;

  -program-suffix | --program-suffix | --program-suffi | --program-suff \
  | --program-suf | --program-su | --program-s)
    ac_prev=program_suffix ;;
  -program-suffix=* | --program-suffix=* | --program-suffi=* \
  | --program-suff=* | --program-suf=* | --program-su=* | --program-s=*)
    program_suffix=$ac_optarg ;;

  -program-transform-name | --program-transform-name \
  | --program-transform-nam | --program-transform-na \
  | --program-transform-n | --program-transform- \
  | --program-transform | --program-transfor \
  | --program-transfo | --program-transf \
  | --program-trans | --program-tran \
  | --progr-tra | --program-tr | --program-t)
    ac_prev=program_transform_name ;;
  -program-transform-name=* | --program-transform-name=* \
  | --program-transform-nam=* | --program-transform-na=* \
  | --program-transform-n=* | --program-transform-=* \
  | --program-transform=* | --program-transfor=* \
  | --program-transfo=* | --program-transf=* \
  | --program-trans=* | --program-tran=* \
  | --progr-tra=* | --program-tr=* | --program-t=*)
    program_transform_name=$ac_optarg ;;

  -pdfdir | --pdfdir | --pdfdi | --pdfd | --pdf | --pd)
    ac_prev=pdfdir ;;
  -pdfdir=* | --pdfdir=* | --pdfdi=* | --pdfd=* | --pdf=* | --pd=*)
    pdfdir=$ac_optarg ;;

  -psdir | --psdir | --psdi | --psd | --ps)
    ac_prev=psdir ;;
  -psdir=* | --psdir=* | --psdi=* | --psd=* | --ps=*)
    psdir=$ac_optarg ;;

  -q | -quiet | --quiet | --quie | --qui | --qu | --q \
  | -silent | --silent | --silen | --sile | --sil)
    silent=yes ;;

  -runstatedir | --runstatedir | --runstatedi | --runstated \
  | --runstate | --runstat | --runsta | --runst | --runs \
  | --run | --ru | --r)
    ac_prev=runstatedir ;;
  -runstatedir=* | --runstatedir=* | --runstatedi=* | --runstated=* \
  | --runstate=* | --runstat=* | --runsta=* | --runst=* | --runs=* \
  | --run=* | --ru=* | --r=*)
    runstatedir=$ac_optarg ;;

  -sbindir | --sbindir | --sbindi | --sbind | --sbin | --sbi | --sb)
    ac_prev=sbindir ;;
  -sbindir=* | --sbindir=* | --sbindi=* | --sbind=* | --sbin=* \
  | --sbi=* | --sb=*)
    sbindir=$ac_optarg ;;

  -sharedstatedir | --sharedstatedir | --sharedstatedi \
  | --sharedstated | --sharedstate | --sharedstat | --sharedsta \
  | --sharedst | --shareds | --shared | --share | --shar \
  | --sha | --sh)
    ac_prev=sharedstatedir ;;
  -sharedstatedir=* | --sharedstatedir=* | --sharedstatedi=* \
  | --sharedstated=* | --sharedstate=* | --sharedstat=* | --sharedsta=* \
  | --sharedst=* | --shareds=* | --shared=* | --share=* | --shar=* \
  | --sha=* | --sh=*)
    sharedstatedir=$ac_optarg ;;

  -site | --site | --sit)
    ac_prev=site ;;
  -site=* | --site=* | --sit=*)
    site=$ac_optarg ;;

  -srcdir | --srcdir | --srcdi | --srcd | --src | --sr)
    ac_prev=srcdir ;;
  -srcdir=* | --srcdir=* | --srcdi=* | --srcd=* | --src=* | --sr=*)
    srcdir=$ac_optarg ;;

  -sysconfdir | --sysconfdir | --sysconfdi | --sysconfd | --sysconf \
  | --syscon | --sysco | --sysc | --sys | --sy)
    ac_prev=sysconfdir ;;
  -sysconfdir=* | --sysconfdir=* | --sysconfdi=* | --sysconfd=* | --sysconf=* \
  | --syscon=* | --sysco=* | --sysc=* | --sys=* | --sy=*)
    sysconfdir=$ac_optarg ;;

  -target | --target | --targe | --targ | --tar | --ta | --t)
    ac_prev=target_alias ;;
  -target=* | --target=* | --targe=* | --targ=* | --tar=* | --ta=* | --t=*)
    target_alias=$ac_optarg ;;

  -v | -verbose | --verbose | --verbos | --verbo | --verb)
    verbose=yes ;;

  -version | --version | --versio | --versi | --vers | -V)
    ac_init_version=: ;;

  -with-* | --with-*)
    ac_useropt=`expr "x$ac_option" : 'x-*with-\([^=]*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_useropt" : ".*[^-+._$as_cr_alnum]" >/dev/null &&
      as_fn_error $? "invalid package name: \`$ac_useropt'"
    ac_useropt_orig=$ac_useropt
    ac_useropt=`printf "%s\n" "$ac_useropt" | sed 's/[-+.]/_/g'`
    case $ac_user_opts in
      *"
"with_$ac_useropt"
"*) ;;
      *) ac_unrecognized_opts="$ac_unrecognized_opts$ac_unrecognized_sep--with-$ac_useropt_orig"
	 ac_unrecognized_sep=', ';;
    esac
    eval with_$ac_useropt=\$ac_optarg ;;

  -without-* | --without-*)
    ac_useropt=`expr "x$ac_option" : 'x-*without-\(.*\)'`
    # Reject names that are not valid shell variable names.
    expr "x$ac_useropt" : ".*[^-+._$as_cr_alnum]" >/dev/null &&
      as_fn_error $? "invalid package name: \`$ac_useropt'"
    ac_useropt_orig=$ac_useropt
    ac_useropt=`printf "%s\n" "$ac_useropt" | sed 's/[-+.]/_/g'`
    case $ac_user_opts in
      *"
"with_$ac_useropt"
"*) ;;
      *) ac_unrecognized_opts="$ac_unrecognized_opts$ac_unrecognized_sep--without-$ac_useropt_orig"
	 ac_unrecognized_sep=', ';;
    esac
    eval with_$ac_useropt=no ;;

  --x)
    # Obsolete; use --with-x.
    with_x=yes ;;

  -x-includes | --x-includes | --x-include | --x-includ | --x-inclu \
  | --x-incl | --x-inc | --x-in | --x-i)
    ac_prev=x_includes ;;
  -x-includes=* | --x-includes=* | --x-include=* | --x-includ=* | --x-inclu=* \
  | --x-incl=* | --x-inc=* | --x-in=* | --x-i=*)
    x_includes=$ac_optarg ;;

  -x-libraries | --x-libraries | --x-librarie | --x-librari \
  | --x-librar | --x-libra | --x-libr | --x-lib | --x-li | --x-l)
    ac_prev=x_libraries ;;
  -x-libraries=* | --x-libraries=* | --x-librarie=* | --x-librari=* \
  | --x-librar=* | --x-libra=* | --x-libr=* | --x-lib=* | --x-li=* | --x-l=*)
    x_libraries=$ac_optarg ;;

  -*) as_fn_error $? "unrecognized option: \`$ac_option'
Try \`$0 --help' for more information"
    ;;

  *=*)
    ac_envvar=`expr "x$ac_option" : 'x\([^=]*\)='`
    # Reject names that are not valid shell variable names.
    case $ac_envvar in #(
      '' | [0-9]* | *[!_$as_cr_alnum]* )
      as_fn_error $? "invalid variable name: \`$ac_envvar'" ;;
    esac
    eval $ac_envvar=\$ac_optarg
    export $ac_envvar ;;

  *)
    # FIXME: should be removed in autoconf 3.0.
    printf "%s\n" "$as_me: WARNING: you should use --build, --host, --target" >&2
    expr "x$ac_option" : ".*[^-._$as_cr_alnum]" >/dev/null &&
      printf "%s\n" "$as_me: WARNING: invalid host type: $ac_option" >&2
    : "${build_alias=$ac_option} ${host_alias=$ac_option} ${target_alias=$ac_option}"
    ;;

  esac
done

if test -n "$ac_prev"; then
  ac_option=--`echo $ac_prev | sed 's/_/-/g'`
  as_fn_error $? "missing argument to $ac_option"
fi

if test -n "$ac_unrecognized_opts"; then
  case $enable_option_checking in
    no) ;;
    fatal) as_fn_error $? "unrecognized options: $ac_unrecognized_opts" ;;
    *)     printf "%s\n" "$as_me: WARNING: unrecognized options: $ac_unrecognized_opts" >&2 ;;
  esac
fi

# Check all directory arguments for consistency.
for ac_var in	exec_prefix prefix bindir sbindir libexecdir datarootdir \
		datadir sysconfdir sharedstatedir localstatedir includedir \
		oldincludedir docdir infodir htmldir dvidir pdfdir psdir \
		libdir localedir mandir runstatedir
do
  eval ac_val=\$$ac_var
  # Remove trailing slashes.
  case $ac_val in
    */ )
      ac_val=`expr "X$ac_val" : 'X\(.*[^/]\)' \| "X$ac_val" : 'X\(.*\)'`
      eval $ac_var=\$ac_val;;
  esac
  # Be sure to have absolute directory names.
  case $ac_val in
    [\\/$]* | ?:[\\/]* )  continue;;
    NONE | '' ) case $ac_var in *prefix ) continue;; esac;;
  esac
  as_fn_error $? "expected an absolute directory name for --$ac_var: $ac_val"
done

# There might be people who depend on the old broken behavior: `$host'
# used to hold the argument of --host etc.
# FIXME: To remove some day.
build=$build_alias
host=$host_alias
target=$target_alias

# FIXME: To remove some day.
if test "x$host_alias" != x; then
  if test "x$build_alias" = x; then
    cross_compiling=maybe
  elif test "x$build_alias" != "x$host_alias"; then
    cross_compiling=yes
  fi
fi

ac_tool_prefix=
test -n "$host_alias" && ac_tool_prefix=$host_alias-

test "$silent" = yes && exec 6>/dev/null


ac_pwd=`pwd` && test -n "$ac_pwd" &&
ac_ls_di=`ls -di .` &&
ac_pwd_ls_di=`cd "$ac_pwd" && ls -di .` ||
  as_fn_error $? "working directory cannot be determined"
test "X$ac_ls_di" = "X$ac_pwd_ls_di" ||
  as_fn_error $? "pwd does not report name of working directory"


# Find the source files, if location was not specified.
if test -z "$srcdir"; then
  ac_srcdir_defaulted=yes
  # Try the directory containing this script, then the parent directory.
  ac_confdir=`$as_dirname -- "$as_myself" ||
$as_expr X"$as_myself" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$as_myself" : 'X\(//\)[^/]' \| \
	 X"$as_myself" : 'X\(//\)$' \| \
	 X"$as_myself" : 'X\(/\)' \| . 2>/dev/null ||
printf "%s\n" X"$as_myself" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
  srcdir=$ac_confdir
  if test ! -r "$srcdir/$ac_unique_file"; then
    srcdir=..
  fi
else
  ac_srcdir_defaulted=no
fi
if test ! -r "$srcdir/$ac_unique_file"; then
  test "$ac_srcdir_defaulted" = yes && srcdir="$ac_confdir or .."
  as_fn_error $? "cannot find sources ($ac_unique_file) in $srcdir"
fi
ac_msg="sources are in $srcdir, but \`cd $srcdir' does not work"
ac_abs_confdir=`(
	cd "$srcdir" && test -r "./$ac_unique_file" || as_fn_error $? "$ac_msg"
	pwd)`
# When building in place, set srcdir=.
if test "$ac_abs_confdir" = "$ac_pwd"; then
  srcdir=.
fi
# Remove unnecessary trailing slashes from srcdir.
# Double slashes in file names in object file debugging info
# mess up M-x gdb in Emacs.
case $srcdir in
*/) srcdir=`expr "X$srcdir" : 'X\(.*[^/]\)' \| "X$srcdir" : 'X\(.*\)'`;;
esac
for ac_var in $ac_precious_vars; do
  eval ac_env_${ac_var}_set=\${${ac_var}+set}
  eval ac_env_${ac_var}_value=\$${ac_var}
  eval ac_cv_env_${ac_var}_set=\${${ac_var}+set}
  eval ac_cv_env_${ac_var}_value=\$${ac_var}
done

#
# Report the --help message.
#
if test "$ac_init_help" = "long"; then
  # Omit some internal or obsolete options to make the list less imposing.
  # This message is too long to be a string in the A/UX 3.1 sh.
  cat <<_ACEOF
\`configure' configures this package to adapt to many kinds of systems.

Usage: $0 [OPTION]... [VAR=VALUE]...

To assign environment variables (e.g., CC, CFLAGS...), specify them as
VAR=VALUE.  See below for descriptions of some of the useful variables.

Defaults for the options are specified in brackets.

Configuration:
  -h, --help              display this help and exit
      --help=short        display options specific to this package
      --help=recursive    display the short help of all the included packages
  -V, --version           display version information and exit
  -q, --quiet, --silent   do not print \`checking ...' messages
      --cache-file=FILE   cache test results in FILE [disabled]
  -C, --config-cache      alias for \`--cache-file=config.cache'
  -n, --no-create         do not create output files
      --srcdir=DIR        find the sources in DIR [configure dir or \`..']

Installation directories:
  --prefix=PREFIX         install architecture-independent files in PREFIX
                          [$ac_default_prefix]
  --exec-prefix=EPREFIX   install architecture-dependent files in EPREFIX
                          [PREFIX]

By default, \`make install' will install all the files in
\`$ac_default_prefix/bin', \`$ac_default_prefix/lib' etc.  You can specify
an installation prefix other than \`$ac_default_prefix' using \`--prefix',
for instance \`--prefix=\$HOME'.

For better control, use the options below.

Fine tuning of the installation directories:
  --bindir=DIR            user executables [EPREFIX/bin]
  --sbindir=DIR           system admin executables [EPREFIX/sbin]
  --libexecdir=DIR        program executables [EPREFIX/libexec]
  --sysconfdir=DIR        read-only single-machine data [PREFIX/etc]
  --sharedstatedir=DIR    modifiable architecture-independent data [PREFIX/com]
  --localstatedir=DIR     modifiable single-machine data [PREFIX/var]
  --runstatedir=DIR       modifiable per-process data [LOCALSTATEDIR/run]
  --libdir=DIR            object code libraries [EPREFIX/lib]
  --includedir=DIR        C header files [PREFIX/include]
  --oldincludedir=DIR     C header files for non-gcc [/usr/include]
  --datarootdir=DIR       read-only arch.-independent data root [PREFIX/share]
  --datadir=DIR           read-only architecture-independent data [DATAROOTDIR]
  --infodir=DIR           info documentation [DATAROOTDIR/info]
  --localedir=DIR         locale-dependent data [DATAROOTDIR/locale]
  --mandir=DIR            man documentation [DATAROOTDIR/man]
  --docdir=DIR            documentation root [DATAROOTDIR/doc/PACKAGE]
  --htmldir=DIR           html documentation [DOCDIR]
  --dvidir=DIR            dvi documentation [DOCDIR]
  --pdfdir=DIR            pdf documentation [DOCDIR]
  --psdir=DIR             ps documentation [DOCDIR]
_ACEOF

  cat <<\_ACEOF

System types:
  --build=BUILD     configure for building on BUILD [guessed]
  --host=HOST       cross-compile to build programs to run on HOST [BUILD]
  --target=TARGET   configure for building compilers for TARGET [HOST]
_ACEOF
fi

if test -n "$ac_init_help"; then

  cat <<\_ACEOF

Optional Packages:
  --with-PACKAGE[=ARG]    use PACKAGE [ARG=yes]
  --without-PACKAGE       do not use PACKAGE (same as --with-PACKAGE=no)
  --with-kpathsea-include=DIR
                          location of the kpathsea include dir
  --with-kpathsea-lib=DIR
                          location of the kpathsea lib dir

Some influential environment variables:
  CC          C compiler command
  CFLAGS      C compiler flags
  LDFLAGS     linker flags, e.g. -L<lib dir> if you have libraries in a
              nonstandard directory <lib dir>
  LIBS        libraries to pass to the linker, e.g. -l<library>
  CPPFLAGS    (Objective) C/C++ preprocessor flags, e.g. -I<include dir> if
              you have headers in a nonstandard directory <include dir>

Use these variables to override the choices made by `configure' or to help
it to find libraries and programs with nonstandard names/locations.

Report bugs to the package provider.
_ACEOF
ac_status=$?
fi

if test "$ac_init_help" = "recursive"; then
  # If there are subdirs, report their specific --help.
  for ac_dir in : $ac_subdirs_all; do test "x$ac_dir" = x: && continue
    test -d "$ac_dir" ||
      { cd "$srcdir" && ac_pwd=`pwd` && srcdir=. && test -d "$ac_dir"; } ||
      continue
    ac_builddir=.

case "$ac_dir" in
.) ac_dir_suffix= ac_top_builddir_sub=. ac_top_build_prefix= ;;
*)
  ac_dir_suffix=/`printf "%s\n" "$ac_dir" | sed 's|^\.[\\/]||'`
  # A ".." for each directory in $ac_dir_suffix.
  ac_top_builddir_sub=`printf "%s\n" "$ac_dir_suffix" | sed 's|/[^\\/]*|/..|g;s|/||'`
  case $ac_top_builddir_sub in
  "") ac_top_builddir_sub=. ac_top_build_prefix= ;;
  *)  ac_top_build_prefix=$ac_top_builddir_sub/ ;;
  esac ;;
esac
ac_abs_top_builddir=$ac_pwd
ac_abs_builddir=$ac_pwd$ac_dir_suffix
# for backward compatibility:
ac_top_builddir=$ac_top_build_prefix

case $srcdir in
  .)  # We are building in place.
    ac_srcdir=.
    ac_top_srcdir=$ac_top_builddir_sub
    ac_abs_top_srcdir=$ac_pwd ;;
  [\\/]* | ?:[\\/]* )  # Absolute name.
    ac_srcdir=$srcdir$ac_dir_suffix;
    ac_top_srcdir=$srcdir
    ac_abs_top_srcdir=$srcdir ;;
  *) # Relative name.
    ac_srcdir=$ac_top_build_prefix$srcdir$ac_dir_suffix
    ac_top_srcdir=$ac_top_build_prefix$srcdir
    ac_abs_top_srcdir=$ac_pwd/$srcdir ;;
esac
ac_abs_srcdir=$ac_abs_top_srcdir$ac_dir_suffix

    cd "$ac_dir" || { ac_status=$?; continue; }
    # Check for configure.gnu first; this name is used for a wrapper for
    # Metaconfig's "Configure" on case-insensitive file systems.
    if test -f "$ac_srcdir/configure.gnu"; then
      echo &&
      $SHELL "$ac_srcdir/configure.gnu" --help=recursive
    elif test -f "$ac_srcdir/configure"; then
      echo &&
      $SHELL "$ac_srcdir/configure" --help=recursive
    else
      printf "%s\n" "$as_me: WARNING: no configuration information is in $ac_dir" >&2
    fi || ac_status=$?
    cd "$ac_pwd" || { ac_status=$?; break; }
  done
fi

test -n "$ac_init_help" && exit $ac_status
if $ac_init_version; then
  cat <<\_ACEOF
configure
generated by GNU Autoconf 2.71

Copyright (C) 2021 Free Software Foundation, Inc.
This configure script is free software; the Free Software Foundation
gives unlimited permission to copy, distribute and modify it.
_ACEOF
  exit
fi

## ------------------------ ##
## Autoconf initialization. ##
## ------------------------ ##

# ac_fn_c_try_compile LINENO
# --------------------------
# Try to compile conftest.$ac_ext, and return whether this succeeded.
ac_fn_c_try_compile ()
{
  as_lineno=${as_lineno-"$1"} as_lineno_stack=as_lineno_stack=$as_lineno_stack
  rm -f conftest.$ac_objext conftest.beam
  if { { ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval ac_try_echo="\"\$as_me:${as_lineno-$LINENO}: $ac_try_echo\""
printf "%s\n" "$ac_try_echo"; } >&5
  (eval "$ac_compile") 2>conftest.err
  ac_status=$?
  if test -s conftest.err; then
    grep -v '^ *+' conftest.err >conftest.er1
    cat conftest.er1 >&5
    mv -f conftest.er1 conftest.err
  fi
  printf "%s\n" "$as_me:${as_lineno-$LINENO}: \$? = $ac_status" >&5
  test $ac_status = 0; } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest.$ac_objext
then :
  ac_retval=0
else $as_nop
  printf "%s\n" "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_retval=1
fi
  eval $as_lineno_stack; ${as_lineno_stack:+:} unset as_lineno
  as_fn_set_status $ac_retval

} # ac_fn_c_try_compile

# ac_fn_c_try_link LINENO
# -----------------------
# Try to link conftest.$ac_ext, and return whether this succeeded.
ac_fn_c_try_link ()
{
  as_lineno=${as_lineno-"$1"} as_lineno_stack=as_lineno_stack=$as_lineno_stack
  rm -f conftest.$ac_objext conftest.beam conftest$ac_exeext
  if { { ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval ac_try_echo="\"\$as_me:${as_lineno-$LINENO}: $ac_try_echo\""
printf "%s\n" "$ac_try_echo"; } >&5
  (eval "$ac_link") 2>conftest.err
  ac_status=$?
  if test -s conftest.err; then
    grep -v '^ *+' conftest.err >conftest.er1
    cat conftest.er1 >&5
    mv -f conftest.er1 conftest.err
  fi
  printf "%s\n" "$as_me:${as_lineno-$LINENO}: \$? = $ac_status" >&5
  test $ac_status = 0; } && {
	 test -z "$ac_c_werror_flag" ||
	 test ! -s conftest.err
       } && test -s conftest$ac_exeext && {
	 test "$cross_compiling" = yes ||
	 test -x conftest$ac_exeext
       }
then :
  ac_retval=0
else $as_nop
  printf "%s\n" "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

	ac_retval=1
fi
  # Delete the IPA/IPO (Inter Procedural Analysis/Optimization) information
  # created by the PGI compiler (conftest_ipa8_conftest.oo), as it would
  # interfere with the next link command; also delete a directory that is
  # left behind by Apple's compiler.  We do this before executing the actions.
  rm -rf conftest.dSYM conftest_ipa8_conftest.oo
  eval $as_lineno_stack; ${as_lineno_stack:+:} unset as_lineno
  as_fn_set_status $ac_retval

} # ac_fn_c_try_link

# ac_fn_c_check_header_compile LINENO HEADER VAR INCLUDES
# -------------------------------------------------------
# Tests whether HEADER exists and can be compiled using the include files in
# INCLUDES, setting the cache variable VAR accordingly.
ac_fn_c_check_header_compile ()
{
  as_lineno=${as_lineno-"$1"} as_lineno_stack=as_lineno_stack=$as_lineno_stack
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $2" >&5
printf %s "checking for $2... " >&6; }
if eval test \${$3+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */
$4
#include <$2>
_ACEOF
if ac_fn_c_try_compile "$LINENO"
then :
  eval "$3=yes"
else $as_nop
  eval "$3=no"
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam conftest.$ac_ext
fi
eval ac_res=\$$3
	       { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_res" >&5
printf "%s\n" "$ac_res" >&6; }
  eval $as_lineno_stack; ${as_lineno_stack:+:} unset as_lineno

} # ac_fn_c_check_header_compile

# ac_fn_c_check_func LINENO FUNC VAR
# ----------------------------------
# Tests whether FUNC exists, setting the cache variable VAR accordingly
ac_fn_c_check_func ()
{
  as_lineno=${as_lineno-"$1"} as_lineno_stack=as_lineno_stack=$as_lineno_stack
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $2" >&5
printf %s "checking for $2... " >&6; }
if eval test \${$3+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */
/* Define $2 to an innocuous variant, in case <limits.h> declares $2.
   For example, HP-UX 11i <limits.h> declares gettimeofday.  */
#define $2 innocuous_$2

/* System header to define __stub macros and hopefully few prototypes,
   which can conflict with char $2 (); below.  */

#include <limits.h>
#undef $2

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
#ifdef __cplusplus
extern "C"
#endif
char $2 ();
/* The GNU C library defines this for functions which it implements
    to always fail with ENOSYS.  Some functions are actually named
    something starting with __ and the normal name is an alias.  */
#if defined __stub_$2 || defined __stub___$2
choke me
#endif

int
main (void)
{
return $2 ();
  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_link "$LINENO"
then :
  eval "$3=yes"
else $as_nop
  eval "$3=no"
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam \
    conftest$ac_exeext conftest.$ac_ext
fi
eval ac_res=\$$3
	       { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_res" >&5
printf "%s\n" "$ac_res" >&6; }
  eval $as_lineno_stack; ${as_lineno_stack:+:} unset as_lineno

} # ac_fn_c_check_func
ac_configure_args_raw=
for ac_arg
do
  case $ac_arg in
  *\'*)
    ac_arg=`printf "%s\n" "$ac_arg" | sed "s/'/'\\\\\\\\''/g"` ;;
  esac
  as_fn_append ac_configure_args_raw " '$ac_arg'"
done

case $ac_configure_args_raw in
  *$as_nl*)
    ac_safe_unquote= ;;
  *)
    ac_unsafe_z='|&;<>()$`\\"*?[ ''	' # This string ends in space, tab.
    ac_unsafe_a="$ac_unsafe_z#~"
    ac_safe_unquote="s/ '\\([^$ac_unsafe_a][^$ac_unsafe_z]*\\)'/ \\1/g"
    ac_configure_args_raw=`      printf "%s\n" "$ac_configure_args_raw" | sed "$ac_safe_unquote"`;;
esac

cat >config.log <<_ACEOF
This file contains any messages produced by compilers while
running configure, to aid debugging if configure makes a mistake.

It was created by $as_me, which was
generated by GNU Autoconf 2.71.  Invocation command line was

  $ $0$ac_configure_args_raw

_ACEOF
exec 5>>config.log
{
cat <<_ASUNAME
## --------- ##
## Platform. ##
## --------- ##

hostname = `(hostname || uname -n) 2>/dev/null | sed 1q`
uname -m = `(uname -m) 2>/dev/null || echo unknown`
uname -r = `(uname -r) 2>/dev/null || echo unknown`
uname -s = `(uname -s) 2>/dev/null || echo unknown`
uname -v = `(uname -v) 2>/dev/null || echo unknown`

/usr/bin/uname -p = `(/usr/bin/uname -p) 2>/dev/null || echo unknown`
/bin/uname -X     = `(/bin/uname -X) 2>/dev/null     || echo unknown`

/bin/arch              = `(/bin/arch) 2>/dev/null              || echo unknown`
/usr/bin/arch -k       = `(/usr/bin/arch -k) 2>/dev/null       || echo unknown`
/usr/convex/getsysinfo = `(/usr/convex/getsysinfo) 2>/dev/null || echo unknown`
/usr/bin/hostinfo      = `(/usr/bin/hostinfo) 2>/dev/null      || echo unknown`
/bin/machine           = `(/bin/machine) 2>/dev/null           || echo unknown`
/usr/bin/oslevel       = `(/usr/bin/oslevel) 2>/dev/null       || echo unknown`
/bin/universe          = `(/bin/universe) 2>/dev/null          || echo unknown`

_ASUNAME

as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    printf "%s\n" "PATH: $as_dir"
  done
IFS=$as_save_IFS

} >&5

cat >&5 <<_ACEOF


## ----------- ##
## Core tests. ##
## ----------- ##

_ACEOF


# Keep a trace of the command line.
# Strip out --no-create and --no-recursion so they do not pile up.
# Strip out --silent because we don't want to record it for future runs.
# Also quote any args containing shell meta-characters.
# Make two passes to allow for proper duplicate-argument suppression.
ac_configure_args=
ac_configure_args0=
ac_configure_args1=
ac_must_keep_next=false
for ac_pass in 1 2
do
  for ac_arg
  do
    case $ac_arg in
    -no-create | --no-c* | -n | -no-recursion | --no-r*) continue ;;
    -q | -quiet | --quiet | --quie | --qui | --qu | --q \
    | -silent | --silent | --silen | --sile | --sil)
      continue ;;
    *\'*)
      ac_arg=`printf "%s\n" "$ac_arg" | sed "s/'/'\\\\\\\\''/g"` ;;
    esac
    case $ac_pass in
    1) as_fn_append ac_configure_args0 " '$ac_arg'" ;;
    2)
      as_fn_append ac_configure_args1 " '$ac_arg'"
      if test $ac_must_keep_next = true; then
	ac_must_keep_next=false # Got value, back to normal.
      else
	case $ac_arg in
	  *=* | --config-cache | -C | -disable-* | --disable-* \
	  | -enable-* | --enable-* | -gas | --g* | -nfp | --nf* \
	  | -q | -quiet | --q* | -silent | --sil* | -v | -verb* \
	  | -with-* | --with-* | -without-* | --without-* | --x)
	    case "$ac_configure_args0 " in
	      "$ac_configure_args1"*" '$ac_arg' "* ) continue ;;
	    esac
	    ;;
	  -* ) ac_must_keep_next=true ;;
	esac
      fi
      as_fn_append ac_configure_args " '$ac_arg'"
      ;;
    esac
  done
done
{ ac_configure_args0=; unset ac_configure_args0;}
{ ac_configure_args1=; unset ac_configure_args1;}

# When interrupted or exit'd, cleanup temporary files, and complete
# config.log.  We remove comments because anyway the quotes in there
# would cause problems or look ugly.
# WARNING: Use '\'' to represent an apostrophe within the trap.
# WARNING: Do not start the trap code with a newline, due to a FreeBSD 4.0 bug.
trap 'exit_status=$?
  # Sanitize IFS.
  IFS=" ""	$as_nl"
  # Save into config.log some information that might help in debugging.
  {
    echo

    printf "%s\n" "## ---------------- ##
## Cache variables. ##
## ---------------- ##"
    echo
    # The following way of writing the cache mishandles newlines in values,
(
  for ac_var in `(set) 2>&1 | sed -n '\''s/^\([a-zA-Z_][a-zA-Z0-9_]*\)=.*/\1/p'\''`; do
    eval ac_val=\$$ac_var
    case $ac_val in #(
    *${as_nl}*)
      case $ac_var in #(
      *_cv_*) { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: cache variable $ac_var contains a newline" >&5
printf "%s\n" "$as_me: WARNING: cache variable $ac_var contains a newline" >&2;} ;;
      esac
      case $ac_var in #(
      _ | IFS | as_nl) ;; #(
      BASH_ARGV | BASH_SOURCE) eval $ac_var= ;; #(
      *) { eval $ac_var=; unset $ac_var;} ;;
      esac ;;
    esac
  done
  (set) 2>&1 |
    case $as_nl`(ac_space='\'' '\''; set) 2>&1` in #(
    *${as_nl}ac_space=\ *)
      sed -n \
	"s/'\''/'\''\\\\'\'''\''/g;
	  s/^\\([_$as_cr_alnum]*_cv_[_$as_cr_alnum]*\\)=\\(.*\\)/\\1='\''\\2'\''/p"
      ;; #(
    *)
      sed -n "/^[_$as_cr_alnum]*_cv_[_$as_cr_alnum]*=/p"
      ;;
    esac |
    sort
)
    echo

    printf "%s\n" "## ----------------- ##
## Output variables. ##
## ----------------- ##"
    echo
    for ac_var in $ac_subst_vars
    do
      eval ac_val=\$$ac_var
      case $ac_val in
      *\'\''*) ac_val=`printf "%s\n" "$ac_val" | sed "s/'\''/'\''\\\\\\\\'\'''\''/g"`;;
      esac
      printf "%s\n" "$ac_var='\''$ac_val'\''"
    done | sort
    echo

    if test -n "$ac_subst_files"; then
      printf "%s\n" "## ------------------- ##
## File substitutions. ##
## ------------------- ##"
      echo
      for ac_var in $ac_subst_files
      do
	eval ac_val=\$$ac_var
	case $ac_val in
	*\'\''*) ac_val=`printf "%s\n" "$ac_val" | sed "s/'\''/'\''\\\\\\\\'\'''\''/g"`;;
	esac
	printf "%s\n" "$ac_var='\''$ac_val'\''"
      done | sort
      echo
    fi

    if test -s confdefs.h; then
      printf "%s\n" "## ----------- ##
## confdefs.h. ##
## ----------- ##"
      echo
      cat confdefs.h
      echo
    fi
    test "$ac_signal" != 0 &&
      printf "%s\n" "$as_me: caught signal $ac_signal"
    printf "%s\n" "$as_me: exit $exit_status"
  } >&5
  rm -f core *.core core.conftest.* &&
    rm -f -r conftest* confdefs* conf$$* $ac_clean_files &&
    exit $exit_status
' 0
for ac_signal in 1 2 13 15; do
  trap 'ac_signal='$ac_signal'; as_fn_exit 1' $ac_signal
done
ac_signal=0

# confdefs.h avoids OS command line length limits that DEFS can exceed.
rm -f -r conftest* confdefs.h

printf "%s\n" "/* confdefs.h */" > confdefs.h

# Predefined preprocessor variables.

printf "%s\n" "#define PACKAGE_NAME \"$PACKAGE_NAME\"" >>confdefs.h

printf "%s\n" "#define PACKAGE_TARNAME \"$PACKAGE_TARNAME\"" >>confdefs.h

printf "%s\n" "#define PACKAGE_VERSION \"$PACKAGE_VERSION\"" >>confdefs.h

printf "%s\n" "#define PACKAGE_STRING \"$PACKAGE_STRING\"" >>confdefs.h

printf "%s\n" "#define PACKAGE_BUGREPORT \"$PACKAGE_BUGREPORT\"" >>confdefs.h

printf "%s\n" "#define PACKAGE_URL \"$PACKAGE_URL\"" >>confdefs.h


# Let the site file select an alternate cache file if it wants to.
# Prefer an explicitly selected file to automatically selected ones.
if test -n "$CONFIG_SITE"; then
  ac_site_files="$CONFIG_SITE"
elif test "x$prefix" != xNONE; then
  ac_site_files="$prefix/share/config.site $prefix/etc/config.site"
else
  ac_site_files="$ac_default_prefix/share/config.site $ac_default_prefix/etc/config.site"
fi

for ac_site_file in $ac_site_files
do
  case $ac_site_file in #(
  */*) :
     ;; #(
  *) :
    ac_site_file=./$ac_site_file ;;
esac
  if test -f "$ac_site_file" && test -r "$ac_site_file"; then
    { printf "%s\n" "$as_me:${as_lineno-$LINENO}: loading site script $ac_site_file" >&5
printf "%s\n" "$as_me: loading site script $ac_site_file" >&6;}
    sed 's/^/| /' "$ac_site_file" >&5
    . "$ac_site_file" \
      || { { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: in \`$ac_pwd':" >&5
printf "%s\n" "$as_me: error: in \`$ac_pwd':" >&2;}
as_fn_error $? "failed to load site script $ac_site_file
See \`config.log' for more details" "$LINENO" 5; }
  fi
done

if test -r "$cache_file"; then
  # Some versions of bash will fail to source /dev/null (special files
  # actually), so we avoid doing that.  DJGPP emulates it as a regular file.
  if test /dev/null != "$cache_file" && test -f "$cache_file"; then
    { printf "%s\n" "$as_me:${as_lineno-$LINENO}: loading cache $cache_file" >&5
printf "%s\n" "$as_me: loading cache $cache_file" >&6;}
    case $cache_file in
      [\\/]* | ?:[\\/]* ) . "$cache_file";;
      *)                      . "./$cache_file";;
    esac
  fi
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: creating cache $cache_file" >&5
printf "%s\n" "$as_me: creating cache $cache_file" >&6;}
  >$cache_file
fi

# Test code for whether the C compiler supports C89 (global declarations)
ac_c_conftest_c89_globals='
/* Does the compiler advertise C89 conformance?
   Do not test the value of __STDC__, because some compilers set it to 0
   while being otherwise adequately conformant. */
#if !defined __STDC__
# error "Compiler does not advertise C89 conformance"
#endif

#include <stddef.h>
#include <stdarg.h>
struct stat;
/* Most of the following tests are stolen from RCS 5.7 src/conf.sh.  */
struct buf { int x; };
struct buf * (*rcsopen) (struct buf *, struct stat *, int);
static char *e (p, i)
     char **p;
     int i;
{
  return p[i];
}
static char *f (char * (*g) (char **, int), char **p, ...)
{
  char *s;
  va_list v;
  va_start (v,p);
  s = g (p, va_arg (v,int));
  va_end (v);
  return s;
}

/* OSF 4.0 Compaq cc is some sort of almost-ANSI by default.  It has
   function prototypes and stuff, but not \xHH hex character constants.
   These do not provoke an error unfortunately, instead are silently treated
   as an "x".  The following induces an error, until -std is added to get
   proper ANSI mode.  Curiously \x00 != x always comes out true, for an
   array size at least.  It is necessary to write \x00 == 0 to get something
   that is true only with -std.  */
int osf4_cc_array ['\''\x00'\'' == 0 ? 1 : -1];

/* IBM C 6 for AIX is almost-ANSI by default, but it replaces macro parameters
   inside strings and character constants.  */
#define FOO(x) '\''x'\''
int xlc6_cc_array[FOO(a) == '\''x'\'' ? 1 : -1];

int test (int i, double x);
struct s1 {int (*f) (int a);};
struct s2 {int (*f) (double a);};
int pairnames (int, char **, int *(*)(struct buf *, struct stat *, int),
               int, int);'

# Test code for whether the C compiler supports C89 (body of main).
ac_c_conftest_c89_main='
ok |= (argc == 0 || f (e, argv, 0) != argv[0] || f (e, argv, 1) != argv[1]);
'

# Test code for whether the C compiler supports C99 (global declarations)
ac_c_conftest_c99_globals='
// Does the compiler advertise C99 conformance?
#if !defined __STDC_VERSION__ || __STDC_VERSION__ < 199901L
# error "Compiler does not advertise C99 conformance"
#endif

#include <stdbool.h>
extern int puts (const char *);
extern int printf (const char *, ...);
extern int dprintf (int, const char *, ...);
extern void *malloc (size_t);

// Check varargs macros.  These examples are taken from C99 6.10.3.5.
// dprintf is used instead of fprintf to avoid needing to declare
// FILE and stderr.
#define debug(...) dprintf (2, __VA_ARGS__)
#define showlist(...) puts (#__VA_ARGS__)
#define report(test,...) ((test) ? puts (#test) : printf (__VA_ARGS__))
static void
test_varargs_macros (void)
{
  int x = 1234;
  int y = 5678;
  debug ("Flag");
  debug ("X = %d\n", x);
  showlist (The first, second, and third items.);
  report (x>y, "x is %d but y is %d", x, y);
}

// Check long long types.
#define BIG64 18446744073709551615ull
#define BIG32 4294967295ul
#define BIG_OK (BIG64 / BIG32 == 4294967297ull && BIG64 % BIG32 == 0)
#if !BIG_OK
  #error "your preprocessor is broken"
#endif
#if BIG_OK
#else
  #error "your preprocessor is broken"
#endif
static long long int bignum = -9223372036854775807LL;
static unsigned long long int ubignum = BIG64;

struct incomplete_array
{
  int datasize;
  double data[];
};

struct named_init {
  int number;
  const wchar_t *name;
  double average;
};

typedef const char *ccp;

static inline int
test_restrict (ccp restrict text)
{
  // See if C++-style comments work.
  // Iterate through items via the restricted pointer.
  // Also check for declarations in for loops.
  for (unsigned int i = 0; *(text+i) != '\''\0'\''; ++i)
    continue;
  return 0;
}

// Check varargs and va_copy.
static bool
test_varargs (const char *format, ...)
{
  va_list args;
  va_start (args, format);
  va_list args_copy;
  va_copy (args_copy, args);

  const char *str = "";
  int number = 0;
  float fnumber = 0;

  while (*format)
    {
      switch (*format++)
	{
	case '\''s'\'': // string
	  str = va_arg (args_copy, const char *);
	  break;
	case '\''d'\'': // int
	  number = va_arg (args_copy, int);
	  break;
	case '\''f'\'': // float
	  fnumber = va_arg (args_copy, double);
	  break;
	default:
	  break;
	}
    }
  va_end (args_copy);
  va_end (args);

  return *str && number && fnumber;
}
'

# Test code for whether the C compiler supports C99 (body of main).
ac_c_conftest_c99_main='
  // Check bool.
  _Bool success = false;
  success |= (argc != 0);

  // Check restrict.
  if (test_restrict ("String literal") == 0)
    success = true;
  char *restrict newvar = "Another string";

  // Check varargs.
  success &= test_varargs ("s, d'\'' f .", "string", 65, 34.234);
  test_varargs_macros ();

  // Check flexible array members.
  struct incomplete_array *ia =
    malloc (sizeof (struct incomplete_array) + (sizeof (double) * 10));
  ia->datasize = 10;
  for (int i = 0; i < ia->datasize; ++i)
    ia->data[i] = i * 1.234;

  // Check named initializers.
  struct named_init ni = {
    .number = 34,
    .name = L"Test wide string",
    .average = 543.34343,
  };

  ni.number = 58;

  int dynamic_array[ni.number];
  dynamic_array[0] = argv[0][0];
  dynamic_array[ni.number - 1] = 543;

  // work around unused variable warnings
  ok |= (!success || bignum == 0LL || ubignum == 0uLL || newvar[0] == '\''x'\''
	 || dynamic_array[ni.number - 1] != 543);
'

# Test code for whether the C compiler supports C11 (global declarations)
ac_c_conftest_c11_globals='
// Does the compiler advertise C11 conformance?
#if !defined __STDC_VERSION__ || __STDC_VERSION__ < 201112L
# error "Compiler does not advertise C11 conformance"
#endif

// Check _Alignas.
char _Alignas (double) aligned_as_double;
char _Alignas (0) no_special_alignment;
extern char aligned_as_int;
char _Alignas (0) _Alignas (int) aligned_as_int;

// Check _Alignof.
enum
{
  int_alignment = _Alignof (int),
  int_array_alignment = _Alignof (int[100]),
  char_alignment = _Alignof (char)
};
_Static_assert (0 < -_Alignof (int), "_Alignof is signed");

// Check _Noreturn.
int _Noreturn does_not_return (void) { for (;;) continue; }

// Check _Static_assert.
struct test_static_assert
{
  int x;
  _Static_assert (sizeof (int) <= sizeof (long int),
                  "_Static_assert does not work in struct");
  long int y;
};

// Check UTF-8 literals.
#define u8 syntax error!
char const utf8_literal[] = u8"happens to be ASCII" "another string";

// Check duplicate typedefs.
typedef long *long_ptr;
typedef long int *long_ptr;
typedef long_ptr long_ptr;

// Anonymous structures and unions -- taken from C11 6.7.2.1 Example 1.
struct anonymous
{
  union {
    struct { int i; int j; };
    struct { int k; long int l; } w;
  };
  int m;
} v1;
'

# Test code for whether the C compiler supports C11 (body of main).
ac_c_conftest_c11_main='
  _Static_assert ((offsetof (struct anonymous, i)
		   == offsetof (struct anonymous, w.k)),
		  "Anonymous union alignment botch");
  v1.i = 2;
  v1.w.k = 5;
  ok |= v1.i != 5;
'

# Test code for whether the C compiler supports C11 (complete).
ac_c_conftest_c11_program="${ac_c_conftest_c89_globals}
${ac_c_conftest_c99_globals}
${ac_c_conftest_c11_globals}

int
main (int argc, char **argv)
{
  int ok = 0;
  ${ac_c_conftest_c89_main}
  ${ac_c_conftest_c99_main}
  ${ac_c_conftest_c11_main}
  return ok;
}
"

# Test code for whether the C compiler supports C99 (complete).
ac_c_conftest_c99_program="${ac_c_conftest_c89_globals}
${ac_c_conftest_c99_globals}

int
main (int argc, char **argv)
{
  int ok = 0;
  ${ac_c_conftest_c89_main}
  ${ac_c_conftest_c99_main}
  return ok;
}
"

# Test code for whether the C compiler supports C89 (complete).
ac_c_conftest_c89_program="${ac_c_conftest_c89_globals}

int
main (int argc, char **argv)
{
  int ok = 0;
  ${ac_c_conftest_c89_main}
  return ok;
}
"

as_fn_append ac_header_c_list " stdio.h stdio_h HAVE_STDIO_H"
as_fn_append ac_header_c_list " stdlib.h stdlib_h HAVE_STDLIB_H"
as_fn_append ac_header_c_list " string.h string_h HAVE_STRING_H"
as_fn_append ac_header_c_list " inttypes.h inttypes_h HAVE_INTTYPES_H"
as_fn_append ac_header_c_list " stdint.h stdint_h HAVE_STDINT_H"
as_fn_append ac_header_c_list " strings.h strings_h HAVE_STRINGS_H"
as_fn_append ac_header_c_list " sys/stat.h sys_stat_h HAVE_SYS_STAT_H"
as_fn_append ac_header_c_list " sys/types.h sys_types_h HAVE_SYS_TYPES_H"
as_fn_append ac_header_c_list " unistd.h unistd_h HAVE_UNISTD_H"
as_fn_append ac_func_c_list " vprintf HAVE_VPRINTF"

# Auxiliary files required by this configure script.
ac_aux_files="install-sh config.guess config.sub"

# Locations in which to look for auxiliary files.
ac_aux_dir_candidates="${srcdir}${PATH_SEPARATOR}${srcdir}/..${PATH_SEPARATOR}${srcdir}/../.."

# Search for a directory containing all of the required auxiliary files,
# $ac_aux_files, from the $PATH-style list $ac_aux_dir_candidates.
# If we don't find one directory that contains all the files we need,
# we report the set of missing files from the *first* directory in
# $ac_aux_dir_candidates and give up.
ac_missing_aux_files=""
ac_first_candidate=:
printf "%s\n" "$as_me:${as_lineno-$LINENO}: looking for aux files: $ac_aux_files" >&5
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
as_found=false
for as_dir in $ac_aux_dir_candidates
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
  as_found=:

  printf "%s\n" "$as_me:${as_lineno-$LINENO}:  trying $as_dir" >&5
  ac_aux_dir_found=yes
  ac_install_sh=
  for ac_aux in $ac_aux_files
  do
    # As a special case, if "install-sh" is required, that requirement
    # can be satisfied by any of "install-sh", "install.sh", or "shtool",
    # and $ac_install_sh is set appropriately for whichever one is found.
    if test x"$ac_aux" = x"install-sh"
    then
      if test -f "${as_dir}install-sh"; then
        printf "%s\n" "$as_me:${as_lineno-$LINENO}:   ${as_dir}install-sh found" >&5
        ac_install_sh="${as_dir}install-sh -c"
      elif test -f "${as_dir}install.sh"; then
        printf "%s\n" "$as_me:${as_lineno-$LINENO}:   ${as_dir}install.sh found" >&5
        ac_install_sh="${as_dir}install.sh -c"
      elif test -f "${as_dir}shtool"; then
        printf "%s\n" "$as_me:${as_lineno-$LINENO}:   ${as_dir}shtool found" >&5
        ac_install_sh="${as_dir}shtool install -c"
      else
        ac_aux_dir_found=no
        if $ac_first_candidate; then
          ac_missing_aux_files="${ac_missing_aux_files} install-sh"
        else
          break
        fi
      fi
    else
      if test -f "${as_dir}${ac_aux}"; then
        printf "%s\n" "$as_me:${as_lineno-$LINENO}:   ${as_dir}${ac_aux} found" >&5
      else
        ac_aux_dir_found=no
        if $ac_first_candidate; then
          ac_missing_aux_files="${ac_missing_aux_files} ${ac_aux}"
        else
          break
        fi
      fi
    fi
  done
  if test "$ac_aux_dir_found" = yes; then
    ac_aux_dir="$as_dir"
    break
  fi
  ac_first_candidate=false

  as_found=false
done
IFS=$as_save_IFS
if $as_found
then :

else $as_nop
  as_fn_error $? "cannot find required auxiliary files:$ac_missing_aux_files" "$LINENO" 5
fi


# These three variables are undocumented and unsupported,
# and are intended to be withdrawn in a future Autoconf release.
# They can cause serious problems if a builder's source tree is in a directory
# whose full name contains unusual characters.
if test -f "${ac_aux_dir}config.guess"; then
  ac_config_guess="$SHELL ${ac_aux_dir}config.guess"
fi
if test -f "${ac_aux_dir}config.sub"; then
  ac_config_sub="$SHELL ${ac_aux_dir}config.sub"
fi
if test -f "$ac_aux_dir/configure"; then
  ac_configure="$SHELL ${ac_aux_dir}configure"
fi

# Check that the precious variables saved in the cache have kept the same
# value.
ac_cache_corrupted=false
for ac_var in $ac_precious_vars; do
  eval ac_old_set=\$ac_cv_env_${ac_var}_set
  eval ac_new_set=\$ac_env_${ac_var}_set
  eval ac_old_val=\$ac_cv_env_${ac_var}_value
  eval ac_new_val=\$ac_env_${ac_var}_value
  case $ac_old_set,$ac_new_set in
    set,)
      { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: \`$ac_var' was set to \`$ac_old_val' in the previous run" >&5
printf "%s\n" "$as_me: error: \`$ac_var' was set to \`$ac_old_val' in the previous run" >&2;}
      ac_cache_corrupted=: ;;
    ,set)
      { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: \`$ac_var' was not set in the previous run" >&5
printf "%s\n" "$as_me: error: \`$ac_var' was not set in the previous run" >&2;}
      ac_cache_corrupted=: ;;
    ,);;
    *)
      if test "x$ac_old_val" != "x$ac_new_val"; then
	# differences in whitespace do not lead to failure.
	ac_old_val_w=`echo x $ac_old_val`
	ac_new_val_w=`echo x $ac_new_val`
	if test "$ac_old_val_w" != "$ac_new_val_w"; then
	  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: \`$ac_var' has changed since the previous run:" >&5
printf "%s\n" "$as_me: error: \`$ac_var' has changed since the previous run:" >&2;}
	  ac_cache_corrupted=:
	else
	  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: warning: ignoring whitespace changes in \`$ac_var' since the previous run:" >&5
printf "%s\n" "$as_me: warning: ignoring whitespace changes in \`$ac_var' since the previous run:" >&2;}
	  eval $ac_var=\$ac_old_val
	fi
	{ printf "%s\n" "$as_me:${as_lineno-$LINENO}:   former value:  \`$ac_old_val'" >&5
printf "%s\n" "$as_me:   former value:  \`$ac_old_val'" >&2;}
	{ printf "%s\n" "$as_me:${as_lineno-$LINENO}:   current value: \`$ac_new_val'" >&5
printf "%s\n" "$as_me:   current value: \`$ac_new_val'" >&2;}
      fi;;
  esac
  # Pass precious variables to config.status.
  if test "$ac_new_set" = set; then
    case $ac_new_val in
    *\'*) ac_arg=$ac_var=`printf "%s\n" "$ac_new_val" | sed "s/'/'\\\\\\\\''/g"` ;;
    *) ac_arg=$ac_var=$ac_new_val ;;
    esac
    case " $ac_configure_args " in
      *" '$ac_arg' "*) ;; # Avoid dups.  Use of quotes ensures accuracy.
      *) as_fn_append ac_configure_args " '$ac_arg'" ;;
    esac
  fi
done
if $ac_cache_corrupted; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: in \`$ac_pwd':" >&5
printf "%s\n" "$as_me: error: in \`$ac_pwd':" >&2;}
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: changes in the environment can compromise the build" >&5
printf "%s\n" "$as_me: error: changes in the environment can compromise the build" >&2;}
  as_fn_error $? "run \`${MAKE-make} distclean' and/or \`rm $cache_file'
	    and start over" "$LINENO" 5
fi
## -------------------- ##
## Main body of script. ##
## -------------------- ##

ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu








  # Make sure we can run config.sub.
$SHELL "${ac_aux_dir}config.sub" sun4 >/dev/null 2>&1 ||
  as_fn_error $? "cannot run $SHELL ${ac_aux_dir}config.sub" "$LINENO" 5

{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking build system type" >&5
printf %s "checking build system type... " >&6; }
if test ${ac_cv_build+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  ac_build_alias=$build_alias
test "x$ac_build_alias" = x &&
  ac_build_alias=`$SHELL "${ac_aux_dir}config.guess"`
test "x$ac_build_alias" = x &&
  as_fn_error $? "cannot guess build type; you must specify one" "$LINENO" 5
ac_cv_build=`$SHELL "${ac_aux_dir}config.sub" $ac_build_alias` ||
  as_fn_error $? "$SHELL ${ac_aux_dir}config.sub $ac_build_alias failed" "$LINENO" 5

fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_build" >&5
printf "%s\n" "$ac_cv_build" >&6; }
case $ac_cv_build in
*-*-*) ;;
*) as_fn_error $? "invalid value of canonical build" "$LINENO" 5;;
esac
build=$ac_cv_build
ac_save_IFS=$IFS; IFS='-'
set x $ac_cv_build
shift
build_cpu=$1
build_vendor=$2
shift; shift
# Remember, the first character of IFS is used to create $*,
# except with old shells:
build_os=$*
IFS=$ac_save_IFS
case $build_os in *\ *) build_os=`echo "$build_os" | sed 's/ /-/g'`;; esac


{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking host system type" >&5
printf %s "checking host system type... " >&6; }
if test ${ac_cv_host+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test "x$host_alias" = x; then
  ac_cv_host=$ac_cv_build
else
  ac_cv_host=`$SHELL "${ac_aux_dir}config.sub" $host_alias` ||
    as_fn_error $? "$SHELL ${ac_aux_dir}config.sub $host_alias failed" "$LINENO" 5
fi

fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_host" >&5
printf "%s\n" "$ac_cv_host" >&6; }
case $ac_cv_host in
*-*-*) ;;
*) as_fn_error $? "invalid value of canonical host" "$LINENO" 5;;
esac
host=$ac_cv_host
ac_save_IFS=$IFS; IFS='-'
set x $ac_cv_host
shift
host_cpu=$1
host_vendor=$2
shift; shift
# Remember, the first character of IFS is used to create $*,
# except with old shells:
host_os=$*
IFS=$ac_save_IFS
case $host_os in *\ *) host_os=`echo "$host_os" | sed 's/ /-/g'`;; esac


{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking target system type" >&5
printf %s "checking target system type... " >&6; }
if test ${ac_cv_target+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test "x$target_alias" = x; then
  ac_cv_target=$ac_cv_host
else
  ac_cv_target=`$SHELL "${ac_aux_dir}config.sub" $target_alias` ||
    as_fn_error $? "$SHELL ${ac_aux_dir}config.sub $target_alias failed" "$LINENO" 5
fi

fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_target" >&5
printf "%s\n" "$ac_cv_target" >&6; }
case $ac_cv_target in
*-*-*) ;;
*) as_fn_error $? "invalid value of canonical target" "$LINENO" 5;;
esac
target=$ac_cv_target
ac_save_IFS=$IFS; IFS='-'
set x $ac_cv_target
shift
target_cpu=$1
target_vendor=$2
shift; shift
# Remember, the first character of IFS is used to create $*,
# except with old shells:
target_os=$*
IFS=$ac_save_IFS
case $target_os in *\ *) target_os=`echo "$target_os" | sed 's/ /-/g'`;; esac


# The aliases save the names the user supplied, while $host etc.
# will get canonicalized.
test -n "$target_alias" &&
  test "$program_prefix$program_suffix$program_transform_name" = \
    NONENONEs,x,x, &&
  program_prefix=${target_alias}-











ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu
if test -n "$ac_tool_prefix"; then
  # Extract the first word of "${ac_tool_prefix}gcc", so it can be a program name with args.
set dummy ${ac_tool_prefix}gcc; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_CC+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    ac_cv_prog_CC="${ac_tool_prefix}gcc"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $CC" >&5
printf "%s\n" "$CC" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi


fi
if test -z "$ac_cv_prog_CC"; then
  ac_ct_CC=$CC
  # Extract the first word of "gcc", so it can be a program name with args.
set dummy gcc; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_ac_ct_CC+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$ac_ct_CC"; then
  ac_cv_prog_ac_ct_CC="$ac_ct_CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    ac_cv_prog_ac_ct_CC="gcc"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

fi
fi
ac_ct_CC=$ac_cv_prog_ac_ct_CC
if test -n "$ac_ct_CC"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_ct_CC" >&5
printf "%s\n" "$ac_ct_CC" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi

  if test "x$ac_ct_CC" = x; then
    CC=""
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: using cross tools not prefixed with host triplet" >&5
printf "%s\n" "$as_me: WARNING: using cross tools not prefixed with host triplet" >&2;}
ac_tool_warned=yes ;;
esac
    CC=$ac_ct_CC
  fi
else
  CC="$ac_cv_prog_CC"
fi

if test -z "$CC"; then
          if test -n "$ac_tool_prefix"; then
    # Extract the first word of "${ac_tool_prefix}cc", so it can be a program name with args.
set dummy ${ac_tool_prefix}cc; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_CC+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    ac_cv_prog_CC="${ac_tool_prefix}cc"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $CC" >&5
printf "%s\n" "$CC" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi


  fi
fi
if test -z "$CC"; then
  # Extract the first word of "cc", so it can be a program name with args.
set dummy cc; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_CC+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
  ac_prog_rejected=no
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    if test "$as_dir$ac_word$ac_exec_ext" = "/usr/ucb/cc"; then
       ac_prog_rejected=yes
       continue
     fi
    ac_cv_prog_CC="cc"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

if test $ac_prog_rejected = yes; then
  # We found a bogon in the path, so make sure we never use it.
  set dummy $ac_cv_prog_CC
  shift
  if test $# != 0; then
    # We chose a different compiler from the bogus one.
    # However, it has the same basename, so the bogon will be chosen
    # first if we set CC to just the basename; use the full file name.
    shift
    ac_cv_prog_CC="$as_dir$ac_word${1+' '}$@"
  fi
fi
fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $CC" >&5
printf "%s\n" "$CC" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi


fi
if test -z "$CC"; then
  if test -n "$ac_tool_prefix"; then
  for ac_prog in cl.exe
  do
    # Extract the first word of "$ac_tool_prefix$ac_prog", so it can be a program name with args.
set dummy $ac_tool_prefix$ac_prog; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_CC+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    ac_cv_prog_CC="$ac_tool_prefix$ac_prog"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $CC" >&5
printf "%s\n" "$CC" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi


    test -n "$CC" && break
  done
fi
if test -z "$CC"; then
  ac_ct_CC=$CC
  for ac_prog in cl.exe
do
  # Extract the first word of "$ac_prog", so it can be a program name with args.
set dummy $ac_prog; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_ac_ct_CC+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$ac_ct_CC"; then
  ac_cv_prog_ac_ct_CC="$ac_ct_CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    ac_cv_prog_ac_ct_CC="$ac_prog"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

fi
fi
ac_ct_CC=$ac_cv_prog_ac_ct_CC
if test -n "$ac_ct_CC"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_ct_CC" >&5
printf "%s\n" "$ac_ct_CC" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi


  test -n "$ac_ct_CC" && break
done

  if test "x$ac_ct_CC" = x; then
    CC=""
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: using cross tools not prefixed with host triplet" >&5
printf "%s\n" "$as_me: WARNING: using cross tools not prefixed with host triplet" >&2;}
ac_tool_warned=yes ;;
esac
    CC=$ac_ct_CC
  fi
fi

fi
if test -z "$CC"; then
  if test -n "$ac_tool_prefix"; then
  # Extract the first word of "${ac_tool_prefix}clang", so it can be a program name with args.
set dummy ${ac_tool_prefix}clang; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_CC+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$CC"; then
  ac_cv_prog_CC="$CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    ac_cv_prog_CC="${ac_tool_prefix}clang"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

fi
fi
CC=$ac_cv_prog_CC
if test -n "$CC"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $CC" >&5
printf "%s\n" "$CC" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi


fi
if test -z "$ac_cv_prog_CC"; then
  ac_ct_CC=$CC
  # Extract the first word of "clang", so it can be a program name with args.
set dummy clang; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_ac_ct_CC+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$ac_ct_CC"; then
  ac_cv_prog_ac_ct_CC="$ac_ct_CC" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    ac_cv_prog_ac_ct_CC="clang"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

fi
fi
ac_ct_CC=$ac_cv_prog_ac_ct_CC
if test -n "$ac_ct_CC"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_ct_CC" >&5
printf "%s\n" "$ac_ct_CC" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi

  if test "x$ac_ct_CC" = x; then
    CC=""
  else
    case $cross_compiling:$ac_tool_warned in
yes:)
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: using cross tools not prefixed with host triplet" >&5
printf "%s\n" "$as_me: WARNING: using cross tools not prefixed with host triplet" >&2;}
ac_tool_warned=yes ;;
esac
    CC=$ac_ct_CC
  fi
else
  CC="$ac_cv_prog_CC"
fi

fi


test -z "$CC" && { { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: in \`$ac_pwd':" >&5
printf "%s\n" "$as_me: error: in \`$ac_pwd':" >&2;}
as_fn_error $? "no acceptable C compiler found in \$PATH
See \`config.log' for more details" "$LINENO" 5; }

# Provide some information about the compiler.
printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for C compiler version" >&5
set X $ac_compile
ac_compiler=$2
for ac_option in --version -v -V -qversion -version; do
  { { ac_try="$ac_compiler $ac_option >&5"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval ac_try_echo="\"\$as_me:${as_lineno-$LINENO}: $ac_try_echo\""
printf "%s\n" "$ac_try_echo"; } >&5
  (eval "$ac_compiler $ac_option >&5") 2>conftest.err
  ac_status=$?
  if test -s conftest.err; then
    sed '10a\
... rest of stderr output deleted ...
         10q' conftest.err >conftest.er1
    cat conftest.er1 >&5
  fi
  rm -f conftest.er1 conftest.err
  printf "%s\n" "$as_me:${as_lineno-$LINENO}: \$? = $ac_status" >&5
  test $ac_status = 0; }
done

cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

int
main (void)
{

  ;
  return 0;
}
_ACEOF
ac_clean_files_save=$ac_clean_files
ac_clean_files="$ac_clean_files a.out a.out.dSYM a.exe b.out"
# Try to create an executable without -o first, disregard a.out.
# It will help us diagnose broken compilers, and finding out an intuition
# of exeext.
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking whether the C compiler works" >&5
printf %s "checking whether the C compiler works... " >&6; }
ac_link_default=`printf "%s\n" "$ac_link" | sed 's/ -o *conftest[^ ]*//'`

# The possible output files:
ac_files="a.out conftest.exe conftest a.exe a_out.exe b.out conftest.*"

ac_rmfiles=
for ac_file in $ac_files
do
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.dSYM | *.o | *.obj ) ;;
    * ) ac_rmfiles="$ac_rmfiles $ac_file";;
  esac
done
rm -f $ac_rmfiles

if { { ac_try="$ac_link_default"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval ac_try_echo="\"\$as_me:${as_lineno-$LINENO}: $ac_try_echo\""
printf "%s\n" "$ac_try_echo"; } >&5
  (eval "$ac_link_default") 2>&5
  ac_status=$?
  printf "%s\n" "$as_me:${as_lineno-$LINENO}: \$? = $ac_status" >&5
  test $ac_status = 0; }
then :
  # Autoconf-2.13 could set the ac_cv_exeext variable to `no'.
# So ignore a value of `no', otherwise this would lead to `EXEEXT = no'
# in a Makefile.  We should not override ac_cv_exeext if it was cached,
# so that the user can short-circuit this test for compilers unknown to
# Autoconf.
for ac_file in $ac_files ''
do
  test -f "$ac_file" || continue
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.dSYM | *.o | *.obj )
	;;
    [ab].out )
	# We found the default executable, but exeext='' is most
	# certainly right.
	break;;
    *.* )
	if test ${ac_cv_exeext+y} && test "$ac_cv_exeext" != no;
	then :; else
	   ac_cv_exeext=`expr "$ac_file" : '[^.]*\(\..*\)'`
	fi
	# We set ac_cv_exeext here because the later test for it is not
	# safe: cross compilers may not add the suffix if given an `-o'
	# argument, so we may need to know it at that point already.
	# Even if this section looks crufty: it has the advantage of
	# actually working.
	break;;
    * )
	break;;
  esac
done
test "$ac_cv_exeext" = no && ac_cv_exeext=

else $as_nop
  ac_file=''
fi
if test -z "$ac_file"
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
printf "%s\n" "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

{ { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: in \`$ac_pwd':" >&5
printf "%s\n" "$as_me: error: in \`$ac_pwd':" >&2;}
as_fn_error 77 "C compiler cannot create executables
See \`config.log' for more details" "$LINENO" 5; }
else $as_nop
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: yes" >&5
printf "%s\n" "yes" >&6; }
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for C compiler default output file name" >&5
printf %s "checking for C compiler default output file name... " >&6; }
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_file" >&5
printf "%s\n" "$ac_file" >&6; }
ac_exeext=$ac_cv_exeext

rm -f -r a.out a.out.dSYM a.exe conftest$ac_cv_exeext b.out
ac_clean_files=$ac_clean_files_save
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for suffix of executables" >&5
printf %s "checking for suffix of executables... " >&6; }
if { { ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval ac_try_echo="\"\$as_me:${as_lineno-$LINENO}: $ac_try_echo\""
printf "%s\n" "$ac_try_echo"; } >&5
  (eval "$ac_link") 2>&5
  ac_status=$?
  printf "%s\n" "$as_me:${as_lineno-$LINENO}: \$? = $ac_status" >&5
  test $ac_status = 0; }
then :
  # If both `conftest.exe' and `conftest' are `present' (well, observable)
# catch `conftest.exe'.  For instance with Cygwin, `ls conftest' will
# work properly (i.e., refer to `conftest.exe'), while it won't with
# `rm'.
for ac_file in conftest.exe conftest conftest.*; do
  test -f "$ac_file" || continue
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.dSYM | *.o | *.obj ) ;;
    *.* ) ac_cv_exeext=`expr "$ac_file" : '[^.]*\(\..*\)'`
	  break;;
    * ) break;;
  esac
done
else $as_nop
  { { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: in \`$ac_pwd':" >&5
printf "%s\n" "$as_me: error: in \`$ac_pwd':" >&2;}
as_fn_error $? "cannot compute suffix of executables: cannot compile and link
See \`config.log' for more details" "$LINENO" 5; }
fi
rm -f conftest conftest$ac_cv_exeext
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_exeext" >&5
printf "%s\n" "$ac_cv_exeext" >&6; }

rm -f conftest.$ac_ext
EXEEXT=$ac_cv_exeext
ac_exeext=$EXEEXT
cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */
#include <stdio.h>
int
main (void)
{
FILE *f = fopen ("conftest.out", "w");
 return ferror (f) || fclose (f) != 0;

  ;
  return 0;
}
_ACEOF
ac_clean_files="$ac_clean_files conftest.out"
# Check that the compiler produces executables we can run.  If not, either
# the compiler is broken, or we cross compile.
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking whether we are cross compiling" >&5
printf %s "checking whether we are cross compiling... " >&6; }
if test "$cross_compiling" != yes; then
  { { ac_try="$ac_link"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval ac_try_echo="\"\$as_me:${as_lineno-$LINENO}: $ac_try_echo\""
printf "%s\n" "$ac_try_echo"; } >&5
  (eval "$ac_link") 2>&5
  ac_status=$?
  printf "%s\n" "$as_me:${as_lineno-$LINENO}: \$? = $ac_status" >&5
  test $ac_status = 0; }
  if { ac_try='./conftest$ac_cv_exeext'
  { { case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval ac_try_echo="\"\$as_me:${as_lineno-$LINENO}: $ac_try_echo\""
printf "%s\n" "$ac_try_echo"; } >&5
  (eval "$ac_try") 2>&5
  ac_status=$?
  printf "%s\n" "$as_me:${as_lineno-$LINENO}: \$? = $ac_status" >&5
  test $ac_status = 0; }; }; then
    cross_compiling=no
  else
    if test "$cross_compiling" = maybe; then
	cross_compiling=yes
    else
	{ { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: in \`$ac_pwd':" >&5
printf "%s\n" "$as_me: error: in \`$ac_pwd':" >&2;}
as_fn_error 77 "cannot run C compiled programs.
If you meant to cross compile, use \`--host'.
See \`config.log' for more details" "$LINENO" 5; }
    fi
  fi
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $cross_compiling" >&5
printf "%s\n" "$cross_compiling" >&6; }

rm -f conftest.$ac_ext conftest$ac_cv_exeext conftest.out
ac_clean_files=$ac_clean_files_save
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for suffix of object files" >&5
printf %s "checking for suffix of object files... " >&6; }
if test ${ac_cv_objext+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

int
main (void)
{

  ;
  return 0;
}
_ACEOF
rm -f conftest.o conftest.obj
if { { ac_try="$ac_compile"
case "(($ac_try" in
  *\"* | *\`* | *\\*) ac_try_echo=\$ac_try;;
  *) ac_try_echo=$ac_try;;
esac
eval ac_try_echo="\"\$as_me:${as_lineno-$LINENO}: $ac_try_echo\""
printf "%s\n" "$ac_try_echo"; } >&5
  (eval "$ac_compile") 2>&5
  ac_status=$?
  printf "%s\n" "$as_me:${as_lineno-$LINENO}: \$? = $ac_status" >&5
  test $ac_status = 0; }
then :
  for ac_file in conftest.o conftest.obj conftest.*; do
  test -f "$ac_file" || continue;
  case $ac_file in
    *.$ac_ext | *.xcoff | *.tds | *.d | *.pdb | *.xSYM | *.bb | *.bbg | *.map | *.inf | *.dSYM ) ;;
    *) ac_cv_objext=`expr "$ac_file" : '.*\.\(.*\)'`
       break;;
  esac
done
else $as_nop
  printf "%s\n" "$as_me: failed program was:" >&5
sed 's/^/| /' conftest.$ac_ext >&5

{ { printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: in \`$ac_pwd':" >&5
printf "%s\n" "$as_me: error: in \`$ac_pwd':" >&2;}
as_fn_error $? "cannot compute suffix of object files: cannot compile
See \`config.log' for more details" "$LINENO" 5; }
fi
rm -f conftest.$ac_cv_objext conftest.$ac_ext
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_objext" >&5
printf "%s\n" "$ac_cv_objext" >&6; }
OBJEXT=$ac_cv_objext
ac_objext=$OBJEXT
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking whether the compiler supports GNU C" >&5
printf %s "checking whether the compiler supports GNU C... " >&6; }
if test ${ac_cv_c_compiler_gnu+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

int
main (void)
{
#ifndef __GNUC__
       choke me
#endif

  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_compile "$LINENO"
then :
  ac_compiler_gnu=yes
else $as_nop
  ac_compiler_gnu=no
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam conftest.$ac_ext
ac_cv_c_compiler_gnu=$ac_compiler_gnu

fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_c_compiler_gnu" >&5
printf "%s\n" "$ac_cv_c_compiler_gnu" >&6; }
ac_compiler_gnu=$ac_cv_c_compiler_gnu

if test $ac_compiler_gnu = yes; then
  GCC=yes
else
  GCC=
fi
ac_test_CFLAGS=${CFLAGS+y}
ac_save_CFLAGS=$CFLAGS
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking whether $CC accepts -g" >&5
printf %s "checking whether $CC accepts -g... " >&6; }
if test ${ac_cv_prog_cc_g+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  ac_save_c_werror_flag=$ac_c_werror_flag
   ac_c_werror_flag=yes
   ac_cv_prog_cc_g=no
   CFLAGS="-g"
   cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

int
main (void)
{

  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_compile "$LINENO"
then :
  ac_cv_prog_cc_g=yes
else $as_nop
  CFLAGS=""
      cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

int
main (void)
{

  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_compile "$LINENO"
then :

else $as_nop
  ac_c_werror_flag=$ac_save_c_werror_flag
	 CFLAGS="-g"
	 cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

int
main (void)
{

  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_compile "$LINENO"
then :
  ac_cv_prog_cc_g=yes
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam conftest.$ac_ext
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam conftest.$ac_ext
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam conftest.$ac_ext
   ac_c_werror_flag=$ac_save_c_werror_flag
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_prog_cc_g" >&5
printf "%s\n" "$ac_cv_prog_cc_g" >&6; }
if test $ac_test_CFLAGS; then
  CFLAGS=$ac_save_CFLAGS
elif test $ac_cv_prog_cc_g = yes; then
  if test "$GCC" = yes; then
    CFLAGS="-g -O2"
  else
    CFLAGS="-g"
  fi
else
  if test "$GCC" = yes; then
    CFLAGS="-O2"
  else
    CFLAGS=
  fi
fi
ac_prog_cc_stdc=no
if test x$ac_prog_cc_stdc = xno
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $CC option to enable C11 features" >&5
printf %s "checking for $CC option to enable C11 features... " >&6; }
if test ${ac_cv_prog_cc_c11+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  ac_cv_prog_cc_c11=no
ac_save_CC=$CC
cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */
$ac_c_conftest_c11_program
_ACEOF
for ac_arg in '' -std=gnu11
do
  CC="$ac_save_CC $ac_arg"
  if ac_fn_c_try_compile "$LINENO"
then :
  ac_cv_prog_cc_c11=$ac_arg
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam
  test "x$ac_cv_prog_cc_c11" != "xno" && break
done
rm -f conftest.$ac_ext
CC=$ac_save_CC
fi

if test "x$ac_cv_prog_cc_c11" = xno
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: unsupported" >&5
printf "%s\n" "unsupported" >&6; }
else $as_nop
  if test "x$ac_cv_prog_cc_c11" = x
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: none needed" >&5
printf "%s\n" "none needed" >&6; }
else $as_nop
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_prog_cc_c11" >&5
printf "%s\n" "$ac_cv_prog_cc_c11" >&6; }
     CC="$CC $ac_cv_prog_cc_c11"
fi
  ac_cv_prog_cc_stdc=$ac_cv_prog_cc_c11
  ac_prog_cc_stdc=c11
fi
fi
if test x$ac_prog_cc_stdc = xno
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $CC option to enable C99 features" >&5
printf %s "checking for $CC option to enable C99 features... " >&6; }
if test ${ac_cv_prog_cc_c99+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  ac_cv_prog_cc_c99=no
ac_save_CC=$CC
cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */
$ac_c_conftest_c99_program
_ACEOF
for ac_arg in '' -std=gnu99 -std=c99 -c99 -qlanglvl=extc1x -qlanglvl=extc99 -AC99 -D_STDC_C99=
do
  CC="$ac_save_CC $ac_arg"
  if ac_fn_c_try_compile "$LINENO"
then :
  ac_cv_prog_cc_c99=$ac_arg
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam
  test "x$ac_cv_prog_cc_c99" != "xno" && break
done
rm -f conftest.$ac_ext
CC=$ac_save_CC
fi

if test "x$ac_cv_prog_cc_c99" = xno
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: unsupported" >&5
printf "%s\n" "unsupported" >&6; }
else $as_nop
  if test "x$ac_cv_prog_cc_c99" = x
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: none needed" >&5
printf "%s\n" "none needed" >&6; }
else $as_nop
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_prog_cc_c99" >&5
printf "%s\n" "$ac_cv_prog_cc_c99" >&6; }
     CC="$CC $ac_cv_prog_cc_c99"
fi
  ac_cv_prog_cc_stdc=$ac_cv_prog_cc_c99
  ac_prog_cc_stdc=c99
fi
fi
if test x$ac_prog_cc_stdc = xno
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $CC option to enable C89 features" >&5
printf %s "checking for $CC option to enable C89 features... " >&6; }
if test ${ac_cv_prog_cc_c89+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  ac_cv_prog_cc_c89=no
ac_save_CC=$CC
cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */
$ac_c_conftest_c89_program
_ACEOF
for ac_arg in '' -qlanglvl=extc89 -qlanglvl=ansi -std -Ae "-Aa -D_HPUX_SOURCE" "-Xc -D__EXTENSIONS__"
do
  CC="$ac_save_CC $ac_arg"
  if ac_fn_c_try_compile "$LINENO"
then :
  ac_cv_prog_cc_c89=$ac_arg
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam
  test "x$ac_cv_prog_cc_c89" != "xno" && break
done
rm -f conftest.$ac_ext
CC=$ac_save_CC
fi

if test "x$ac_cv_prog_cc_c89" = xno
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: unsupported" >&5
printf "%s\n" "unsupported" >&6; }
else $as_nop
  if test "x$ac_cv_prog_cc_c89" = x
then :
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: none needed" >&5
printf "%s\n" "none needed" >&6; }
else $as_nop
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_prog_cc_c89" >&5
printf "%s\n" "$ac_cv_prog_cc_c89" >&6; }
     CC="$CC $ac_cv_prog_cc_c89"
fi
  ac_cv_prog_cc_stdc=$ac_cv_prog_cc_c89
  ac_prog_cc_stdc=c89
fi
fi

ac_ext=c
ac_cpp='$CPP $CPPFLAGS'
ac_compile='$CC -c $CFLAGS $CPPFLAGS conftest.$ac_ext >&5'
ac_link='$CC -o conftest$ac_exeext $CFLAGS $CPPFLAGS $LDFLAGS conftest.$ac_ext $LIBS >&5'
ac_compiler_gnu=$ac_cv_c_compiler_gnu




# Check whether --with-kpathsea-include was given.
if test ${with_kpathsea_include+y}
then :
  withval=$with_kpathsea_include;
  if test x$withval = xyes; then
    { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: Usage is: --with-kpathsea-include=includedir" >&5
printf "%s\n" "$as_me: WARNING: Usage is: --with-kpathsea-include=includedir" >&2;}
  else
    if test x$withval = xno; then
      { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: Usage is: --with-kpathsea-include=includedir" >&5
printf "%s\n" "$as_me: WARNING: Usage is: --with-kpathsea-include=includedir" >&2;}
    else
      kpathsea_include=$withval
    fi
  fi

fi




# Check whether --with-kpathsea-lib was given.
if test ${with_kpathsea_lib+y}
then :
  withval=$with_kpathsea_lib;
  if test x$withval = xyes; then
    { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: Usage is: --with-kpathsea-lib=libdir" >&5
printf "%s\n" "$as_me: WARNING: Usage is: --with-kpathsea-lib=libdir" >&2;}
  else
    if test x$withval = xno; then
      { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: Usage is: --with-kpathsea-lib=libdir" >&5
printf "%s\n" "$as_me: WARNING: Usage is: --with-kpathsea-lib=libdir" >&2;}
    else
      kpathsea_lib=$withval
    fi
  fi

fi



if test -n "$kpathsea_include" -o -n "$kpathsea_lib"; then
  LIBS="$LIBS -L$kpathsea_lib"
  CPPFLAGS="$CPPFLAGS -I$kpathsea_include -I$srcdir"


{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for kpse_set_program_name in -lkpathsea" >&5
printf %s "checking for kpse_set_program_name in -lkpathsea... " >&6; }
if test ${ac_cv_lib_kpathsea_kpse_set_program_name+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lkpathsea  $LIBS"
cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
char kpse_set_program_name ();
int
main (void)
{
return kpse_set_program_name ();
  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_link "$LINENO"
then :
  ac_cv_lib_kpathsea_kpse_set_program_name=yes
else $as_nop
  ac_cv_lib_kpathsea_kpse_set_program_name=no
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam \
    conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_lib_kpathsea_kpse_set_program_name" >&5
printf "%s\n" "$ac_cv_lib_kpathsea_kpse_set_program_name" >&6; }
if test "x$ac_cv_lib_kpathsea_kpse_set_program_name" = xyes
then :
  printf "%s\n" "#define HAVE_LIBKPATHSEA 1" >>confdefs.h

  LIBS="-lkpathsea $LIBS"

else $as_nop
  printf "%s\n" "#define OLD_KPATHSEA 1" >>confdefs.h

fi


  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for kpse_init_prog in -lkpathsea" >&5
printf %s "checking for kpse_init_prog in -lkpathsea... " >&6; }
if test ${ac_cv_lib_kpathsea_kpse_init_prog+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  ac_check_lib_save_LIBS=$LIBS
LIBS="-lkpathsea  $LIBS"
cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

/* Override any GCC internal prototype to avoid an error.
   Use char because int might match the return type of a GCC
   builtin and then its argument prototype would still apply.  */
char kpse_init_prog ();
int
main (void)
{
return kpse_init_prog ();
  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_link "$LINENO"
then :
  ac_cv_lib_kpathsea_kpse_init_prog=yes
else $as_nop
  ac_cv_lib_kpathsea_kpse_init_prog=no
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam \
    conftest$ac_exeext conftest.$ac_ext
LIBS=$ac_check_lib_save_LIBS
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_lib_kpathsea_kpse_init_prog" >&5
printf "%s\n" "$ac_cv_lib_kpathsea_kpse_init_prog" >&6; }
if test "x$ac_cv_lib_kpathsea_kpse_init_prog" = xyes
then :
  printf "%s\n" "#define HAVE_LIBKPATHSEA 1" >>confdefs.h

  LIBS="-lkpathsea $LIBS"

else $as_nop

               as_fn_error $? "Can't find kpathsea library! Use --with-kpathsea-lib option." "$LINENO" 5
fi


    ac_header= ac_cache=
for ac_item in $ac_header_c_list
do
  if test $ac_cache; then
    ac_fn_c_check_header_compile "$LINENO" $ac_header ac_cv_header_$ac_cache "$ac_includes_default"
    if eval test \"x\$ac_cv_header_$ac_cache\" = xyes; then
      printf "%s\n" "#define $ac_item 1" >> confdefs.h
    fi
    ac_header= ac_cache=
  elif test $ac_header; then
    ac_cache=$ac_item
  else
    ac_header=$ac_item
  fi
done








if test $ac_cv_header_stdlib_h = yes && test $ac_cv_header_string_h = yes
then :

printf "%s\n" "#define STDC_HEADERS 1" >>confdefs.h

fi
ac_fn_c_check_header_compile "$LINENO" "kpathsea/kpathsea.h" "ac_cv_header_kpathsea_kpathsea_h" "$ac_includes_default"
if test "x$ac_cv_header_kpathsea_kpathsea_h" = xyes
then :

else $as_nop
  printf "%s\n" "#define VERY_OLD_KPATHSEA 1" >>confdefs.h

fi


  ac_fn_c_check_header_compile "$LINENO" "kpathsea/c-auto.h" "ac_cv_header_kpathsea_c_auto_h" "$ac_includes_default"
if test "x$ac_cv_header_kpathsea_c_auto_h" = xyes
then :

else $as_nop

                  as_fn_error $? "Can't find kpathsea include files! Use --with-kpathsea-include option." "$LINENO" 5
fi

else
  CPPFLAGS="$CPPFLAGS -I$srcdir"
fi


if test "x$CC" = xgcc; then
	XX_CFLAGS="-Wall"
else
	case "$host" in
  		alpha-dec-osf*)
        	XX_CFLAGS="-std1 -O2 -g3"
       		;;
  		*)
          	XX_CFLAGS=
       		;;
	esac
fi



{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for an ANSI C-conforming const" >&5
printf %s "checking for an ANSI C-conforming const... " >&6; }
if test ${ac_cv_c_const+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */

int
main (void)
{

#ifndef __cplusplus
  /* Ultrix mips cc rejects this sort of thing.  */
  typedef int charset[2];
  const charset cs = { 0, 0 };
  /* SunOS 4.1.1 cc rejects this.  */
  char const *const *pcpcc;
  char **ppc;
  /* NEC SVR4.0.2 mips cc rejects this.  */
  struct point {int x, y;};
  static struct point const zero = {0,0};
  /* IBM XL C 1.02.0.0 rejects this.
     It does not let you subtract one const X* pointer from another in
     an arm of an if-expression whose if-part is not a constant
     expression */
  const char *g = "string";
  pcpcc = &g + (g ? g-g : 0);
  /* HPUX 7.0 cc rejects these. */
  ++pcpcc;
  ppc = (char**) pcpcc;
  pcpcc = (char const *const *) ppc;
  { /* SCO 3.2v4 cc rejects this sort of thing.  */
    char tx;
    char *t = &tx;
    char const *s = 0 ? (char *) 0 : (char const *) 0;

    *t++ = 0;
    if (s) return 0;
  }
  { /* Someone thinks the Sun supposedly-ANSI compiler will reject this.  */
    int x[] = {25, 17};
    const int *foo = &x[0];
    ++foo;
  }
  { /* Sun SC1.0 ANSI compiler rejects this -- but not the above. */
    typedef const int *iptr;
    iptr p = 0;
    ++p;
  }
  { /* IBM XL C 1.02.0.0 rejects this sort of thing, saying
       "k.c", line 2.27: 1506-025 (S) Operand must be a modifiable lvalue. */
    struct s { int j; const int *ap[3]; } bx;
    struct s *b = &bx; b->j = 5;
  }
  { /* ULTRIX-32 V3.1 (Rev 9) vcc rejects this */
    const int foo = 10;
    if (!foo) return 0;
  }
  return !cs[0] && !zero.x;
#endif

  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_compile "$LINENO"
then :
  ac_cv_c_const=yes
else $as_nop
  ac_cv_c_const=no
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam conftest.$ac_ext
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_c_const" >&5
printf "%s\n" "$ac_cv_c_const" >&6; }
if test $ac_cv_c_const = no; then

printf "%s\n" "#define const /**/" >>confdefs.h

fi

{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking whether struct tm is in sys/time.h or time.h" >&5
printf %s "checking whether struct tm is in sys/time.h or time.h... " >&6; }
if test ${ac_cv_struct_tm+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  cat confdefs.h - <<_ACEOF >conftest.$ac_ext
/* end confdefs.h.  */
#include <sys/types.h>
#include <time.h>

int
main (void)
{
struct tm tm;
				     int *p = &tm.tm_sec;
				     return !p;
  ;
  return 0;
}
_ACEOF
if ac_fn_c_try_compile "$LINENO"
then :
  ac_cv_struct_tm=time.h
else $as_nop
  ac_cv_struct_tm=sys/time.h
fi
rm -f core conftest.err conftest.$ac_objext conftest.beam conftest.$ac_ext
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $ac_cv_struct_tm" >&5
printf "%s\n" "$ac_cv_struct_tm" >&6; }
if test $ac_cv_struct_tm = sys/time.h; then

printf "%s\n" "#define TM_IN_SYS_TIME 1" >>confdefs.h

fi



ac_func=
for ac_item in $ac_func_c_list
do
  if test $ac_func; then
    ac_fn_c_check_func "$LINENO" $ac_func ac_cv_func_$ac_func
    if eval test \"x\$ac_cv_func_$ac_func\" = xyes; then
      echo "#define $ac_item 1" >> confdefs.h
    fi
    ac_func=
  else
    ac_func=$ac_item
  fi
done

if test "x$ac_cv_func_vprintf" = xno
then :
  ac_fn_c_check_func "$LINENO" "_doprnt" "ac_cv_func__doprnt"
if test "x$ac_cv_func__doprnt" = xyes
then :

printf "%s\n" "#define HAVE_DOPRNT 1" >>confdefs.h

fi

fi
ac_fn_c_check_func "$LINENO" "strdup" "ac_cv_func_strdup"
if test "x$ac_cv_func_strdup" = xyes
then :
  printf "%s\n" "#define HAVE_STRDUP 1" >>confdefs.h

fi
ac_fn_c_check_func "$LINENO" "strstr" "ac_cv_func_strstr"
if test "x$ac_cv_func_strstr" = xyes
then :
  printf "%s\n" "#define HAVE_STRSTR 1" >>confdefs.h

fi
ac_fn_c_check_func "$LINENO" "strtol" "ac_cv_func_strtol"
if test "x$ac_cv_func_strtol" = xyes
then :
  printf "%s\n" "#define HAVE_STRTOL 1" >>confdefs.h

fi
ac_fn_c_check_func "$LINENO" "strtoul" "ac_cv_func_strtoul"
if test "x$ac_cv_func_strtoul" = xyes
then :
  printf "%s\n" "#define HAVE_STRTOUL 1" >>confdefs.h

fi


if test "x$ac_cv_func_strdup" = xno; then
  no_strdup=-DNO_STRDUP
fi


# Extract the first word of "rm", so it can be a program name with args.
set dummy rm; ac_word=$2
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for $ac_word" >&5
printf %s "checking for $ac_word... " >&6; }
if test ${ac_cv_prog_RM+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  if test -n "$RM"; then
  ac_cv_prog_RM="$RM" # Let the user override the test.
else
as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    for ac_exec_ext in '' $ac_executable_extensions; do
  if as_fn_executable_p "$as_dir$ac_word$ac_exec_ext"; then
    ac_cv_prog_RM="rm"
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: found $as_dir$ac_word$ac_exec_ext" >&5
    break 2
  fi
done
  done
IFS=$as_save_IFS

fi
fi
RM=$ac_cv_prog_RM
if test -n "$RM"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $RM" >&5
printf "%s\n" "$RM" >&6; }
else
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: no" >&5
printf "%s\n" "no" >&6; }
fi



  # Find a good install program.  We prefer a C program (faster),
# so one script is as good as another.  But avoid the broken or
# incompatible versions:
# SysV /etc/install, /usr/sbin/install
# SunOS /usr/etc/install
# IRIX /sbin/install
# AIX /bin/install
# AmigaOS /C/install, which installs bootblocks on floppy discs
# AIX 4 /usr/bin/installbsd, which doesn't work without a -g flag
# AFS /usr/afsws/bin/install, which mishandles nonexistent args
# SVR4 /usr/ucb/install, which tries to use the nonexistent group "staff"
# OS/2's system install, which has a completely different semantic
# ./install, which can be erroneously created by make from ./install.sh.
# Reject install programs that cannot install multiple files.
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: checking for a BSD-compatible install" >&5
printf %s "checking for a BSD-compatible install... " >&6; }
if test -z "$INSTALL"; then
if test ${ac_cv_path_install+y}
then :
  printf %s "(cached) " >&6
else $as_nop
  as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    # Account for fact that we put trailing slashes in our PATH walk.
case $as_dir in #((
  ./ | /[cC]/* | \
  /etc/* | /usr/sbin/* | /usr/etc/* | /sbin/* | /usr/afsws/bin/* | \
  ?:[\\/]os2[\\/]install[\\/]* | ?:[\\/]OS2[\\/]INSTALL[\\/]* | \
  /usr/ucb/* ) ;;
  *)
    # OSF1 and SCO ODT 3.0 have their own names for install.
    # Don't use installbsd from OSF since it installs stuff as root
    # by default.
    for ac_prog in ginstall scoinst install; do
      for ac_exec_ext in '' $ac_executable_extensions; do
	if as_fn_executable_p "$as_dir$ac_prog$ac_exec_ext"; then
	  if test $ac_prog = install &&
	    grep dspmsg "$as_dir$ac_prog$ac_exec_ext" >/dev/null 2>&1; then
	    # AIX install.  It has an incompatible calling convention.
	    :
	  elif test $ac_prog = install &&
	    grep pwplus "$as_dir$ac_prog$ac_exec_ext" >/dev/null 2>&1; then
	    # program-specific install script used by HP pwplus--don't use.
	    :
	  else
	    rm -rf conftest.one conftest.two conftest.dir
	    echo one > conftest.one
	    echo two > conftest.two
	    mkdir conftest.dir
	    if "$as_dir$ac_prog$ac_exec_ext" -c conftest.one conftest.two "`pwd`/conftest.dir/" &&
	      test -s conftest.one && test -s conftest.two &&
	      test -s conftest.dir/conftest.one &&
	      test -s conftest.dir/conftest.two
	    then
	      ac_cv_path_install="$as_dir$ac_prog$ac_exec_ext -c"
	      break 3
	    fi
	  fi
	fi
      done
    done
    ;;
esac

  done
IFS=$as_save_IFS

rm -rf conftest.one conftest.two conftest.dir

fi
  if test ${ac_cv_path_install+y}; then
    INSTALL=$ac_cv_path_install
  else
    # As a last resort, use the slow shell script.  Don't cache a
    # value for INSTALL within a source directory, because that will
    # break other packages using the cache if that directory is
    # removed, or if the value is a relative name.
    INSTALL=$ac_install_sh
  fi
fi
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: result: $INSTALL" >&5
printf "%s\n" "$INSTALL" >&6; }

# Use test -z because SunOS4 sh mishandles braces in ${var-val}.
# It thinks the first close brace ends the variable substitution.
test -z "$INSTALL_PROGRAM" && INSTALL_PROGRAM='${INSTALL}'

test -z "$INSTALL_SCRIPT" && INSTALL_SCRIPT='${INSTALL}'

test -z "$INSTALL_DATA" && INSTALL_DATA='${INSTALL} -m 644'


if test -z "$kpathsea_include" -a -z "$kpathsea_lib"; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING:

    hbf2gf will be compiled without file search library support!
    For kpathsea support use the --with-kpathsea-lib and
    --with-kpathsea-include options.
              " >&5
printf "%s\n" "$as_me: WARNING:

    hbf2gf will be compiled without file search library support!
    For kpathsea support use the --with-kpathsea-lib and
    --with-kpathsea-include options.
              " >&2;}
fi

ac_config_files="$ac_config_files Makefile"

cat >confcache <<\_ACEOF
# This file is a shell script that caches the results of configure
# tests run on this system so they can be shared between configure
# scripts and configure runs, see configure's option --config-cache.
# It is not useful on other systems.  If it contains results you don't
# want to keep, you may remove or edit it.
#
# config.status only pays attention to the cache file if you give it
# the --recheck option to rerun configure.
#
# `ac_cv_env_foo' variables (set or unset) will be overridden when
# loading this file, other *unset* `ac_cv_foo' will be assigned the
# following values.

_ACEOF

# The following way of writing the cache mishandles newlines in values,
# but we know of no workaround that is simple, portable, and efficient.
# So, we kill variables containing newlines.
# Ultrix sh set writes to stderr and can't be redirected directly,
# and sets the high bit in the cache file unless we assign to the vars.
(
  for ac_var in `(set) 2>&1 | sed -n 's/^\([a-zA-Z_][a-zA-Z0-9_]*\)=.*/\1/p'`; do
    eval ac_val=\$$ac_var
    case $ac_val in #(
    *${as_nl}*)
      case $ac_var in #(
      *_cv_*) { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: cache variable $ac_var contains a newline" >&5
printf "%s\n" "$as_me: WARNING: cache variable $ac_var contains a newline" >&2;} ;;
      esac
      case $ac_var in #(
      _ | IFS | as_nl) ;; #(
      BASH_ARGV | BASH_SOURCE) eval $ac_var= ;; #(
      *) { eval $ac_var=; unset $ac_var;} ;;
      esac ;;
    esac
  done

  (set) 2>&1 |
    case $as_nl`(ac_space=' '; set) 2>&1` in #(
    *${as_nl}ac_space=\ *)
      # `set' does not quote correctly, so add quotes: double-quote
      # substitution turns \\\\ into \\, and sed turns \\ into \.
      sed -n \
	"s/'/'\\\\''/g;
	  s/^\\([_$as_cr_alnum]*_cv_[_$as_cr_alnum]*\\)=\\(.*\\)/\\1='\\2'/p"
      ;; #(
    *)
      # `set' quotes correctly as required by POSIX, so do not add quotes.
      sed -n "/^[_$as_cr_alnum]*_cv_[_$as_cr_alnum]*=/p"
      ;;
    esac |
    sort
) |
  sed '
     /^ac_cv_env_/b end
     t clear
     :clear
     s/^\([^=]*\)=\(.*[{}].*\)$/test ${\1+y} || &/
     t end
     s/^\([^=]*\)=\(.*\)$/\1=${\1=\2}/
     :end' >>confcache
if diff "$cache_file" confcache >/dev/null 2>&1; then :; else
  if test -w "$cache_file"; then
    if test "x$cache_file" != "x/dev/null"; then
      { printf "%s\n" "$as_me:${as_lineno-$LINENO}: updating cache $cache_file" >&5
printf "%s\n" "$as_me: updating cache $cache_file" >&6;}
      if test ! -f "$cache_file" || test -h "$cache_file"; then
	cat confcache >"$cache_file"
      else
        case $cache_file in #(
        */* | ?:*)
	  mv -f confcache "$cache_file"$$ &&
	  mv -f "$cache_file"$$ "$cache_file" ;; #(
        *)
	  mv -f confcache "$cache_file" ;;
	esac
      fi
    fi
  else
    { printf "%s\n" "$as_me:${as_lineno-$LINENO}: not updating unwritable cache $cache_file" >&5
printf "%s\n" "$as_me: not updating unwritable cache $cache_file" >&6;}
  fi
fi
rm -f confcache

test "x$prefix" = xNONE && prefix=$ac_default_prefix
# Let make expand exec_prefix.
test "x$exec_prefix" = xNONE && exec_prefix='${prefix}'

# Transform confdefs.h into DEFS.
# Protect against shell expansion while executing Makefile rules.
# Protect against Makefile macro expansion.
#
# If the first sed substitution is executed (which looks for macros that
# take arguments), then branch to the quote section.  Otherwise,
# look for a macro that doesn't take arguments.
ac_script='
:mline
/\\$/{
 N
 s,\\\n,,
 b mline
}
t clear
:clear
s/^[	 ]*#[	 ]*define[	 ][	 ]*\([^	 (][^	 (]*([^)]*)\)[	 ]*\(.*\)/-D\1=\2/g
t quote
s/^[	 ]*#[	 ]*define[	 ][	 ]*\([^	 ][^	 ]*\)[	 ]*\(.*\)/-D\1=\2/g
t quote
b any
:quote
s/[	 `~#$^&*(){}\\|;'\''"<>?]/\\&/g
s/\[/\\&/g
s/\]/\\&/g
s/\$/$$/g
H
:any
${
	g
	s/^\n//
	s/\n/ /g
	p
}
'
DEFS=`sed -n "$ac_script" confdefs.h`


ac_libobjs=
ac_ltlibobjs=
U=
for ac_i in : $LIBOBJS; do test "x$ac_i" = x: && continue
  # 1. Remove the extension, and $U if already installed.
  ac_script='s/\$U\././;s/\.o$//;s/\.obj$//'
  ac_i=`printf "%s\n" "$ac_i" | sed "$ac_script"`
  # 2. Prepend LIBOBJDIR.  When used with automake>=1.10 LIBOBJDIR
  #    will be set to the directory where LIBOBJS objects are built.
  as_fn_append ac_libobjs " \${LIBOBJDIR}$ac_i\$U.$ac_objext"
  as_fn_append ac_ltlibobjs " \${LIBOBJDIR}$ac_i"'$U.lo'
done
LIBOBJS=$ac_libobjs

LTLIBOBJS=$ac_ltlibobjs



: "${CONFIG_STATUS=./config.status}"
ac_write_fail=0
ac_clean_files_save=$ac_clean_files
ac_clean_files="$ac_clean_files $CONFIG_STATUS"
{ printf "%s\n" "$as_me:${as_lineno-$LINENO}: creating $CONFIG_STATUS" >&5
printf "%s\n" "$as_me: creating $CONFIG_STATUS" >&6;}
as_write_fail=0
cat >$CONFIG_STATUS <<_ASEOF || as_write_fail=1
#! $SHELL
# Generated by $as_me.
# Run this file to recreate the current configuration.
# Compiler output produced by configure, useful for debugging
# configure, is in config.log if it exists.

debug=false
ac_cs_recheck=false
ac_cs_silent=false

SHELL=\${CONFIG_SHELL-$SHELL}
export SHELL
_ASEOF
cat >>$CONFIG_STATUS <<\_ASEOF || as_write_fail=1
## -------------------- ##
## M4sh Initialization. ##
## -------------------- ##

# Be more Bourne compatible
DUALCASE=1; export DUALCASE # for MKS sh
as_nop=:
if test ${ZSH_VERSION+y} && (emulate sh) >/dev/null 2>&1
then :
  emulate sh
  NULLCMD=:
  # Pre-4.2 versions of Zsh do word splitting on ${1+"$@"}, which
  # is contrary to our usage.  Disable this feature.
  alias -g '${1+"$@"}'='"$@"'
  setopt NO_GLOB_SUBST
else $as_nop
  case `(set -o) 2>/dev/null` in #(
  *posix*) :
    set -o posix ;; #(
  *) :
     ;;
esac
fi



# Reset variables that may have inherited troublesome values from
# the environment.

# IFS needs to be set, to space, tab, and newline, in precisely that order.
# (If _AS_PATH_WALK were called with IFS unset, it would have the
# side effect of setting IFS to empty, thus disabling word splitting.)
# Quoting is to prevent editors from complaining about space-tab.
as_nl='
'
export as_nl
IFS=" ""	$as_nl"

PS1='$ '
PS2='> '
PS4='+ '

# Ensure predictable behavior from utilities with locale-dependent output.
LC_ALL=C
export LC_ALL
LANGUAGE=C
export LANGUAGE

# We cannot yet rely on "unset" to work, but we need these variables
# to be unset--not just set to an empty or harmless value--now, to
# avoid bugs in old shells (e.g. pre-3.0 UWIN ksh).  This construct
# also avoids known problems related to "unset" and subshell syntax
# in other old shells (e.g. bash 2.01 and pdksh 5.2.14).
for as_var in BASH_ENV ENV MAIL MAILPATH CDPATH
do eval test \${$as_var+y} \
  && ( (unset $as_var) || exit 1) >/dev/null 2>&1 && unset $as_var || :
done

# Ensure that fds 0, 1, and 2 are open.
if (exec 3>&0) 2>/dev/null; then :; else exec 0</dev/null; fi
if (exec 3>&1) 2>/dev/null; then :; else exec 1>/dev/null; fi
if (exec 3>&2)            ; then :; else exec 2>/dev/null; fi

# The user is always right.
if ${PATH_SEPARATOR+false} :; then
  PATH_SEPARATOR=:
  (PATH='/bin;/bin'; FPATH=$PATH; sh -c :) >/dev/null 2>&1 && {
    (PATH='/bin:/bin'; FPATH=$PATH; sh -c :) >/dev/null 2>&1 ||
      PATH_SEPARATOR=';'
  }
fi


# Find who we are.  Look in the path if we contain no directory separator.
as_myself=
case $0 in #((
  *[\\/]* ) as_myself=$0 ;;
  *) as_save_IFS=$IFS; IFS=$PATH_SEPARATOR
for as_dir in $PATH
do
  IFS=$as_save_IFS
  case $as_dir in #(((
    '') as_dir=./ ;;
    */) ;;
    *) as_dir=$as_dir/ ;;
  esac
    test -r "$as_dir$0" && as_myself=$as_dir$0 && break
  done
IFS=$as_save_IFS

     ;;
esac
# We did not find ourselves, most probably we were run as `sh COMMAND'
# in which case we are not to be found in the path.
if test "x$as_myself" = x; then
  as_myself=$0
fi
if test ! -f "$as_myself"; then
  printf "%s\n" "$as_myself: error: cannot find myself; rerun with an absolute file name" >&2
  exit 1
fi



# as_fn_error STATUS ERROR [LINENO LOG_FD]
# ----------------------------------------
# Output "`basename $0`: error: ERROR" to stderr. If LINENO and LOG_FD are
# provided, also output the error to LOG_FD, referencing LINENO. Then exit the
# script with STATUS, using 1 if that was 0.
as_fn_error ()
{
  as_status=$1; test $as_status -eq 0 && as_status=1
  if test "$4"; then
    as_lineno=${as_lineno-"$3"} as_lineno_stack=as_lineno_stack=$as_lineno_stack
    printf "%s\n" "$as_me:${as_lineno-$LINENO}: error: $2" >&$4
  fi
  printf "%s\n" "$as_me: error: $2" >&2
  as_fn_exit $as_status
} # as_fn_error



# as_fn_set_status STATUS
# -----------------------
# Set $? to STATUS, without forking.
as_fn_set_status ()
{
  return $1
} # as_fn_set_status

# as_fn_exit STATUS
# -----------------
# Exit the shell with STATUS, even in a "trap 0" or "set -e" context.
as_fn_exit ()
{
  set +e
  as_fn_set_status $1
  exit $1
} # as_fn_exit

# as_fn_unset VAR
# ---------------
# Portably unset VAR.
as_fn_unset ()
{
  { eval $1=; unset $1;}
}
as_unset=as_fn_unset

# as_fn_append VAR VALUE
# ----------------------
# Append the text in VALUE to the end of the definition contained in VAR. Take
# advantage of any shell optimizations that allow amortized linear growth over
# repeated appends, instead of the typical quadratic growth present in naive
# implementations.
if (eval "as_var=1; as_var+=2; test x\$as_var = x12") 2>/dev/null
then :
  eval 'as_fn_append ()
  {
    eval $1+=\$2
  }'
else $as_nop
  as_fn_append ()
  {
    eval $1=\$$1\$2
  }
fi # as_fn_append

# as_fn_arith ARG...
# ------------------
# Perform arithmetic evaluation on the ARGs, and store the result in the
# global $as_val. Take advantage of shells that can avoid forks. The arguments
# must be portable across $(()) and expr.
if (eval "test \$(( 1 + 1 )) = 2") 2>/dev/null
then :
  eval 'as_fn_arith ()
  {
    as_val=$(( $* ))
  }'
else $as_nop
  as_fn_arith ()
  {
    as_val=`expr "$@" || test $? -eq 1`
  }
fi # as_fn_arith


if expr a : '\(a\)' >/dev/null 2>&1 &&
   test "X`expr 00001 : '.*\(...\)'`" = X001; then
  as_expr=expr
else
  as_expr=false
fi

if (basename -- /) >/dev/null 2>&1 && test "X`basename -- / 2>&1`" = "X/"; then
  as_basename=basename
else
  as_basename=false
fi

if (as_dir=`dirname -- /` && test "X$as_dir" = X/) >/dev/null 2>&1; then
  as_dirname=dirname
else
  as_dirname=false
fi

as_me=`$as_basename -- "$0" ||
$as_expr X/"$0" : '.*/\([^/][^/]*\)/*$' \| \
	 X"$0" : 'X\(//\)$' \| \
	 X"$0" : 'X\(/\)' \| . 2>/dev/null ||
printf "%s\n" X/"$0" |
    sed '/^.*\/\([^/][^/]*\)\/*$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\/\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`

# Avoid depending upon Character Ranges.
as_cr_letters='abcdefghijklmnopqrstuvwxyz'
as_cr_LETTERS='ABCDEFGHIJKLMNOPQRSTUVWXYZ'
as_cr_Letters=$as_cr_letters$as_cr_LETTERS
as_cr_digits='0123456789'
as_cr_alnum=$as_cr_Letters$as_cr_digits


# Determine whether it's possible to make 'echo' print without a newline.
# These variables are no longer used directly by Autoconf, but are AC_SUBSTed
# for compatibility with existing Makefiles.
ECHO_C= ECHO_N= ECHO_T=
case `echo -n x` in #(((((
-n*)
  case `echo 'xy\c'` in
  *c*) ECHO_T='	';;	# ECHO_T is single tab character.
  xy)  ECHO_C='\c';;
  *)   echo `echo ksh88 bug on AIX 6.1` > /dev/null
       ECHO_T='	';;
  esac;;
*)
  ECHO_N='-n';;
esac

# For backward compatibility with old third-party macros, we provide
# the shell variables $as_echo and $as_echo_n.  New code should use
# AS_ECHO(["message"]) and AS_ECHO_N(["message"]), respectively.
as_echo='printf %s\n'
as_echo_n='printf %s'

rm -f conf$$ conf$$.exe conf$$.file
if test -d conf$$.dir; then
  rm -f conf$$.dir/conf$$.file
else
  rm -f conf$$.dir
  mkdir conf$$.dir 2>/dev/null
fi
if (echo >conf$$.file) 2>/dev/null; then
  if ln -s conf$$.file conf$$ 2>/dev/null; then
    as_ln_s='ln -s'
    # ... but there are two gotchas:
    # 1) On MSYS, both `ln -s file dir' and `ln file dir' fail.
    # 2) DJGPP < 2.04 has no symlinks; `ln -s' creates a wrapper executable.
    # In both cases, we have to default to `cp -pR'.
    ln -s conf$$.file conf$$.dir 2>/dev/null && test ! -f conf$$.exe ||
      as_ln_s='cp -pR'
  elif ln conf$$.file conf$$ 2>/dev/null; then
    as_ln_s=ln
  else
    as_ln_s='cp -pR'
  fi
else
  as_ln_s='cp -pR'
fi
rm -f conf$$ conf$$.exe conf$$.dir/conf$$.file conf$$.file
rmdir conf$$.dir 2>/dev/null


# as_fn_mkdir_p
# -------------
# Create "$as_dir" as a directory, including parents if necessary.
as_fn_mkdir_p ()
{

  case $as_dir in #(
  -*) as_dir=./$as_dir;;
  esac
  test -d "$as_dir" || eval $as_mkdir_p || {
    as_dirs=
    while :; do
      case $as_dir in #(
      *\'*) as_qdir=`printf "%s\n" "$as_dir" | sed "s/'/'\\\\\\\\''/g"`;; #'(
      *) as_qdir=$as_dir;;
      esac
      as_dirs="'$as_qdir' $as_dirs"
      as_dir=`$as_dirname -- "$as_dir" ||
$as_expr X"$as_dir" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$as_dir" : 'X\(//\)[^/]' \| \
	 X"$as_dir" : 'X\(//\)$' \| \
	 X"$as_dir" : 'X\(/\)' \| . 2>/dev/null ||
printf "%s\n" X"$as_dir" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
      test -d "$as_dir" && break
    done
    test -z "$as_dirs" || eval "mkdir $as_dirs"
  } || test -d "$as_dir" || as_fn_error $? "cannot create directory $as_dir"


} # as_fn_mkdir_p
if mkdir -p . 2>/dev/null; then
  as_mkdir_p='mkdir -p "$as_dir"'
else
  test -d ./-p && rmdir ./-p
  as_mkdir_p=false
fi


# as_fn_executable_p FILE
# -----------------------
# Test if FILE is an executable regular file.
as_fn_executable_p ()
{
  test -f "$1" && test -x "$1"
} # as_fn_executable_p
as_test_x='test -x'
as_executable_p=as_fn_executable_p

# Sed expression to map a string onto a valid CPP name.
as_tr_cpp="eval sed 'y%*$as_cr_letters%P$as_cr_LETTERS%;s%[^_$as_cr_alnum]%_%g'"

# Sed expression to map a string onto a valid variable name.
as_tr_sh="eval sed 'y%*+%pp%;s%[^_$as_cr_alnum]%_%g'"


exec 6>&1
## ----------------------------------- ##
## Main body of $CONFIG_STATUS script. ##
## ----------------------------------- ##
_ASEOF
test $as_write_fail = 0 && chmod +x $CONFIG_STATUS || ac_write_fail=1

cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1
# Save the log message, to keep $0 and so on meaningful, and to
# report actual input values of CONFIG_FILES etc. instead of their
# values after options handling.
ac_log="
This file was extended by $as_me, which was
generated by GNU Autoconf 2.71.  Invocation command line was

  CONFIG_FILES    = $CONFIG_FILES
  CONFIG_HEADERS  = $CONFIG_HEADERS
  CONFIG_LINKS    = $CONFIG_LINKS
  CONFIG_COMMANDS = $CONFIG_COMMANDS
  $ $0 $@

on `(hostname || uname -n) 2>/dev/null | sed 1q`
"

_ACEOF

case $ac_config_files in *"
"*) set x $ac_config_files; shift; ac_config_files=$*;;
esac



cat >>$CONFIG_STATUS <<_ACEOF || ac_write_fail=1
# Files that config.status was made for.
config_files="$ac_config_files"

_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1
ac_cs_usage="\
\`$as_me' instantiates files and other configuration actions
from templates according to the current configuration.  Unless the files
and actions are specified as TAGs, all are instantiated by default.

Usage: $0 [OPTION]... [TAG]...

  -h, --help       print this help, then exit
  -V, --version    print version number and configuration settings, then exit
      --config     print configuration, then exit
  -q, --quiet, --silent
                   do not print progress messages
  -d, --debug      don't remove temporary files
      --recheck    update $as_me by reconfiguring in the same conditions
      --file=FILE[:TEMPLATE]
                   instantiate the configuration file FILE

Configuration files:
$config_files

Report bugs to the package provider."

_ACEOF
ac_cs_config=`printf "%s\n" "$ac_configure_args" | sed "$ac_safe_unquote"`
ac_cs_config_escaped=`printf "%s\n" "$ac_cs_config" | sed "s/^ //; s/'/'\\\\\\\\''/g"`
cat >>$CONFIG_STATUS <<_ACEOF || ac_write_fail=1
ac_cs_config='$ac_cs_config_escaped'
ac_cs_version="\\
config.status
configured by $0, generated by GNU Autoconf 2.71,
  with options \\"\$ac_cs_config\\"

Copyright (C) 2021 Free Software Foundation, Inc.
This config.status script is free software; the Free Software Foundation
gives unlimited permission to copy, distribute and modify it."

ac_pwd='$ac_pwd'
srcdir='$srcdir'
INSTALL='$INSTALL'
test -n "\$AWK" || AWK=awk
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1
# The default lists apply if the user does not specify any file.
ac_need_defaults=:
while test $# != 0
do
  case $1 in
  --*=?*)
    ac_option=`expr "X$1" : 'X\([^=]*\)='`
    ac_optarg=`expr "X$1" : 'X[^=]*=\(.*\)'`
    ac_shift=:
    ;;
  --*=)
    ac_option=`expr "X$1" : 'X\([^=]*\)='`
    ac_optarg=
    ac_shift=:
    ;;
  *)
    ac_option=$1
    ac_optarg=$2
    ac_shift=shift
    ;;
  esac

  case $ac_option in
  # Handling of the options.
  -recheck | --recheck | --rechec | --reche | --rech | --rec | --re | --r)
    ac_cs_recheck=: ;;
  --version | --versio | --versi | --vers | --ver | --ve | --v | -V )
    printf "%s\n" "$ac_cs_version"; exit ;;
  --config | --confi | --conf | --con | --co | --c )
    printf "%s\n" "$ac_cs_config"; exit ;;
  --debug | --debu | --deb | --de | --d | -d )
    debug=: ;;
  --file | --fil | --fi | --f )
    $ac_shift
    case $ac_optarg in
    *\'*) ac_optarg=`printf "%s\n" "$ac_optarg" | sed "s/'/'\\\\\\\\''/g"` ;;
    '') as_fn_error $? "missing file argument" ;;
    esac
    as_fn_append CONFIG_FILES " '$ac_optarg'"
    ac_need_defaults=false;;
  --he | --h |  --help | --hel | -h )
    printf "%s\n" "$ac_cs_usage"; exit ;;
  -q | -quiet | --quiet | --quie | --qui | --qu | --q \
  | -silent | --silent | --silen | --sile | --sil | --si | --s)
    ac_cs_silent=: ;;

  # This is an error.
  -*) as_fn_error $? "unrecognized option: \`$1'
Try \`$0 --help' for more information." ;;

  *) as_fn_append ac_config_targets " $1"
     ac_need_defaults=false ;;

  esac
  shift
done

ac_configure_extra_args=

if $ac_cs_silent; then
  exec 6>/dev/null
  ac_configure_extra_args="$ac_configure_extra_args --silent"
fi

_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF || ac_write_fail=1
if \$ac_cs_recheck; then
  set X $SHELL '$0' $ac_configure_args \$ac_configure_extra_args --no-create --no-recursion
  shift
  \printf "%s\n" "running CONFIG_SHELL=$SHELL \$*" >&6
  CONFIG_SHELL='$SHELL'
  export CONFIG_SHELL
  exec "\$@"
fi

_ACEOF
cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1
exec 5>>config.log
{
  echo
  sed 'h;s/./-/g;s/^.../## /;s/...$/ ##/;p;x;p;x' <<_ASBOX
## Running $as_me. ##
_ASBOX
  printf "%s\n" "$ac_log"
} >&5

_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF || ac_write_fail=1
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1

# Handling of arguments.
for ac_config_target in $ac_config_targets
do
  case $ac_config_target in
    "Makefile") CONFIG_FILES="$CONFIG_FILES Makefile" ;;

  *) as_fn_error $? "invalid argument: \`$ac_config_target'" "$LINENO" 5;;
  esac
done


# If the user did not use the arguments to specify the items to instantiate,
# then the envvar interface is used.  Set only those that are not.
# We use the long form for the default assignment because of an extremely
# bizarre bug on SunOS 4.1.3.
if $ac_need_defaults; then
  test ${CONFIG_FILES+y} || CONFIG_FILES=$config_files
fi

# Have a temporary directory for convenience.  Make it in the build tree
# simply because there is no reason against having it here, and in addition,
# creating and moving files from /tmp can sometimes cause problems.
# Hook for its removal unless debugging.
# Note that there is a small window in which the directory will not be cleaned:
# after its creation but before its name has been assigned to `$tmp'.
$debug ||
{
  tmp= ac_tmp=
  trap 'exit_status=$?
  : "${ac_tmp:=$tmp}"
  { test ! -d "$ac_tmp" || rm -fr "$ac_tmp"; } && exit $exit_status
' 0
  trap 'as_fn_exit 1' 1 2 13 15
}
# Create a (secure) tmp directory for tmp files.

{
  tmp=`(umask 077 && mktemp -d "./confXXXXXX") 2>/dev/null` &&
  test -d "$tmp"
}  ||
{
  tmp=./conf$$-$RANDOM
  (umask 077 && mkdir "$tmp")
} || as_fn_error $? "cannot create a temporary directory in ." "$LINENO" 5
ac_tmp=$tmp

# Set up the scripts for CONFIG_FILES section.
# No need to generate them if there are no CONFIG_FILES.
# This happens for instance with `./config.status config.h'.
if test -n "$CONFIG_FILES"; then


ac_cr=`echo X | tr X '\015'`
# On cygwin, bash can eat \r inside `` if the user requested igncr.
# But we know of no other shell where ac_cr would be empty at this
# point, so we can use a bashism as a fallback.
if test "x$ac_cr" = x; then
  eval ac_cr=\$\'\\r\'
fi
ac_cs_awk_cr=`$AWK 'BEGIN { print "a\rb" }' </dev/null 2>/dev/null`
if test "$ac_cs_awk_cr" = "a${ac_cr}b"; then
  ac_cs_awk_cr='\\r'
else
  ac_cs_awk_cr=$ac_cr
fi

echo 'BEGIN {' >"$ac_tmp/subs1.awk" &&
_ACEOF


{
  echo "cat >conf$$subs.awk <<_ACEOF" &&
  echo "$ac_subst_vars" | sed 's/.*/&!$&$ac_delim/' &&
  echo "_ACEOF"
} >conf$$subs.sh ||
  as_fn_error $? "could not make $CONFIG_STATUS" "$LINENO" 5
ac_delim_num=`echo "$ac_subst_vars" | grep -c '^'`
ac_delim='%!_!# '
for ac_last_try in false false false false false :; do
  . ./conf$$subs.sh ||
    as_fn_error $? "could not make $CONFIG_STATUS" "$LINENO" 5

  ac_delim_n=`sed -n "s/.*$ac_delim\$/X/p" conf$$subs.awk | grep -c X`
  if test $ac_delim_n = $ac_delim_num; then
    break
  elif $ac_last_try; then
    as_fn_error $? "could not make $CONFIG_STATUS" "$LINENO" 5
  else
    ac_delim="$ac_delim!$ac_delim _$ac_delim!! "
  fi
done
rm -f conf$$subs.sh

cat >>$CONFIG_STATUS <<_ACEOF || ac_write_fail=1
cat >>"\$ac_tmp/subs1.awk" <<\\_ACAWK &&
_ACEOF
sed -n '
h
s/^/S["/; s/!.*/"]=/
p
g
s/^[^!]*!//
:repl
t repl
s/'"$ac_delim"'$//
t delim
:nl
h
s/\(.\{148\}\)..*/\1/
t more1
s/["\\]/\\&/g; s/^/"/; s/$/\\n"\\/
p
n
b repl
:more1
s/["\\]/\\&/g; s/^/"/; s/$/"\\/
p
g
s/.\{148\}//
t nl
:delim
h
s/\(.\{148\}\)..*/\1/
t more2
s/["\\]/\\&/g; s/^/"/; s/$/"/
p
b
:more2
s/["\\]/\\&/g; s/^/"/; s/$/"\\/
p
g
s/.\{148\}//
t delim
' <conf$$subs.awk | sed '
/^[^""]/{
  N
  s/\n//
}
' >>$CONFIG_STATUS || ac_write_fail=1
rm -f conf$$subs.awk
cat >>$CONFIG_STATUS <<_ACEOF || ac_write_fail=1
_ACAWK
cat >>"\$ac_tmp/subs1.awk" <<_ACAWK &&
  for (key in S) S_is_set[key] = 1
  FS = ""

}
{
  line = $ 0
  nfields = split(line, field, "@")
  substed = 0
  len = length(field[1])
  for (i = 2; i < nfields; i++) {
    key = field[i]
    keylen = length(key)
    if (S_is_set[key]) {
      value = S[key]
      line = substr(line, 1, len) "" value "" substr(line, len + keylen + 3)
      len += length(value) + length(field[++i])
      substed = 1
    } else
      len += 1 + keylen
  }

  print line
}

_ACAWK
_ACEOF
cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1
if sed "s/$ac_cr//" < /dev/null > /dev/null 2>&1; then
  sed "s/$ac_cr\$//; s/$ac_cr/$ac_cs_awk_cr/g"
else
  cat
fi < "$ac_tmp/subs1.awk" > "$ac_tmp/subs.awk" \
  || as_fn_error $? "could not setup config files machinery" "$LINENO" 5
_ACEOF

# VPATH may cause trouble with some makes, so we remove sole $(srcdir),
# ${srcdir} and @srcdir@ entries from VPATH if srcdir is ".", strip leading and
# trailing colons and then remove the whole line if VPATH becomes empty
# (actually we leave an empty line to preserve line numbers).
if test "x$srcdir" = x.; then
  ac_vpsub='/^[	 ]*VPATH[	 ]*=[	 ]*/{
h
s///
s/^/:/
s/[	 ]*$/:/
s/:\$(srcdir):/:/g
s/:\${srcdir}:/:/g
s/:@srcdir@:/:/g
s/^:*//
s/:*$//
x
s/\(=[	 ]*\).*/\1/
G
s/\n//
s/^[^=]*=[	 ]*$//
}'
fi

cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1
fi # test -n "$CONFIG_FILES"


eval set X "  :F $CONFIG_FILES      "
shift
for ac_tag
do
  case $ac_tag in
  :[FHLC]) ac_mode=$ac_tag; continue;;
  esac
  case $ac_mode$ac_tag in
  :[FHL]*:*);;
  :L* | :C*:*) as_fn_error $? "invalid tag \`$ac_tag'" "$LINENO" 5;;
  :[FH]-) ac_tag=-:-;;
  :[FH]*) ac_tag=$ac_tag:$ac_tag.in;;
  esac
  ac_save_IFS=$IFS
  IFS=:
  set x $ac_tag
  IFS=$ac_save_IFS
  shift
  ac_file=$1
  shift

  case $ac_mode in
  :L) ac_source=$1;;
  :[FH])
    ac_file_inputs=
    for ac_f
    do
      case $ac_f in
      -) ac_f="$ac_tmp/stdin";;
      *) # Look for the file first in the build tree, then in the source tree
	 # (if the path is not absolute).  The absolute path cannot be DOS-style,
	 # because $ac_f cannot contain `:'.
	 test -f "$ac_f" ||
	   case $ac_f in
	   [\\/$]*) false;;
	   *) test -f "$srcdir/$ac_f" && ac_f="$srcdir/$ac_f";;
	   esac ||
	   as_fn_error 1 "cannot find input file: \`$ac_f'" "$LINENO" 5;;
      esac
      case $ac_f in *\'*) ac_f=`printf "%s\n" "$ac_f" | sed "s/'/'\\\\\\\\''/g"`;; esac
      as_fn_append ac_file_inputs " '$ac_f'"
    done

    # Let's still pretend it is `configure' which instantiates (i.e., don't
    # use $as_me), people would be surprised to read:
    #    /* config.h.  Generated by config.status.  */
    configure_input='Generated from '`
	  printf "%s\n" "$*" | sed 's|^[^:]*/||;s|:[^:]*/|, |g'
	`' by configure.'
    if test x"$ac_file" != x-; then
      configure_input="$ac_file.  $configure_input"
      { printf "%s\n" "$as_me:${as_lineno-$LINENO}: creating $ac_file" >&5
printf "%s\n" "$as_me: creating $ac_file" >&6;}
    fi
    # Neutralize special characters interpreted by sed in replacement strings.
    case $configure_input in #(
    *\&* | *\|* | *\\* )
       ac_sed_conf_input=`printf "%s\n" "$configure_input" |
       sed 's/[\\\\&|]/\\\\&/g'`;; #(
    *) ac_sed_conf_input=$configure_input;;
    esac

    case $ac_tag in
    *:-:* | *:-) cat >"$ac_tmp/stdin" \
      || as_fn_error $? "could not create $ac_file" "$LINENO" 5 ;;
    esac
    ;;
  esac

  ac_dir=`$as_dirname -- "$ac_file" ||
$as_expr X"$ac_file" : 'X\(.*[^/]\)//*[^/][^/]*/*$' \| \
	 X"$ac_file" : 'X\(//\)[^/]' \| \
	 X"$ac_file" : 'X\(//\)$' \| \
	 X"$ac_file" : 'X\(/\)' \| . 2>/dev/null ||
printf "%s\n" X"$ac_file" |
    sed '/^X\(.*[^/]\)\/\/*[^/][^/]*\/*$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)[^/].*/{
	    s//\1/
	    q
	  }
	  /^X\(\/\/\)$/{
	    s//\1/
	    q
	  }
	  /^X\(\/\).*/{
	    s//\1/
	    q
	  }
	  s/.*/./; q'`
  as_dir="$ac_dir"; as_fn_mkdir_p
  ac_builddir=.

case "$ac_dir" in
.) ac_dir_suffix= ac_top_builddir_sub=. ac_top_build_prefix= ;;
*)
  ac_dir_suffix=/`printf "%s\n" "$ac_dir" | sed 's|^\.[\\/]||'`
  # A ".." for each directory in $ac_dir_suffix.
  ac_top_builddir_sub=`printf "%s\n" "$ac_dir_suffix" | sed 's|/[^\\/]*|/..|g;s|/||'`
  case $ac_top_builddir_sub in
  "") ac_top_builddir_sub=. ac_top_build_prefix= ;;
  *)  ac_top_build_prefix=$ac_top_builddir_sub/ ;;
  esac ;;
esac
ac_abs_top_builddir=$ac_pwd
ac_abs_builddir=$ac_pwd$ac_dir_suffix
# for backward compatibility:
ac_top_builddir=$ac_top_build_prefix

case $srcdir in
  .)  # We are building in place.
    ac_srcdir=.
    ac_top_srcdir=$ac_top_builddir_sub
    ac_abs_top_srcdir=$ac_pwd ;;
  [\\/]* | ?:[\\/]* )  # Absolute name.
    ac_srcdir=$srcdir$ac_dir_suffix;
    ac_top_srcdir=$srcdir
    ac_abs_top_srcdir=$srcdir ;;
  *) # Relative name.
    ac_srcdir=$ac_top_build_prefix$srcdir$ac_dir_suffix
    ac_top_srcdir=$ac_top_build_prefix$srcdir
    ac_abs_top_srcdir=$ac_pwd/$srcdir ;;
esac
ac_abs_srcdir=$ac_abs_top_srcdir$ac_dir_suffix


  case $ac_mode in
  :F)
  #
  # CONFIG_FILE
  #

  case $INSTALL in
  [\\/$]* | ?:[\\/]* ) ac_INSTALL=$INSTALL ;;
  *) ac_INSTALL=$ac_top_build_prefix$INSTALL ;;
  esac
_ACEOF

cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1
# If the template does not know about datarootdir, expand it.
# FIXME: This hack should be removed a few years after 2.60.
ac_datarootdir_hack=; ac_datarootdir_seen=
ac_sed_dataroot='
/datarootdir/ {
  p
  q
}
/@datadir@/p
/@docdir@/p
/@infodir@/p
/@localedir@/p
/@mandir@/p'
case `eval "sed -n \"\$ac_sed_dataroot\" $ac_file_inputs"` in
*datarootdir*) ac_datarootdir_seen=yes;;
*@datadir@*|*@docdir@*|*@infodir@*|*@localedir@*|*@mandir@*)
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: $ac_file_inputs seems to ignore the --datarootdir setting" >&5
printf "%s\n" "$as_me: WARNING: $ac_file_inputs seems to ignore the --datarootdir setting" >&2;}
_ACEOF
cat >>$CONFIG_STATUS <<_ACEOF || ac_write_fail=1
  ac_datarootdir_hack='
  s&@datadir@&$datadir&g
  s&@docdir@&$docdir&g
  s&@infodir@&$infodir&g
  s&@localedir@&$localedir&g
  s&@mandir@&$mandir&g
  s&\\\${datarootdir}&$datarootdir&g' ;;
esac
_ACEOF

# Neutralize VPATH when `$srcdir' = `.'.
# Shell code in configure.ac might set extrasub.
# FIXME: do we really want to maintain this feature?
cat >>$CONFIG_STATUS <<_ACEOF || ac_write_fail=1
ac_sed_extra="$ac_vpsub
$extrasub
_ACEOF
cat >>$CONFIG_STATUS <<\_ACEOF || ac_write_fail=1
:t
/@[a-zA-Z_][a-zA-Z_0-9]*@/!b
s|@configure_input@|$ac_sed_conf_input|;t t
s&@top_builddir@&$ac_top_builddir_sub&;t t
s&@top_build_prefix@&$ac_top_build_prefix&;t t
s&@srcdir@&$ac_srcdir&;t t
s&@abs_srcdir@&$ac_abs_srcdir&;t t
s&@top_srcdir@&$ac_top_srcdir&;t t
s&@abs_top_srcdir@&$ac_abs_top_srcdir&;t t
s&@builddir@&$ac_builddir&;t t
s&@abs_builddir@&$ac_abs_builddir&;t t
s&@abs_top_builddir@&$ac_abs_top_builddir&;t t
s&@INSTALL@&$ac_INSTALL&;t t
$ac_datarootdir_hack
"
eval sed \"\$ac_sed_extra\" "$ac_file_inputs" | $AWK -f "$ac_tmp/subs.awk" \
  >$ac_tmp/out || as_fn_error $? "could not create $ac_file" "$LINENO" 5

test -z "$ac_datarootdir_hack$ac_datarootdir_seen" &&
  { ac_out=`sed -n '/\${datarootdir}/p' "$ac_tmp/out"`; test -n "$ac_out"; } &&
  { ac_out=`sed -n '/^[	 ]*datarootdir[	 ]*:*=/p' \
      "$ac_tmp/out"`; test -z "$ac_out"; } &&
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: $ac_file contains a reference to the variable \`datarootdir'
which seems to be undefined.  Please make sure it is defined" >&5
printf "%s\n" "$as_me: WARNING: $ac_file contains a reference to the variable \`datarootdir'
which seems to be undefined.  Please make sure it is defined" >&2;}

  rm -f "$ac_tmp/stdin"
  case $ac_file in
  -) cat "$ac_tmp/out" && rm -f "$ac_tmp/out";;
  *) rm -f "$ac_file" && mv "$ac_tmp/out" "$ac_file";;
  esac \
  || as_fn_error $? "could not create $ac_file" "$LINENO" 5
 ;;



  esac

done # for ac_tag


as_fn_exit 0
_ACEOF
ac_clean_files=$ac_clean_files_save

test $ac_write_fail = 0 ||
  as_fn_error $? "write failure creating $CONFIG_STATUS" "$LINENO" 5


# configure is writing to config.log, and then calls config.status.
# config.status does its own redirection, appending to config.log.
# Unfortunately, on DOS this fails, as config.log is still kept open
# by configure, so config.status won't be able to write to it; its
# output is simply discarded.  So we exec the FD to /dev/null,
# effectively closing config.log, so it can be properly (re)opened and
# appended to by config.status.  When coming back to configure, we
# need to make the FD available again.
if test "$no_create" != yes; then
  ac_cs_success=:
  ac_config_status_args=
  test "$silent" = yes &&
    ac_config_status_args="$ac_config_status_args --quiet"
  exec 5>/dev/null
  $SHELL $CONFIG_STATUS $ac_config_status_args || ac_cs_success=false
  exec 5>>config.log
  # Use ||, not &&, to avoid exiting from the if with $? = 1, which
  # would make configure fail if this is the last instruction.
  $ac_cs_success || as_fn_exit 1
fi
if test -n "$ac_unrecognized_opts" && test "$enable_option_checking" != no; then
  { printf "%s\n" "$as_me:${as_lineno-$LINENO}: WARNING: unrecognized options: $ac_unrecognized_opts" >&5
printf "%s\n" "$as_me: WARNING: unrecognized options: $ac_unrecognized_opts" >&2;}
fi




==> cjk-4.8.5/utils/hbf2gf/hbf2gf.1 <==
.\" man page for hbf2gf
.\"
.\" Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
.\"
.\" This program is free software; you can redistribute it and/or modify
.\" it under the terms of the GNU General Public License as published by
.\" the Free Software Foundation; either version 2 of the License, or
.\" (at your option) any later version.
.\"
.\" This program is distributed in the hope that it will be useful,
.\" but WITHOUT ANY WARRANTY; without even the implied warranty of
.\" MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
.\" GNU General Public License for more details.
.\"
.\" You should have received a copy of the GNU General Public License
.\" along with this program in doc/COPYING; if not, write to the Free
.\" Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
.\" MA 02110-1301 USA
.\"
.
.TH HBF2GF 1 16-Oct-2021 "CJK Version 4.8.5"
.SH NAME
hbf2gf \- convert a CJK bitmap font into subfonts usable by TeX and Omega.
.
.
.SH SYNOPSIS
.na
.nh
.B hbf2gf
.RB [ \-q ]
.IR \%configuration-file [ .cfg ]
.br
.B hbf2gf
'in +\n(.ku
.RB [ \-q ]
.RB [ \-p ]
.RB [ \-g ]
.RB [ \-n ]
.I \%subfont-name \%x-resolution
.RI [ \%y-scale \ | \ \%y-resolution ]
.br
.in
.B hbf2gf
.B \-t
.RB [ \-q ]
.I \%subfont-name
.br
.B "hbf2gf \-\-version"
|
.B \-\-help
.ad
.hy
.
.
.
.\" ====
.\" ==== macro definitions
.\" ====
.
.\" here we define \TeX for troff and nroff
.if t .ds TX \fRT\h'-0.1667m'\v'0.20v'E\v'-0.20v'\h'-0.125m'X\fP
.if n .ds TX TeX
.
.\" and here the same for \LaTeX
.if t \{\
.ie '\*(.T'dvi' \
.ds LX \fRL\h'-0.36m'\v'-0.15v'\s-3A\s0\h'-0.15m'\v'0.15v'\fP\*(TX
.el .ds LX \fRL\h'-0.36m'\v'-0.22v'\s-2A\s0\h'-0.15m'\v'0.22v'\fP\*(TX
.\}
.if n .ds LX LaTeX
.
.\" \LaTeXe
.\" note that we need \vareps for TeX instead of \eps which can only be
.\" accessed with the \N escape sequence (in the Math Italic font)
.if t \{\
.ie '\*(.T'dvi' .ds LE \*(LX\h'0.15m'2\v'0.20v'\f(MI\N'34'\fP\v'-0.20v'
.el .ds LE \*(LX\h'0.15m'2\v'0.20v'\(*e\v'-0.20v'
.\}
.if n .ds LE LaTeX\ 2e
.
.\" a definition for \Delta
.if t .ds DE \(*D
.if n .ds DE Delta_
.
.\" a typewriter font
.if t \{\
.de C
\fC\\$1\fP\\$2
..
.\}
.if n \{\
.de C
\\$1\\$2
..
.\}
.
.\" an addition to .TP to allow two labels for the same item
.de TQ
.br
.ns
.TP
..
.
.\" ====
.\" ==== end of macro definitions
.\" ====
.
.
.
.SH DESCRIPTION
CJK bitmap fonts can't be directly used with \*(TX
because the number of characters in such fonts exceeds\ 256, the limit of a
\*(TX
font.
Thus it is necessary to split these fonts into subfonts, and this is
exactly what
.B hbf2gf
does.
.PP
As the name says,
.B hbf2gf
uses CJK fonts in a certain format which is called
.B Hanzi Bitmap Font
.RB ( HBF )
format.
It simply consists of the CJK bitmap file(s) and a text file in a format
very similar to the BDF format of the X\ Window System which describes the
bitmap font files: the encoding, the size, etc.
The produced
.C GF
files can then be converted with
.B gftopk
into standard
.C PK
files.
.PP
.B hbf2gf
can be called in three modes:
.
.PP
.in +2m
.B hbf2gf
.RB [ \-q ]
.IR configuration-file [ .cfg ]
.PP
.in +5m
This call normally creates a set of
.C GF
files, one
.C PL
file, and a batch file which must be executed after
.B hbf2gf
has finished.
This script will then call
.B gftopk
to convert all
.C GF
files into
.C PK
files, and it will call
.B pltotf
to convert the
.C PL
file into a
.C TFM
file.
Finally it will copy the
.C TFM
file so that each
.C PK
file has its
.C TFM
file (which are all identical).
.PP
.in +5m
If
.B ofm_file
is set to \(oqyes\(cq in the configuration file,
.C OFM
and
.C OVF
files will be created too.
.
.PP
.in +5m
.B \-q
makes
.B hbf2gf
quiet.
.PP
.in +2m
.na
.nh
.B hbf2gf
'in +\n(.ku
.RB [ \-q ]
.RB [ \-p ]
.RB [ \-g ]
.RB [ \-n ]
.I \%subfont-name \%x-resolution
.RI [ \%y-scale \ | \ \%y-resolution ]
.ad
.hy
.PP
.in +5m
This mode is intended for use with
.B \%mktexpk
and its derivates.
Only one
.C GF
file together with a 
.C PL
file for the given subfont will be computed, taking the horizontal
resolution and a vertical scaling factor (if the value is smaller than\ 10)
resp. the vertical resolution (otherwise) from the command line, ignoring
the
.B nmb_fonts
parameter of the configuration file.
The last two characters (which are interpreted as the subfont number) are
stripped to get the name for the configuration file (which must end with
\(oq\c
.C \&.cfg \(cq).
No job file will be created.
If option
.B \-p
is set, no
.C PL
file is created.
If
.B \-g
is set, no
.C GF
file is created.
The extension can be controlled with
.BR \-n ;
if set, the extension is \(oq\c
.C \&.gf \(cq,
otherwise \(oq\c
.C \&. <\c
.IR resolution >\c
.C gf \(cq.
.B \-q
makes
.B hbf2gf
quiet.
.
.PP
.in +2m
.na
.nh
.B hbf2gf
'in +\n(.ku
.B \-t
.RB [ \-q ]
.I \%subfont-name
.ad
.hy
.PP
.in +5m
This mode is intended for use with scripts like
.BR \%mktexpk ;
it tests whether the specified subfont name leads to an
.B hbf2gf
configuration file.
It returns 0 on success and prints out the name of that configuration file
(provided the
.B \-q
switch isn't set).
This test isn't a thorough one; it only removes the last two characters
and checks whether a configuration file with that name exists.
.PP
See the next section for more details about configuration files.
.PP
Specifying the option
.B \-\-version
returns the current version of
.B hbf2gf
and the used file search library (e.g.\ \c
.BR kpathsea ).
Usage information is shown with the
.B \-\-help
parameter.
.
.
.SH "CONFIGURATION FILE"
Here a sample configuration file (\c
.C gsfs14.cfg )
for a 56\(mu56 Chinese font in GB encoding; note that all information
about the font is in the
.C jfs56.hbf
file.
See the
.B "FILE SEARCHING"
section how HBF fonts and
.B hbf2gf
configuration files are found.
See the
.B AVAILABILITY
section where to get CJK fonts together with its
.C HBF
files:
.PP
.if t \fC
.nf
  hbf_header     jfs56.hbf
  mag_x          1
  threshold      128
  comment        jianti fansongti 56x56 pixel font

  design_size    14.4

  y_offset       \-13

  nmb_files      \-1

  output_name    gsfs14

  checksum       123456789

  dpi_x          300

  pk_files       no
  tfm_files      yes

  coding         codingscheme GuoBiao encoded TeX text

  pk_directory   $HBF_TARGET/pk/modeless/gb2312/gsfs14/
  tfm_directory  $HBF_TARGET/tfm/gb2312/gsfs14/
.fi
.if t \fP
.PP
A configuration file is a plain text file consisting of keywords and its
arguments.
A keyword must start a line, otherwise the whole line will be ignored.
If the word starting a line is not a keyword, the line will be ignored too.
Empty lines will also be skipped.
The search for keywords is case insensitive; in contrast, the arguments will
be taken exactly as given (except \(oqyes\(cq and \(oqno\(cq which can be written with
uppercase or lowercase letters).
Each keyword has one argument which must be separated by whitespace (blanks
or tabs) from the keyword and must be on the same line.
Each line must not be longer than 256 characters.
.PP
You can use environment variables in the configuration file.
The escape character starting an environment variable in the configuration
file is always \(oq\c
.C $ \(cq,
even for operating systems like DOS which has other conventions.
.B hbf2gf
recognizes only environment variable names which start with a letter or an
underscore, followed by alphanumeric characters or underscores.
You can surround the variable with braces to indicate where the variable
name ends, for example
.C ${FOO} .
To get a dollar sign you must write \(oq\c
.C $$ \(cq.
The expansion of environment variables in hbf2gf itself (without the help of
either kpathsea, emtexdir, or MiKTeX searching routines) is very limited;
this feature has been carried over from previous versions.
It can't expand variables set in texmf.cnf; it also can't handle more than
one directory as the variable's value.
.B Don't use it except for the \(oqpk_directory\(cq and \(oqtfm_directory\(cq
.B parameters!
.PP
This is the list of all necessary keywords:
.TP
.B hbf_header
The HBF header file name of the input font(s).
.B hbf2gf
uses the given searching mechanism (kpathsea, emtexdir, or MiKTeX) to locate
this file.
.TP
.B output_name
The name stem of the output files.
A running two digit decimal number starting with \(oq\c
.C 01 \(cq
will be appended.
For Unicode fonts see the keyword
.B unicode
below.
This value is in almost all cases identical to the name of the configuration
file.
.PP
And now all optional keywords:
.TP
.B x_offset
Increases the character width.
Will be applied on both sides; default for non-rotated glyphs is the value
given in the HBF header
.RB ( HBF_BITMAP_BOUNDING_BOX )
scaled to
.B design_size
(in pixels).
.TP
.B y_offset
Shifts all characters up or down; default for non-rotated glyphs is the value
given in the HBF header
.RB ( HBF_BITMAP_BOUNDING_BOX )
scaled to
.B design_size
(in pixels).
.TP
.B design_size
The design size (in points) of the font.
.B x_offset
and 
.B y_offset
refer to this size.
Default is\ 10.0.
.TP
.B slant
The slant of the font (given as \*(DEx\ /\ \*(DEy).
Only values in the range 0\ \(<=\ \fBslant\fP\ \(<=\ 1 are allowed.
Default is\ 0.0.
.TP
.B rotation
If set to \(oqyes\(cq, all glyphs will be rotated 90\ degrees counter-clockwise.
The default offsets as given in the HBF header will be ignored (and set
to\ 0).
Default is \(oqno\(cq.
.TP
.B mag_x
.TQ
.B mag_y
Scaling values of the characters to reach design size.
If only one magnification is given, x and y values are assumed to be equal.
Default is \fBmag_x\fP\ =\ \fBmag_y\fP\ =\ 1.0.
.PP
.TP
.B threshold
A value between 1 and\ 254 defining a threshold for converting the internal
graymap into the output bitmap; lower values cut more pixels.
Default value is\ 128.
.PP
.TP
.B comment
A comment describing the font; default is none.
.PP
.TP
.B nmb_fonts
The number of subfonts to create.
Default value is \-1 for creating all fonts.
.TP
.B unicode
If \(oqyes\(cq, a two digit hexadecimal number will be used as a running number,
starting with the value of the first byte of the first code range.
Default is \(oqno\(cq.
.TP
.B min_char
The minimum value of the encoding.
You should set this value to get correct subfile offsets if it is not
identical to the lowest character code in the HBF file.
.PP
.TP
.B dpi_x
.TQ
.B dpi_y
The horizontal and vertical resolution (in dpi) of the printer.
If only one resolution is given, x and y values are assumed to be equal.
Default is\ 300.
.TP
.B checksum
A checksum to identify the 
.C GF
files with the appropriate 
.C TFM
files.
The default value of this unsigned 32bit integer is\ 0.
.TP
.B coding
A comment describing the coding scheme; default is none.
.PP
.TP
.B pk_directory
The destination directory of the
.C PK
files; default: none.
Attention!
The batch file will not check whether this directory exists.
.TP
.B tfm_directory
The destination directory of the
.C TFM
files; default: none.
Attention!
The batch file will not check whether this directory exists.
.TP
.B pk_files
Whether to create
.C PK
files or not; default is \(oqyes\(cq.
.TP
.B tfm_files
Whether to create
.C TFM
files or not; default is \(oqyes\(cq.
.TP
.B ofm_file
Whether to create an
.C OPL
file or not; default is \(oqno\(cq.
The batch file will then use
.B ovp2ovf
of the Omega distribution to convert it into an
.C OFM
and an
.C OVF
file.
The
.C OPL
file simply maps all subfonts back to a single Omega font.
.TP
.B long_extension
If \(oqyes\(cq,
.C PK
files will include the resolution in the extension (e.g.
.C gsso1201.300pk ).
This affects the batch file only (default is \(oqyes\(cq).
.TP
.B rm_command
The shell command to remove files; default: \(oqrm\(cq.
.TP
.B cp_command
The shell command to copy files; default: \(oqcp\(cq.
.TP
.B job_extension
The extension of the batch file which calls
.B gftopk
and
.B pltotf
to convert the
.C GF
and the
.C PL
files into
.C PK
and
.C TFM
files respectively; default is none.
.
.
.SH "FILE SEARCHING"
.B hbf2gf
uses either the
.BR kpathsea ,
.BR emtexdir ,
or
.B MiKTeX
library for searching files 
.RB ( emtexdir
will work only on operating systems which have an MS-DOSish background,
i.e., MS-DOS, OS/2, Windows;
.B MiKTeX
is for Win32 systems).
.
.SS kpathsea
The actual version of kpathsea is displayed on screen if you call
.B hbf2gf
.BR \-\-version .
.PP
Here is a table of the file type and the corresponding
.B kpathsea
variables.
.PP
.in +4m
.ta 2i
.br
.C "\&.hbf	MISCFONTS"
.br
.C "\&.cfg	HBF2GFINPUTS"
.PP
Please consult the info files of
.B kpathsea
for details on these variables.
The decision which naming scheme to use for variables will be done during
compilation.
.PP
You should set the
.C TEXMFCNF
variable to the directory where your
.C texmf.cnf
configuration file resides.
.PP
Here is the proper command to find out to which value a
.B kpathsea
variable is set (we use
.C MISCFONTS
as an example).
This is especially useful if a variable isn't set in
.C texmf.cnf
or in the environment, thus pointing to the default value which is
hard-coded into the
.B kpathsea
library.
.PP
.in +2m
.C "kpsewhich \-progname=hbf2gf \-expand\-var='$MISCFONTS'"
.PP
We select the program name also since it is possible to specify
variables which are searched only for a certain program \(en in our
example it would be
.C MISCFONTS.hbf2gf .
.PP
A similar but not identical method is to say
.PP
.in +2m
.C "kpsewhich \-progname=hbf2gf \-show\-path='misc fonts'"
.PP
[A full list of format types can be obtained by saying \(oq\c
.C "kpsewhich \-\-help" \(cq
on the command line prompt.]
This is exactly how
.B hbf2gf
searches for files; the disadvantage is that all variables are expanded
which can cause very long strings.
.
.SS emtexdir
.PP
Here the list of suffixes and its related environment variables to be set in
.C autoexec.bat
(resp. in
.C config.sys
for OS/2):
.PP
.in +4m
.ta 2i
.br
.C "\&.hbf	HBFONTS"
.br
.C "\&.cfg	HBFCFG"
.PP
If one of the variables isn't set, a warning message is emitted.
The current directory will always be searched.
As usual, one exclamation mark appended to a directory path causes
subdirectories one level deep to be searched, two exclamation marks causes
all subdirectories to be searched.
Example:
.PP
.in +2m
.C HBFONTS=c:\\\\fonts\\\\hbf!!;d:\\\\myfonts\\\\hbf!
.PP
Constructions like \(oq\c
.C c:\\\\fonts!!\\\\hbf \(cq
aren't possible.
.
.SS MikTeX
.PP
Please consult the documentation files of
.B MiKTeX
for more details.
.
.
.SH LIMITATIONS
The x and y output size must not exceed
.BR MAX_CHAR_SIZE ,
which is defined at compile time; its default value is 1023\ (pixel).
.
.
.SH "SEE ALSO"
.BR ttf2pk (1)
.PP
.C hbf2gf.w :
'in +\n(.ku
this is the source code written in
.B CWEB
which can be converted into a pretty-printed \*(TX
document using
.BR cweave .
The CJK package also contains a preformatted
.C hbf2gf.pdf
file.
.PP
the
.B CJK
documentation files (\c
.C hbf2gf.txt ).
.PP
the
.B Hanzi Bitmap File
.RB ( HBF )
standard version\ 1.3; available at
.C \%ftp.ifcss.org .
.PP
the Omega documentation available at
.C ftp.ens.fr
and the CTAN hosts and mirrors.
.
.
.SH FILES
.TP
.C *.cfg
The
.B hbf2gf
configuration scripts.
.TP
.C *.hbf
HBF header files which describe fixed-width bitmap fonts.
Note that the bitmap font name(s) themselves as specified in the header files
are irrelevant for
.BR hbf2gf .
.
.
.SH AVAILABILITY
.B hbf2gf
is part of the CJK macro package for \*(LE
available at the CTAN hosts and its mirrors.
.PP
CJK fonts together with HBF header files can be found at
.C ftp.ifcss.org
and its mirrors.
.
.
.SH AUTHORS
Werner Lemberg
.C <wl@gnu.org>
.br
Ross Paterson (the HBF API)
.C <ross@soi.city.ac.uk>


==> cjk-4.8.5/utils/hbf2gf/install-sh <==
#!/bin/sh
# install - install a program, script, or datafile

scriptversion=2020-11-14.01; # UTC

# This originates from X11R5 (mit/util/scripts/install.sh), which was
# later released in X11R6 (xc/config/util/install.sh) with the
# following copyright and license.
#
# Copyright (C) 1994 X Consortium
#
# Permission is hereby granted, free of charge, to any person obtaining a copy
# of this software and associated documentation files (the "Software"), to
# deal in the Software without restriction, including without limitation the
# rights to use, copy, modify, merge, publish, distribute, sublicense, and/or
# sell copies of the Software, and to permit persons to whom the Software is
# furnished to do so, subject to the following conditions:
#
# The above copyright notice and this permission notice shall be included in
# all copies or substantial portions of the Software.
#
# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND, EXPRESS OR
# IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF MERCHANTABILITY,
# FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.  IN NO EVENT SHALL THE
# X CONSORTIUM BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN
# AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNEC-
# TION WITH THE SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE.
#
# Except as contained in this notice, the name of the X Consortium shall not
# be used in advertising or otherwise to promote the sale, use or other deal-
# ings in this Software without prior written authorization from the X Consor-
# tium.
#
#
# FSF changes to this file are in the public domain.
#
# Calling this script install-sh is preferred over install.sh, to prevent
# 'make' implicit rules from creating a file called install from it
# when there is no Makefile.
#
# This script is compatible with the BSD install script, but was written
# from scratch.

tab='	'
nl='
'
IFS=" $tab$nl"

# Set DOITPROG to "echo" to test this script.

doit=${DOITPROG-}
doit_exec=${doit:-exec}

# Put in absolute file names if you don't have them in your path;
# or use environment vars.

chgrpprog=${CHGRPPROG-chgrp}
chmodprog=${CHMODPROG-chmod}
chownprog=${CHOWNPROG-chown}
cmpprog=${CMPPROG-cmp}
cpprog=${CPPROG-cp}
mkdirprog=${MKDIRPROG-mkdir}
mvprog=${MVPROG-mv}
rmprog=${RMPROG-rm}
stripprog=${STRIPPROG-strip}

posix_mkdir=

# Desired mode of installed file.
mode=0755

# Create dirs (including intermediate dirs) using mode 755.
# This is like GNU 'install' as of coreutils 8.32 (2020).
mkdir_umask=22

backupsuffix=
chgrpcmd=
chmodcmd=$chmodprog
chowncmd=
mvcmd=$mvprog
rmcmd="$rmprog -f"
stripcmd=

src=
dst=
dir_arg=
dst_arg=

copy_on_change=false
is_target_a_directory=possibly

usage="\
Usage: $0 [OPTION]... [-T] SRCFILE DSTFILE
   or: $0 [OPTION]... SRCFILES... DIRECTORY
   or: $0 [OPTION]... -t DIRECTORY SRCFILES...
   or: $0 [OPTION]... -d DIRECTORIES...

In the 1st form, copy SRCFILE to DSTFILE.
In the 2nd and 3rd, copy all SRCFILES to DIRECTORY.
In the 4th, create DIRECTORIES.

Options:
     --help     display this help and exit.
     --version  display version info and exit.

  -c            (ignored)
  -C            install only if different (preserve data modification time)
  -d            create directories instead of installing files.
  -g GROUP      $chgrpprog installed files to GROUP.
  -m MODE       $chmodprog installed files to MODE.
  -o USER       $chownprog installed files to USER.
  -p            pass -p to $cpprog.
  -s            $stripprog installed files.
  -S SUFFIX     attempt to back up existing files, with suffix SUFFIX.
  -t DIRECTORY  install into DIRECTORY.
  -T            report an error if DSTFILE is a directory.

Environment variables override the default commands:
  CHGRPPROG CHMODPROG CHOWNPROG CMPPROG CPPROG MKDIRPROG MVPROG
  RMPROG STRIPPROG

By default, rm is invoked with -f; when overridden with RMPROG,
it's up to you to specify -f if you want it.

If -S is not specified, no backups are attempted.

Email bug reports to bug-automake@gnu.org.
Automake home page: https://www.gnu.org/software/automake/
"

while test $# -ne 0; do
  case $1 in
    -c) ;;

    -C) copy_on_change=true;;

    -d) dir_arg=true;;

    -g) chgrpcmd="$chgrpprog $2"
        shift;;

    --help) echo "$usage"; exit $?;;

    -m) mode=$2
        case $mode in
          *' '* | *"$tab"* | *"$nl"* | *'*'* | *'?'* | *'['*)
            echo "$0: invalid mode: $mode" >&2
            exit 1;;
        esac
        shift;;

    -o) chowncmd="$chownprog $2"
        shift;;

    -p) cpprog="$cpprog -p";;

    -s) stripcmd=$stripprog;;

    -S) backupsuffix="$2"
        shift;;

    -t)
        is_target_a_directory=always
        dst_arg=$2
        # Protect names problematic for 'test' and other utilities.
        case $dst_arg in
          -* | [=\(\)!]) dst_arg=./$dst_arg;;
        esac
        shift;;

    -T) is_target_a_directory=never;;

    --version) echo "$0 $scriptversion"; exit $?;;

    --) shift
        break;;

    -*) echo "$0: invalid option: $1" >&2
        exit 1;;

    *)  break;;
  esac
  shift
done

# We allow the use of options -d and -T together, by making -d
# take the precedence; this is for compatibility with GNU install.

if test -n "$dir_arg"; then
  if test -n "$dst_arg"; then
    echo "$0: target directory not allowed when installing a directory." >&2
    exit 1
  fi
fi

if test $# -ne 0 && test -z "$dir_arg$dst_arg"; then
  # When -d is used, all remaining arguments are directories to create.
  # When -t is used, the destination is already specified.
  # Otherwise, the last argument is the destination.  Remove it from $@.
  for arg
  do
    if test -n "$dst_arg"; then
      # $@ is not empty: it contains at least $arg.
      set fnord "$@" "$dst_arg"
      shift # fnord
    fi
    shift # arg
    dst_arg=$arg
    # Protect names problematic for 'test' and other utilities.
    case $dst_arg in
      -* | [=\(\)!]) dst_arg=./$dst_arg;;
    esac
  done
fi

if test $# -eq 0; then
  if test -z "$dir_arg"; then
    echo "$0: no input file specified." >&2
    exit 1
  fi
  # It's OK to call 'install-sh -d' without argument.
  # This can happen when creating conditional directories.
  exit 0
fi

if test -z "$dir_arg"; then
  if test $# -gt 1 || test "$is_target_a_directory" = always; then
    if test ! -d "$dst_arg"; then
      echo "$0: $dst_arg: Is not a directory." >&2
      exit 1
    fi
  fi
fi

if test -z "$dir_arg"; then
  do_exit='(exit $ret); exit $ret'
  trap "ret=129; $do_exit" 1
  trap "ret=130; $do_exit" 2
  trap "ret=141; $do_exit" 13
  trap "ret=143; $do_exit" 15

  # Set umask so as not to create temps with too-generous modes.
  # However, 'strip' requires both read and write access to temps.
  case $mode in
    # Optimize common cases.
    *644) cp_umask=133;;
    *755) cp_umask=22;;

    *[0-7])
      if test -z "$stripcmd"; then
        u_plus_rw=
      else
        u_plus_rw='% 200'
      fi
      cp_umask=`expr '(' 777 - $mode % 1000 ')' $u_plus_rw`;;
    *)
      if test -z "$stripcmd"; then
        u_plus_rw=
      else
        u_plus_rw=,u+rw
      fi
      cp_umask=$mode$u_plus_rw;;
  esac
fi

for src
do
  # Protect names problematic for 'test' and other utilities.
  case $src in
    -* | [=\(\)!]) src=./$src;;
  esac

  if test -n "$dir_arg"; then
    dst=$src
    dstdir=$dst
    test -d "$dstdir"
    dstdir_status=$?
    # Don't chown directories that already exist.
    if test $dstdir_status = 0; then
      chowncmd=""
    fi
  else

    # Waiting for this to be detected by the "$cpprog $src $dsttmp" command
    # might cause directories to be created, which would be especially bad
    # if $src (and thus $dsttmp) contains '*'.
    if test ! -f "$src" && test ! -d "$src"; then
      echo "$0: $src does not exist." >&2
      exit 1
    fi

    if test -z "$dst_arg"; then
      echo "$0: no destination specified." >&2
      exit 1
    fi
    dst=$dst_arg

    # If destination is a directory, append the input filename.
    if test -d "$dst"; then
      if test "$is_target_a_directory" = never; then
        echo "$0: $dst_arg: Is a directory" >&2
        exit 1
      fi
      dstdir=$dst
      dstbase=`basename "$src"`
      case $dst in
	*/) dst=$dst$dstbase;;
	*)  dst=$dst/$dstbase;;
      esac
      dstdir_status=0
    else
      dstdir=`dirname "$dst"`
      test -d "$dstdir"
      dstdir_status=$?
    fi
  fi

  case $dstdir in
    */) dstdirslash=$dstdir;;
    *)  dstdirslash=$dstdir/;;
  esac

  obsolete_mkdir_used=false

  if test $dstdir_status != 0; then
    case $posix_mkdir in
      '')
        # With -d, create the new directory with the user-specified mode.
        # Otherwise, rely on $mkdir_umask.
        if test -n "$dir_arg"; then
          mkdir_mode=-m$mode
        else
          mkdir_mode=
        fi

        posix_mkdir=false
	# The $RANDOM variable is not portable (e.g., dash).  Use it
	# here however when possible just to lower collision chance.
	tmpdir=${TMPDIR-/tmp}/ins$RANDOM-$$

	trap '
	  ret=$?
	  rmdir "$tmpdir/a/b" "$tmpdir/a" "$tmpdir" 2>/dev/null
	  exit $ret
	' 0

	# Because "mkdir -p" follows existing symlinks and we likely work
	# directly in world-writeable /tmp, make sure that the '$tmpdir'
	# directory is successfully created first before we actually test
	# 'mkdir -p'.
	if (umask $mkdir_umask &&
	    $mkdirprog $mkdir_mode "$tmpdir" &&
	    exec $mkdirprog $mkdir_mode -p -- "$tmpdir/a/b") >/dev/null 2>&1
	then
	  if test -z "$dir_arg" || {
	       # Check for POSIX incompatibilities with -m.
	       # HP-UX 11.23 and IRIX 6.5 mkdir -m -p sets group- or
	       # other-writable bit of parent directory when it shouldn't.
	       # FreeBSD 6.1 mkdir -m -p sets mode of existing directory.
	       test_tmpdir="$tmpdir/a"
	       ls_ld_tmpdir=`ls -ld "$test_tmpdir"`
	       case $ls_ld_tmpdir in
		 d????-?r-*) different_mode=700;;
		 d????-?--*) different_mode=755;;
		 *) false;;
	       esac &&
	       $mkdirprog -m$different_mode -p -- "$test_tmpdir" && {
		 ls_ld_tmpdir_1=`ls -ld "$test_tmpdir"`
		 test "$ls_ld_tmpdir" = "$ls_ld_tmpdir_1"
	       }
	     }
	  then posix_mkdir=:
	  fi
	  rmdir "$tmpdir/a/b" "$tmpdir/a" "$tmpdir"
	else
	  # Remove any dirs left behind by ancient mkdir implementations.
	  rmdir ./$mkdir_mode ./-p ./-- "$tmpdir" 2>/dev/null
	fi
	trap '' 0;;
    esac

    if
      $posix_mkdir && (
        umask $mkdir_umask &&
        $doit_exec $mkdirprog $mkdir_mode -p -- "$dstdir"
      )
    then :
    else

      # mkdir does not conform to POSIX,
      # or it failed possibly due to a race condition.  Create the
      # directory the slow way, step by step, checking for races as we go.

      case $dstdir in
        /*) prefix='/';;
        [-=\(\)!]*) prefix='./';;
        *)  prefix='';;
      esac

      oIFS=$IFS
      IFS=/
      set -f
      set fnord $dstdir
      shift
      set +f
      IFS=$oIFS

      prefixes=

      for d
      do
        test X"$d" = X && continue

        prefix=$prefix$d
        if test -d "$prefix"; then
          prefixes=
        else
          if $posix_mkdir; then
            (umask $mkdir_umask &&
             $doit_exec $mkdirprog $mkdir_mode -p -- "$dstdir") && break
            # Don't fail if two instances are running concurrently.
            test -d "$prefix" || exit 1
          else
            case $prefix in
              *\'*) qprefix=`echo "$prefix" | sed "s/'/'\\\\\\\\''/g"`;;
              *) qprefix=$prefix;;
            esac
            prefixes="$prefixes '$qprefix'"
          fi
        fi
        prefix=$prefix/
      done

      if test -n "$prefixes"; then
        # Don't fail if two instances are running concurrently.
        (umask $mkdir_umask &&
         eval "\$doit_exec \$mkdirprog $prefixes") ||
          test -d "$dstdir" || exit 1
        obsolete_mkdir_used=true
      fi
    fi
  fi

  if test -n "$dir_arg"; then
    { test -z "$chowncmd" || $doit $chowncmd "$dst"; } &&
    { test -z "$chgrpcmd" || $doit $chgrpcmd "$dst"; } &&
    { test "$obsolete_mkdir_used$chowncmd$chgrpcmd" = false ||
      test -z "$chmodcmd" || $doit $chmodcmd $mode "$dst"; } || exit 1
  else

    # Make a couple of temp file names in the proper directory.
    dsttmp=${dstdirslash}_inst.$$_
    rmtmp=${dstdirslash}_rm.$$_

    # Trap to clean up those temp files at exit.
    trap 'ret=$?; rm -f "$dsttmp" "$rmtmp" && exit $ret' 0

    # Copy the file name to the temp name.
    (umask $cp_umask &&
     { test -z "$stripcmd" || {
	 # Create $dsttmp read-write so that cp doesn't create it read-only,
	 # which would cause strip to fail.
	 if test -z "$doit"; then
	   : >"$dsttmp" # No need to fork-exec 'touch'.
	 else
	   $doit touch "$dsttmp"
	 fi
       }
     } &&
     $doit_exec $cpprog "$src" "$dsttmp") &&

    # and set any options; do chmod last to preserve setuid bits.
    #
    # If any of these fail, we abort the whole thing.  If we want to
    # ignore errors from any of these, just make sure not to ignore
    # errors from the above "$doit $cpprog $src $dsttmp" command.
    #
    { test -z "$chowncmd" || $doit $chowncmd "$dsttmp"; } &&
    { test -z "$chgrpcmd" || $doit $chgrpcmd "$dsttmp"; } &&
    { test -z "$stripcmd" || $doit $stripcmd "$dsttmp"; } &&
    { test -z "$chmodcmd" || $doit $chmodcmd $mode "$dsttmp"; } &&

    # If -C, don't bother to copy if it wouldn't change the file.
    if $copy_on_change &&
       old=`LC_ALL=C ls -dlL "$dst"     2>/dev/null` &&
       new=`LC_ALL=C ls -dlL "$dsttmp"  2>/dev/null` &&
       set -f &&
       set X $old && old=:$2:$4:$5:$6 &&
       set X $new && new=:$2:$4:$5:$6 &&
       set +f &&
       test "$old" = "$new" &&
       $cmpprog "$dst" "$dsttmp" >/dev/null 2>&1
    then
      rm -f "$dsttmp"
    else
      # If $backupsuffix is set, and the file being installed
      # already exists, attempt a backup.  Don't worry if it fails,
      # e.g., if mv doesn't support -f.
      if test -n "$backupsuffix" && test -f "$dst"; then
        $doit $mvcmd -f "$dst" "$dst$backupsuffix" 2>/dev/null
      fi

      # Rename the file to the real destination.
      $doit $mvcmd -f "$dsttmp" "$dst" 2>/dev/null ||

      # The rename failed, perhaps because mv can't rename something else
      # to itself, or perhaps because mv is so ancient that it does not
      # support -f.
      {
        # Now remove or move aside any old file at destination location.
        # We try this two ways since rm can't unlink itself on some
        # systems and the destination file might be busy for other
        # reasons.  In this case, the final cleanup might fail but the new
        # file should still install successfully.
        {
          test ! -f "$dst" ||
          $doit $rmcmd "$dst" 2>/dev/null ||
          { $doit $mvcmd -f "$dst" "$rmtmp" 2>/dev/null &&
            { $doit $rmcmd "$rmtmp" 2>/dev/null; :; }
          } ||
          { echo "$0: cannot unlink or rename $dst" >&2
            (exit 1); exit 1
          }
        } &&

        # Now rename the file to the real destination.
        $doit $mvcmd "$dsttmp" "$dst"
      }
    fi || exit 1

    trap '' 0
  fi
done

# Local variables:
# eval: (add-hook 'before-save-hook 'time-stamp)
# time-stamp-start: "scriptversion="
# time-stamp-format: "%:y-%02m-%02d.%02H"
# time-stamp-time-zone: "UTC0"
# time-stamp-end: "; # UTC"
# End:


==> cjk-4.8.5/utils/hbf2gf/mkinstalldirs <==
#! /bin/sh
# mkinstalldirs --- make directory hierarchy

scriptversion=2020-07-26.22; # UTC

# Original author: Noah Friedman <friedman@prep.ai.mit.edu>
# Created: 1993-05-16
# Public domain.
#
# This file is maintained in Automake, please report
# bugs to <bug-automake@gnu.org> or send patches to
# <automake-patches@gnu.org>.

nl='
'
IFS=" ""	$nl"
errstatus=0
dirmode=

usage="\
Usage: mkinstalldirs [-h] [--help] [--version] [-m MODE] DIR ...

Create each directory DIR (with mode MODE, if specified), including all
leading file name components.

Report bugs to <bug-automake@gnu.org>."

# process command line arguments
while test $# -gt 0 ; do
  case $1 in
    -h | --help | --h*)         # -h for help
      echo "$usage"
      exit $?
      ;;
    -m)                         # -m PERM arg
      shift
      test $# -eq 0 && { echo "$usage" 1>&2; exit 1; }
      dirmode=$1
      shift
      ;;
    --version)
      echo "$0 $scriptversion"
      exit $?
      ;;
    --)                         # stop option processing
      shift
      break
      ;;
    -*)                         # unknown option
      echo "$usage" 1>&2
      exit 1
      ;;
    *)                          # first non-opt arg
      break
      ;;
  esac
done

for file
do
  if test -d "$file"; then
    shift
  else
    break
  fi
done

case $# in
  0) exit 0 ;;
esac

# Solaris 8's mkdir -p isn't thread-safe.  If you mkdir -p a/b and
# mkdir -p a/c at the same time, both will detect that a is missing,
# one will create a, then the other will try to create a and die with
# a "File exists" error.  This is a problem when calling mkinstalldirs
# from a parallel make.  We use --version in the probe to restrict
# ourselves to GNU mkdir, which is thread-safe.
case $dirmode in
  '')
    if mkdir -p --version . >/dev/null 2>&1 && test ! -d ./--version; then
      echo "mkdir -p -- $*"
      exec mkdir -p -- "$@"
    else
      # On NextStep and OpenStep, the 'mkdir' command does not
      # recognize any option.  It will interpret all options as
      # directories to create, and then abort because '.' already
      # exists.
      test -d ./-p && rmdir ./-p
      test -d ./--version && rmdir ./--version
    fi
    ;;
  *)
    if mkdir -m "$dirmode" -p --version . >/dev/null 2>&1 &&
       test ! -d ./--version; then
      echo "umask 22"
      umask 22
      echo "mkdir -m $dirmode -p -- $*"
      exec mkdir -m "$dirmode" -p -- "$@"
    else
      # Clean up after NextStep and OpenStep mkdir.
      for d in ./-m ./-p ./--version "./$dirmode";
      do
        test -d $d && rmdir $d
      done
    fi
    ;;
esac

echo "umask 22"
umask 22

for file
do
  case $file in
    /*) pathcomp=/ ;;
    *)  pathcomp= ;;
  esac
  oIFS=$IFS
  IFS=/
  set fnord $file
  shift
  IFS=$oIFS

  for d
  do
    test "x$d" = x && continue

    pathcomp=$pathcomp$d
    case $pathcomp in
      -*) pathcomp=./$pathcomp ;;
    esac

    if test ! -d "$pathcomp"; then
      echo "mkdir $pathcomp"

      mkdir "$pathcomp" || lasterr=$?

      if test ! -d "$pathcomp"; then
	errstatus=$lasterr
      fi
    fi

    pathcomp=$pathcomp/
  done

  if test ! -z "$dirmode"; then
    echo "chmod $dirmode $file"
    chmod "$dirmode" "$file" || errstatus=$?
  fi
done

exit $errstatus

# Local Variables:
# mode: shell-script
# sh-indentation: 2
# eval: (add-hook 'before-save-hook 'time-stamp)
# time-stamp-start: "scriptversion="
# time-stamp-format: "%:y-%02m-%02d.%02H"
# time-stamp-time-zone: "UTC0"
# time-stamp-end: "; # UTC"
# End:


==> cjk-4.8.5/utils/pyhyphen/GNUmakefile <==
# Makefile to create hyphenation patterns for pinyin with tone marks and
# pinyin without tone marks.

BASH = bash
CC = cc
DATE = date
GIT = git
ICONV = iconv -f latin1 -t utf8
RM = rm -f
SED = sed # should be GNU sed

GIT_VERSION = $(shell $(GIT) log --format=%H -1 HEAD --)
LEFTHYPHENMIN = $(strip $(shell $(SED) 's/^\(..\).*/\1/;q' < pinyin.tr))
RIGHTHYPHENMIN = $(strip $(shell $(SED) 's/^..\(..\).*/\1/;q' < pinyin.tr))
TODAY = $(shell $(DATE) '+%Y-%m-%d')


all: hyph-zh-latn-pinyin.tex \
     hyph-zh-latn-tonepinyin.tex

pinyin: pinyin.c
	$(CC) -o $@ $<

pinyin.dic: pinyin
	./$< > $@

pattern.rules pinyin.pat: make-patterns.sh \
                          pinyin.dic \
                          pinyin.tr
	$(BASH) make-patterns.sh pinyin.dic pinyin.tr \
        && $(ICONV) < pattern.2 > pinyin.pat

tonepinyin.pat: pinyin.pat
	LANG=en_US.UTF-8 \
        $(SED) -e 's/\(.*\)a\(.*\)/\1a\2 \1ā\2 \1á\2 \1ǎ\2 \1à\2/' \
               -e 's/\(.*\)e\(.*\)/\1e\2 \1ē\2 \1é\2 \1ě\2 \1è\2/' \
               -e 's/\(.*\)i\(.*\)/\1i\2 \1ī\2 \1í\2 \1ǐ\2 \1ì\2/' \
               -e 's/\(.*\)o\(.*\)/\1o\2 \1ō\2 \1ó\2 \1ǒ\2 \1ò\2/' \
               -e 's/\(.*\)u\(.*\)/\1u\2 \1ū\2 \1ú\2 \1ǔ\2 \1ù\2/' \
               -e 's/\(.*\)ü\(.*\)/\1ü\2 \1ǖ\2 \1ǘ\2 \1ǚ\2 \1ǜ\2/' \
               < $< > $@

hyph-zh-latn-pinyin.tex: hyph-zh-latn-pinyin.in \
                         pattern.rules \
                         pinyin.pat
	$(SED) -e 's/@WITH@/without/' \
               -e 's/@DATE@/$(TODAY)/' \
               -e 's/@GIT_VERSION@/$(GIT_VERSION)/' \
               -e 's/@LEFTHYPHENMIN@/$(LEFTHYPHENMIN)/' \
               -e 's/@RIGHTHYPHENMIN@/$(RIGHTHYPHENMIN)/' \
               -e '/used patgen parameters/ r pattern.rules' \
               -e '/\\patterns/ r pinyin.pat' \
               < $< > $@

hyph-zh-latn-tonepinyin.tex: hyph-zh-latn-pinyin.in \
                             pattern.rules \
                             tonepinyin.pat
	$(SED) -e 's/@WITH@/with/' \
               -e 's/@DATE@/$(TODAY)/' \
               -e 's/@GIT_VERSION@/$(GIT_VERSION)/' \
               -e 's/@LEFTHYPHENMIN@/$(LEFTHYPHENMIN)/' \
               -e 's/@RIGHTHYPHENMIN@/$(RIGHTHYPHENMIN)/' \
               -e '/used patgen parameters/ r pattern.rules' \
               -e '/\\patterns/ r tonepinyin.pat' \
               < $< > $@

clean:
	$(RM) pinyin pinyin.dic pinyin.pat tonepinyin.pat
	$(RM) pattern.*
	$(RM) pattmp.*

# Local Variables:
# mode: makefile
# coding: utf-8
# End:


==> cjk-4.8.5/utils/pyhyphen/hyph-zh-latn-pinyin.tex <==
% title: Hyphenation patterns for Chinese pinyin (Mandarin), without tone
%        markers
%
% version: 2018-11-25
%
% authors:
%   -
%     name:    Werner Lemberg
%     contact: wl (at) gnu.org
%
% copyright: Copyright (C) 1994-2018 Werner Lemberg
%
% licence:
%     name: MIT
%     url:  http://opensource.org/licenses/mit-license.php
%     text: >
%           Permission is hereby granted, free of charge, to any person
%           obtaining a copy of this software and associated documentation
%           files (the “Software”), to deal in the Software without
%           restriction, including without limitation the rights to use,
%           copy, modify, merge, publish, distribute, sublicense, and/or
%           sell copies of the Software, and to permit persons to whom the
%           Software is furnished to do so, subject to the following
%           conditions:
%
%           The above copyright notice and this permission notice shall be
%           included in all copies or substantial portions of the Software.
%
%           THE SOFTWARE IS PROVIDED “AS IS”, WITHOUT WARRANTY OF ANY KIND,
%           EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES
%           OF MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND
%           NONINFRINGEMENT.  IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT
%           HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER LIABILITY,
%           WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING
%           FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR
%           OTHER DEALINGS IN THE SOFTWARE.
%
% source: http://git.savannah.gnu.org/gitweb/?p=cjk.git;a=commit;h=e058ceae5561a89e33828f593b094c8b57f6a72e
%
% language:
%     name: Mandarin Chinese, pinyin transliteration (without tone markers)
%     tag:  zh-latn-pinyin
%
% hyphenmins:
%     generation:
%         left:  1
%         right: 2
%     typesetting:
%         left:  1
%         right: 2

\message{Pinyin Hyphenation Patterns (without tone markers) 2018-11-25 (WL)}

%
% The used patgen parameters are
%
%   1 1 | 2 5 | 1 1 1
%   2 2 | 2 5 | 1 2 1
%

\patterns{
a1b
a1c
a1d
a1f
a1g
a1h
a1j
a1k
a1l
a1m
a1p
a1q
a1r
a1s
a1t
a1w
a1x
a1y
a1z
e1b
e1c
e1d
e1f
e1g
e1h
e1j
e1k
e1l
e1m
e1p
e1q
e1r
e1s
e1t
e1w
e1x
e1y
e1z
1ga
g1b
g1c
g1d
1ge
g1f
g1g
g1h
g1j
g1k
g1l
g1m
g1n
1go
g1p
g1q
g1r
g1s
g1t
1gu
g1w
g1x
g1y
g1z
i1b
i1c
i1d
i1f
i1g
i1h
i1j
i1k
i1l
i1m
i1p
i1q
i1r
i1s
i1t
i1w
i1x
i1y
i1z
1na
n1b
n1c
n1d
1ne
n1f
n1h
1ni
n1j
n1k
n1l
n1m
n1n
1no
n1p
n1q
n1r
n1s
n1t
1nu
1nü
n1w
n1x
n1y
n1z
o1b
o1c
o1d
o1f
o1g
o1h
o1j
o1k
o1l
o1m
o1p
o1q
o1r
o1s
o1t
o1w
o1x
o1y
o1z
2r1b
2r1c
2r1d
2r1f
2r1g
2r1h
2r1j
2r1k
2r1l
2r1m
2r1n
2r1p
2r1q
2r1r
2r1s
2r1t
2r1w
2r1x
2r1y
2r1z
u1b
u1c
u1d
u1f
u1g
u1h
u1j
u1k
u1l
u1m
u1p
u1q
u1r
u1s
u1t
u1w
u1x
u1y
u1z
ü1b
ü1c
ü1d
ü1f
ü1g
ü1h
ü1j
ü1k
ü1l
ü1m
ü1n
ü1p
ü1q
ü1r
ü1s
ü1t
ü1w
ü1x
ü1y
ü1z
}

\endinput

%%% Local Variables:
%%% mode: tex
%%% coding: utf-8
%%% End:


==> cjk-4.8.5/utils/pyhyphen/hyph-zh-latn-tonepinyin.tex <==
% title: Hyphenation patterns for Chinese pinyin (Mandarin), with tone
%        markers
%
% version: 2018-11-25
%
% authors:
%   -
%     name:    Werner Lemberg
%     contact: wl (at) gnu.org
%
% copyright: Copyright (C) 1994-2018 Werner Lemberg
%
% licence:
%     name: MIT
%     url:  http://opensource.org/licenses/mit-license.php
%     text: >
%           Permission is hereby granted, free of charge, to any person
%           obtaining a copy of this software and associated documentation
%           files (the “Software”), to deal in the Software without
%           restriction, including without limitation the rights to use,
%           copy, modify, merge, publish, distribute, sublicense, and/or
%           sell copies of the Software, and to permit persons to whom the
%           Software is furnished to do so, subject to the following
%           conditions:
%
%           The above copyright notice and this permission notice shall be
%           included in all copies or substantial portions of the Software.
%
%           THE SOFTWARE IS PROVIDED “AS IS”, WITHOUT WARRANTY OF ANY KIND,
%           EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES
%           OF MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND
%           NONINFRINGEMENT.  IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT
%           HOLDERS BE LIABLE FOR ANY CLAIM, DAMAGES OR OTHER LIABILITY,
%           WHETHER IN AN ACTION OF CONTRACT, TORT OR OTHERWISE, ARISING
%           FROM, OUT OF OR IN CONNECTION WITH THE SOFTWARE OR THE USE OR
%           OTHER DEALINGS IN THE SOFTWARE.
%
% source: http://git.savannah.gnu.org/gitweb/?p=cjk.git;a=commit;h=e058ceae5561a89e33828f593b094c8b57f6a72e
%
% language:
%     name: Mandarin Chinese, pinyin transliteration (with tone markers)
%     tag:  zh-latn-pinyin
%
% hyphenmins:
%     generation:
%         left:  1
%         right: 2
%     typesetting:
%         left:  1
%         right: 2

\message{Pinyin Hyphenation Patterns (with tone markers) 2018-11-25 (WL)}

%
% The used patgen parameters are
%
%   1 1 | 2 5 | 1 1 1
%   2 2 | 2 5 | 1 2 1
%

\patterns{
a1b ā1b á1b ǎ1b à1b
a1c ā1c á1c ǎ1c à1c
a1d ā1d á1d ǎ1d à1d
a1f ā1f á1f ǎ1f à1f
a1g ā1g á1g ǎ1g à1g
a1h ā1h á1h ǎ1h à1h
a1j ā1j á1j ǎ1j à1j
a1k ā1k á1k ǎ1k à1k
a1l ā1l á1l ǎ1l à1l
a1m ā1m á1m ǎ1m à1m
a1p ā1p á1p ǎ1p à1p
a1q ā1q á1q ǎ1q à1q
a1r ā1r á1r ǎ1r à1r
a1s ā1s á1s ǎ1s à1s
a1t ā1t á1t ǎ1t à1t
a1w ā1w á1w ǎ1w à1w
a1x ā1x á1x ǎ1x à1x
a1y ā1y á1y ǎ1y à1y
a1z ā1z á1z ǎ1z à1z
e1b ē1b é1b ě1b è1b
e1c ē1c é1c ě1c è1c
e1d ē1d é1d ě1d è1d
e1f ē1f é1f ě1f è1f
e1g ē1g é1g ě1g è1g
e1h ē1h é1h ě1h è1h
e1j ē1j é1j ě1j è1j
e1k ē1k é1k ě1k è1k
e1l ē1l é1l ě1l è1l
e1m ē1m é1m ě1m è1m
e1p ē1p é1p ě1p è1p
e1q ē1q é1q ě1q è1q
e1r ē1r é1r ě1r è1r
e1s ē1s é1s ě1s è1s
e1t ē1t é1t ě1t è1t
e1w ē1w é1w ě1w è1w
e1x ē1x é1x ě1x è1x
e1y ē1y é1y ě1y è1y
e1z ē1z é1z ě1z è1z
1ga 1gā 1gá 1gǎ 1gà
g1b
g1c
g1d
1ge 1gē 1gé 1gě 1gè
g1f
g1g
g1h
g1j
g1k
g1l
g1m
g1n
1go 1gō 1gó 1gǒ 1gò
g1p
g1q
g1r
g1s
g1t
1gu 1gū 1gú 1gǔ 1gù
g1w
g1x
g1y
g1z
i1b ī1b í1b ǐ1b ì1b
i1c ī1c í1c ǐ1c ì1c
i1d ī1d í1d ǐ1d ì1d
i1f ī1f í1f ǐ1f ì1f
i1g ī1g í1g ǐ1g ì1g
i1h ī1h í1h ǐ1h ì1h
i1j ī1j í1j ǐ1j ì1j
i1k ī1k í1k ǐ1k ì1k
i1l ī1l í1l ǐ1l ì1l
i1m ī1m í1m ǐ1m ì1m
i1p ī1p í1p ǐ1p ì1p
i1q ī1q í1q ǐ1q ì1q
i1r ī1r í1r ǐ1r ì1r
i1s ī1s í1s ǐ1s ì1s
i1t ī1t í1t ǐ1t ì1t
i1w ī1w í1w ǐ1w ì1w
i1x ī1x í1x ǐ1x ì1x
i1y ī1y í1y ǐ1y ì1y
i1z ī1z í1z ǐ1z ì1z
1na 1nā 1ná 1nǎ 1nà
n1b
n1c
n1d
1ne 1nē 1né 1ně 1nè
n1f
n1h
1ni 1nī 1ní 1nǐ 1nì
n1j
n1k
n1l
n1m
n1n
1no 1nō 1nó 1nǒ 1nò
n1p
n1q
n1r
n1s
n1t
1nu 1nū 1nú 1nǔ 1nù
1nü 1nǖ 1nǘ 1nǚ 1nǜ
n1w
n1x
n1y
n1z
o1b ō1b ó1b ǒ1b ò1b
o1c ō1c ó1c ǒ1c ò1c
o1d ō1d ó1d ǒ1d ò1d
o1f ō1f ó1f ǒ1f ò1f
o1g ō1g ó1g ǒ1g ò1g
o1h ō1h ó1h ǒ1h ò1h
o1j ō1j ó1j ǒ1j ò1j
o1k ō1k ó1k ǒ1k ò1k
o1l ō1l ó1l ǒ1l ò1l
o1m ō1m ó1m ǒ1m ò1m
o1p ō1p ó1p ǒ1p ò1p
o1q ō1q ó1q ǒ1q ò1q
o1r ō1r ó1r ǒ1r ò1r
o1s ō1s ó1s ǒ1s ò1s
o1t ō1t ó1t ǒ1t ò1t
o1w ō1w ó1w ǒ1w ò1w
o1x ō1x ó1x ǒ1x ò1x
o1y ō1y ó1y ǒ1y ò1y
o1z ō1z ó1z ǒ1z ò1z
2r1b
2r1c
2r1d
2r1f
2r1g
2r1h
2r1j
2r1k
2r1l
2r1m
2r1n
2r1p
2r1q
2r1r
2r1s
2r1t
2r1w
2r1x
2r1y
2r1z
u1b ū1b ú1b ǔ1b ù1b
u1c ū1c ú1c ǔ1c ù1c
u1d ū1d ú1d ǔ1d ù1d
u1f ū1f ú1f ǔ1f ù1f
u1g ū1g ú1g ǔ1g ù1g
u1h ū1h ú1h ǔ1h ù1h
u1j ū1j ú1j ǔ1j ù1j
u1k ū1k ú1k ǔ1k ù1k
u1l ū1l ú1l ǔ1l ù1l
u1m ū1m ú1m ǔ1m ù1m
u1p ū1p ú1p ǔ1p ù1p
u1q ū1q ú1q ǔ1q ù1q
u1r ū1r ú1r ǔ1r ù1r
u1s ū1s ú1s ǔ1s ù1s
u1t ū1t ú1t ǔ1t ù1t
u1w ū1w ú1w ǔ1w ù1w
u1x ū1x ú1x ǔ1x ù1x
u1y ū1y ú1y ǔ1y ù1y
u1z ū1z ú1z ǔ1z ù1z
ü1b ǖ1b ǘ1b ǚ1b ǜ1b
ü1c ǖ1c ǘ1c ǚ1c ǜ1c
ü1d ǖ1d ǘ1d ǚ1d ǜ1d
ü1f ǖ1f ǘ1f ǚ1f ǜ1f
ü1g ǖ1g ǘ1g ǚ1g ǜ1g
ü1h ǖ1h ǘ1h ǚ1h ǜ1h
ü1j ǖ1j ǘ1j ǚ1j ǜ1j
ü1k ǖ1k ǘ1k ǚ1k ǜ1k
ü1l ǖ1l ǘ1l ǚ1l ǜ1l
ü1m ǖ1m ǘ1m ǚ1m ǜ1m
ü1n ǖ1n ǘ1n ǚ1n ǜ1n
ü1p ǖ1p ǘ1p ǚ1p ǜ1p
ü1q ǖ1q ǘ1q ǚ1q ǜ1q
ü1r ǖ1r ǘ1r ǚ1r ǜ1r
ü1s ǖ1s ǘ1s ǚ1s ǜ1s
ü1t ǖ1t ǘ1t ǚ1t ǜ1t
ü1w ǖ1w ǘ1w ǚ1w ǜ1w
ü1x ǖ1x ǘ1x ǚ1x ǜ1x
ü1y ǖ1y ǘ1y ǚ1y ǜ1y
ü1z ǖ1z ǘ1z ǚ1z ǜ1z
}

\endinput

%%% Local Variables:
%%% mode: tex
%%% coding: utf-8
%%% End:


==> cjk-4.8.5/utils/thaifont/tools/INSTALL <==
Installation of Thai fonts for TeX with fontinst
------------------------------------------------

0. The files `c90.etx' and `c90.mtx' must be in the TEXINPUTS path.
   Normally, the current directory also works.  Note that you need
   fontinst version 1.918 or higher.

1. In case your Thai font doesn't come with an AFM metrics file you
   must extract it from the font using tools like `type1afm' (from the
   t1lib package) or ghostscript's `ps2afm' program.

2. Create a control file for fontinst.

   Example:

     Let us assume that we have the following AFM files for the Garuda
     family, using version 0.5 of the `fonts-tlwg' project:

       garuda.afm
       garuda_b.afm
       garuda_o.afm
       garuda_bo.afm

     You should use glyph names compliant to Karl Berry's `fontname'
     scheme.  For `garuda', this could be `fgdr8z': `f' is the foundry
     (`small foundry'), `gd' is the typeface name, `r' means the
     weight (`regular'), and `8z' the encoding (`8bit user').
     Similarly, suitable names for the other fonts are `fgdb8z',
     `fgdo8z', and `fgdbo8z', respectively.

     Fonts with `f' as the supplier should go into a `public' font
     directory.  The typeface `Garuda' already exists in the latest
     fontname version (typeface.map version 4-Jul-2005 at the time of
     writing), the associated directory is `garuda'.  Please consult
     the `fontname' standard for more information.

     A template for the fontinst control file can be found as
     `garuda-c90.fontinst' which looks like the following.

     ==== garuda-c90.fontinst ====

       \input fontinst.sty

       \needsfontinstversion{1.918}


       % we explicitly set all slots in the encoding, so provide all
       % glyph names in AFM files equally (this is, don't create
       % `<glyph>-not' names)
       \let\setnotglyph \setrawglyph

       % we want warnings for missing glyphs
       \fontinstcc
       \add_to\pre_fourth_etx_pass_hook{
         \def\do_slot{
           \if_undefined{g-\slot_name}\then
             \fontinstwarningnoline{fontinst}
                                   {missing~glyph~`\slot_name'\space
                                    for~slot~\the\slot_number\space
                                    in~font~`\out_filename'}
           \fi
           \do_character
         }
       }
       \normalcc


       % create PL files and an FD file
       \installfonts
         \setint{fontdimen(2)}{500}  % SPACE
         \setint{fontdimen(3)}{300}  % STRETCH
         \setint{fontdimen(4)}{100}  % SHRINK
         \setint{fontdimen(6)}{1000} % QUAD
         \setint{fontdimen(7)}{0}    % EXTRASPACE

         \installrawfont{fdbr8z}{garuda,c90}{c90}
                        {C90}{garuda}{m}{n}{}
         \installrawfont{fdbb8z}{garuda_b,c90}{c90}
                        {C90}{garuda}{bx}{n}{}
         \installrawfont{fdbbo8z}{garuda_bo,c90}{c90}
                        {C90}{garuda}{bx}{sl}{}
         \installrawfont{fdbo8z}{garuda_o,c90}{c90}
                        {C90}{garuda}{m}{sl}{}
       \endinstallfonts


       \input finstmsc.sty


       % create the c90.enc file
       \installfonts
         % the `makeenc' flag is used in c90.etx
         \setint{makeenc}{1}
         \setstr{encodingname}{C90Encoding}
         \etxtoenc{c90}{c90}
       \endinstallfonts

       \end

     ==== garuda-c90.fontinst ====

     Some explanations.

     - The control files also create MTX and PL files for the AFM
       files (e.g., garuda.mtx and garuda.pl) which aren't needed and
       can be deleted.

     - AFM files don't provide all necessary font dimensions for TeX.
       Consequently, you have to set some dimensions manually.  The
       `SPACE' value must be larger than for a Latin font; a
       reasonable value is 500.  You should increase the `STRETCH'
       value also -- some tests have shown that 300 yields good
       results, but this depends on the font.  `EXTRASPACE' can be set
       to zero since you must always use TeX's \frenchspacing command
       for Thai.  All other font dimension values given above are
       default values and can stay unmodified.

       There is nothing for free: The changed font dimensions improve
       spacing between Thai words, but Latin words are far too widely
       spaced.

     - The arguments to \installrawfont are as follows.

         #1    The target font name.
         #2    A comma separated list (without spaces) of metric
               files.  Above, the first one is the AFM file, the
               second one is c90.mtx which sets up the three mandatory
               alias glyph slots.
         #3    The name of the encoding file (c90.etx).
         #4-#7 The NFSS attributes for the font.
         #8    The size command.  If it is empty, `<->' is used.

     - The second \installfonts...\endinstallfonts block creates an
       encoding file.

3. Run fontinst:

     tex garuda-c90.fontinst

   If you get warnings about missing glyphs which are critical (this
   is, if they affect Thai characters), you have to configure fontinst
   to use an alias file for glyph names.  This is described below.

4. Say

     pltotf <PL-file>

  for all target PL files to create TFM files.

  Example:

     pltotf fgdr8z
     pltotf fgdb8z
     pltotf fgdo8z
     pltotf fgdbo8z

  After the conversion, the PL files are no longer needed and can be
  deleted.  As mentioned above, the PL files created directly from the
  AFM files need not be converted.

5. Create a mapping file <font>.map for the PS fonts (which can be
   used by both dvips and pdftex).

   Example `garuda-c90.map' (the lines are split for readability only):

     fgdr8z Garuda \
       " C90Encoding ReEncodeFont " <c90.enc <garuda.pfb
     fgdb8z Garuda-Bold \
       " C90Encoding ReEncodeFont " <c90.enc <garuda_b.pfb
     fgdo8z Garuda-Oblique \
       " C90Encoding ReEncodeFont " <c90.enc <garuda_o.pfb
     fgdbo8z Garuda-BoldOblique \
       " C90Encoding ReEncodeFont " <c90.enc <garuda_bo.pfb

  A proper entry for the mapping file (dvipdfm.map) of dvipdfm (and
  dvipdfmx) looks like this:

     fgdr8z c90 garuda
     fgdb8z c90 garuda_b
     fgdo8z c90 garuda_o
     fgdbo8z c90 garuda_bo

  Note that teTeX's (and TeXLive's) `updmap' script can automatically
  convert a map line for dvips to a proper entry for dvipdfm and
  dvipdfmx.

6. There are two possibilities how to make the Thai fonts known to
   dvips.

  - Append the contents of the map file to `psfonts.map' (or the map
    file specified in the configuration file of dvips, `config.ps',
    with the `p' option).  How to do this may vary depending on the
    used TeX system; for example, teTeX and TeXLive both use a script
    called `updmap' to maintain `psfonts.map'.

  - Write a small file called config.<font> (e.g. `config.garuda-c90')
    with the following line in it:

      p +<map_file>

    Example:

      p +garuda-c90.map

    Then you can use the `-P' command line option of dvips to include
    the reencoded font.  Example:

      dvips -P garuda-c90 test.dvi

7. After testing, install the font and its support files in your TeX
   tree.  In the following example, `TEXMF' denotes the location of
   your (local) `texmf' directory (we assume a TeX installation
   compliant to TDS 1.1 as provided recent versions of TeXLive and
   teTeX).

     garuda.pfb    ->   TEXMF/fonts/type1/public/garuda/
     garuda.afm    ->   TEXMF/fonts/afm/public/garuda/
     ...

     c90.enc       ->   TEXMF/fonts/enc/dvips/thai/

     garuda.map    ->   TEXMF/fonts/map/dvips/garuda-c90/
     config.garuda ->   TEXMF/dvips/garuda-c90/

     fgdr8z.tfm    ->   TEXMF/fonts/tfm/public/garuda-c90/
     ...

     c90gar.fd     ->   TEXMF/tex/latex/CJK/thai/

8. Run texhash or a similar program to update the TDS database if
   necessary.


You are done!  With plain TeX, say e.g.

  \font\thai = fgdr9z at 16pt

to use the font \thai.  This will typeset TIS-620 encoded Thai.  Note,
however, that you need CJK's cjk-enc.el for Emacs to insert proper
inter-character glue and word breakpoints in case you want to typeset
longer Thai phrases.


Reencoding Thai fonts
---------------------

Older Thai fonts don't use proper glyph names, and recent ones
probably use different suffixes; it is thus necessary to make fontinst
aware of those names.

A complete example can be found in the `dbtt-old' subdirectory (which
can be used for the dbtt fonts from TeXLive 8 or earlier).

a. Set up a file which contains all the aliases, using the \galias
   macro.  This file should have the extension `.tex'.

   Example:

     If glyph `endash' is represented with glyph name `ucircumflex' in
     the font, use the following:

       \galias{ucircumflex}{endash}

b. Set up both ETX and MTX files which load the just created glyph
   alias file.  To do that, use the files `dbtt-old-alias.etx' and
   `dbtt-old-alias.mtx' as templates.  Leave everything unchanged
   except the line with \input which should load your glyph alias
   file.

c. Set up a proper fontinst control file.  Use `dbtt-old.fontinst' as
   a template, replacing the `dbtt-old-alias' items in the
   \installrawfont lines with the name of your MTX file.  Similarly,
   the three last lines in the second \installfonts...\endinstallfonts
   block should be adjusted accordingly.

d. Continue with item 3 above.  Note that in item 5, you have to use
   not `C90Encoding' but the encoding name defined with the \setstr
   line in your fontinst control file.


Using different LaTeX encodings for Thai
----------------------------------------

The used encoding scheme within the CJK package for Thai is `C90', but
it is straightforward to adapt it to other Thai encodings like `LTH'
by reordering the `\setslot ... \endsetslot' blocks in the file
`c90.etx'.

Currently, only CJK's cjk-enc.el output filter for Emacs needs the
Thai ligatures -- other Thai word segmentation programs like `swath'
or `cttex' already replace the input characters with proper glyph
variants.  Anyway, they don't harm, and it is on the TODO list of the
thailatex maintainers to finally use those ligatures also.


Printing c90.etx
----------------

It is possible to convert the main fontinst encoding file for Thai,
c90.etx, into a printable document.  To do so, you have to apply the
patch below to the file `fontdoc.sty' (which is part of the fontinst
package -- tested with fontinst version 1.926; newer versions have
already been corrected and don't need this patch), then simply say

  latex c90.etx


====================================================================


--- fontdoc.sty.old	Mon Feb  9 21:28:59 2004
+++ fontdoc.sty	Wed Jun 23 12:13:04 2004
@@ -1052,7 +1052,7 @@
 \x@cs\def{FD@lig-/LIG}#1#2{%
    \FD@typeset@string{\slot@name}${}*{}$\typeset@glyph{#1}%
    ${}\rightarrow{}$%
-   \FD@typeset@string{\slot@name}${}*{}$\typeset@glyph{#2}$%
+   \FD@typeset@string{\slot@name}${}*{}$\typeset@glyph{#2}%
 }
 \x@cs\def{FD@lig-LIG/}#1#2{%
    \FD@typeset@string{\slot@name}${}*{}$\typeset@glyph{#1}%
@@ -1085,7 +1085,7 @@
    \FD@typeset@string{\slot@name}${}*{}$\typeset@glyph{#1}%
    ${}\rightarrow{}$%
    \FD@typeset@string{\slot@name}${}*{}$%
-   \typeset@glyph{#2}${}*\lfloor$\typeset@glyph{#1}$}
+   \typeset@glyph{#2}${}*\lfloor$\typeset@glyph{#1}}
 \def\nextlarger#1{\Bheading{Next larger} \typeset@glyph{#1}}
 \def\makerightboundary#1{%
    \Bheading{Right boundary marker slot} designation \typeset@glyph{#1}%


---End of INSTALL---


==> cjk-4.8.5/utils/thaifont/tools/dbtt-old/dbtt-old-alias.tex <==
% dbtt-old-alias.tex

% Copyright (C) 1994-2021  Werner Lemberg <wl@gnu.org>
%
% This program is free software; you can redistribute it and/or modify
% it under the terms of the GNU General Public License as published by
% the Free Software Foundation; either version 2 of the License, or
% (at your option) any later version.
%
% This program is distributed in the hope that it will be useful,
% but WITHOUT ANY WARRANTY; without even the implied warranty of
% MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
% GNU General Public License for more details.
%
% You should have received a copy of the GNU General Public License
% along with this program in doc/COPYING; if not, write to the Free
% Software Foundation, Inc., 51 Franklin St, Fifth Floor, Boston,
% MA 02110-1301 USA

\galias{ucircumflex}{endash}
\galias{uacute}{emdash}
\galias{quotedbl}{quotedblleft}
\galias{quotedbl}{quotedblright}
\galias{quotesingle}{quoteright}
\galias{grave}{quoteleft}
\galias{florin}{uni0E48.low_left}
\galias{quotedblbase}{uni0E49.low_left}
\galias{ellipsis}{uni0E4A.low_left}
\galias{dagger}{uni0E4B.low_left}
\galias{daggerdbl}{uni0E4C.low_left}
\galias{circumflex}{uni0E48.low}
\galias{perthousand}{uni0E49.low}
\galias{Scaron}{uni0E4A.low}
\galias{guilsinglleft}{uni0E4B.low}
\galias{OE}{uni0E4C.low}
\galias{u008F}{uni0E4D.left}
\galias{u0090}{uni0E0D.descless}
\galias{quoteright}{uni0E31.left}
\galias{quotedblleft}{uni0E47.left}
\galias{quotedblright}{uni0E34.left}
\galias{bullet}{uni0E35.left}
\galias{emdash}{uni0E36.left}
\galias{endash}{uni0E37.left}
\galias{tilde}{uni0E48.left}
\galias{trademark}{uni0E49.left}
\galias{scaron}{uni0E4A.left}
\galias{guilsinglright}{uni0E4B.left}
\galias{oe}{uni0E4C.left}
\galias{Ydieresis}{uni0E10.descless}
\galias{exclamdown}{uni0E01}
\galias{cent}{uni0E02}
\galias{sterling}{uni0E03}
\galias{currency}{uni0E04}
\galias{yen}{uni0E05}
\galias{brokenbar}{uni0E06}
\galias{section}{uni0E07}
\galias{dieresis}{uni0E08}
\galias{copyright}{uni0E09}
\galias{ordfeminine}{uni0E0A}
\galias{guillemotleft}{uni0E0B}
\galias{logicalnot}{uni0E0C}
\galias{hyphen}{uni0E0D}
\galias{registered}{uni0E0E}
\galias{macron}{uni0E0F}
\galias{degree}{uni0E10}
\galias{plusminus}{uni0E11}
\galias{twosuperior}{uni0E12}
\galias{threesuperior}{uni0E13}
\galias{acute}{uni0E14}
\galias{mu}{uni0E15}
\galias{paragraph}{uni0E16}
\galias{periodcentered}{uni0E17}
\galias{cedilla}{uni0E18}
\galias{onesuperior}{uni0E19}
\galias{ordmasculine}{uni0E1A}
\galias{guillemotright}{uni0E1B}
\galias{onequarter}{uni0E1C}
\galias{onehalf}{uni0E1D}
\galias{threequarters}{uni0E1E}
\galias{questiondown}{uni0E1F}
\galias{Agrave}{uni0E20}
\galias{Aacute}{uni0E21}
\galias{Acircumflex}{uni0E22}
\galias{Atilde}{uni0E23}
\galias{Adieresis}{uni0E24}
\galias{Aring}{uni0E25}
\galias{AE}{uni0E26}
\galias{Ccedilla}{uni0E27}
\galias{Egrave}{uni0E28}
\galias{Eacute}{uni0E29}
\galias{Ecircumflex}{uni0E2A}
\galias{Edieresis}{uni0E2B}
\galias{Igrave}{uni0E2C}
\galias{Iacute}{uni0E2D}
\galias{Icircumflex}{uni0E2E}
\galias{Idieresis}{uni0E2F}
\galias{Eth}{uni0E30}
\galias{Ntilde}{uni0E31}
\galias{Ograve}{uni0E32}
\galias{Oacute}{uni0E33}
\galias{Ocircumflex}{uni0E34}
\galias{Otilde}{uni0E35}
\galias{Odieresis}{uni0E36}
\galias{multiply}{uni0E37}
\galias{Oslash}{uni0E38}
\galias{Ugrave}{uni0E39}
\galias{Uacute}{uni0E3A}
\galias{germandbls}{uni0E3F}
\galias{agrave}{uni0E40}
\galias{aacute}{uni0E41}
\galias{acircumflex}{uni0E42}
\galias{atilde}{uni0E43}
\galias{adieresis}{uni0E44}
\galias{aring}{uni0E45}
\galias{ae}{uni0E46}
\galias{ccedilla}{uni0E47}
\galias{egrave}{uni0E48}
\galias{eacute}{uni0E49}
\galias{ecircumflex}{uni0E4A}
\galias{edieresis}{uni0E4B}
\galias{igrave}{uni0E4C}
\galias{iacute}{uni0E4D}
\galias{icircumflex}{uni0E4E}
\galias{idieresis}{uni0E4F}
\galias{eth}{uni0E50}
\galias{ntilde}{uni0E51}
\galias{ograve}{uni0E52}
\galias{oacute}{uni0E53}
\galias{ocircumflex}{uni0E54}
\galias{otilde}{uni0E55}
\galias{odieresis}{uni0E56}
\galias{divide}{uni0E57}
\galias{oslash}{uni0E58}
\galias{ugrave}{uni0E59}
\galias{udieresis}{uni0E38.low}
\galias{yacute}{uni0E39.low}
\galias{Ucircumflex}{uni0E3A.low}

% end of dbtt-old-alias.tex

